Top-degree solvability for hypocomplex structures and the cohomology of left-invariant involutive structures on compact Lie groups

We use the theory of dual of Fr\'echet-Schwartz (DFS) spaces to establish a sufficient condition for top-degree solvability for the differential complex associated to a hypocomplex locally integrable structure. As an application, we show that the top-degree cohomology of left-invariant hypocomplex structures on a compact Lie group can be computed only by using left-invariant forms, thus reducing the computation to a purely algebraic one. In the case of left-invariant elliptic involutive structures on compact Lie groups, under certain reasonable conditions, we prove that the cohomology associated to the involutive structure can be computed only by using left-invariant forms.

==> chp-involutive-structures-old.tex <==
\chapter{Involutive structures}
\label{chp:involutive_structures}

In this chapter, we will introduce the basic definitions regarding involutive structures along with some tools to study them. The main concepts introduced here are the concept of involutive structure, the associated differential operators and their cohomology spaces, which are the main objects of study in this work.

The tools introduced in this chapter are: \v Cech cohomology, Hodge decomposition and Serre duality. With the Hodge decomposition we establish a relation between the kernel of a partial differential operator and the cohomology spaces mentioned above. With \v Cech cohomology we are able to connect some analytical properties of involutive structures with some topological properties of the cohomology spaces the associated differential operators. With Serre duality, and the topological information obtained with \v Cech cohomology and the Hodge decomposition, we can use results obtained in some cohomology degrees with some complimentary degrees, or ``dual'' degrees.

\v Cech cohomology, Hodge decomposition and Serre duality are going to play a major role in Chapter \ref{chp:involutive_structures_on_compact_lie_groups}.


% hypocomplex structures

\section{Preliminares}

Let $\Omega$ be a smooth manifold and denote by $N$ its dimension. We will always assume that $N \geq 2$. An involutive structure on $\Omega$ is a smooth subbundle $\mathcal V$ of the complexified tangent bundle $\C T \Omega$ of $\Omega$ that satisfies the involutive, or Frobenius, condition $[\mathcal V, \mathcal V] \subset \mathcal V$. We will always denote the rank of $\mathcal V$ by $n$. We denote by $\Lambda^k$ the bundle $\Lambda^k \C T^* \Omega$ and by $\mathcal C^\infty(\Omega; \Lambda^k)$ the space of sections of $\Lambda^k$ with smooth coefficients. % in the sheaf $\mathcal F$. We will be using the following sheaves $\mathcal F = \mathcal D'$ and $\mathcal F = \mathcal C^\infty$.



% It is well known that to each involutive  structure is associated a complex  of differential  operators, and from that point of view, they are well studied in partial differential equations.

There is a natural differential complex associated to each involutive structure $\mathcal{V}$. We briefly recall the construction of such complexes. For each $x \in \Omega$, we define $$T'_x = \{ u \in \C T^*_x \Omega: u(X) = 0 ~ \forall X \in \mathcal V_x \}$$ and we have that
$ T' = \bigcup_{x \in \Omega} T'_x $
is a vector subbundle of $\C T^*\Omega$. For each $p, q \in \Z_+$, we denote by $T^{p,q}_x$ the subspace of $\Lambda^{p+q} \C T_x^*\Omega$ consisting of linear combinations of exterior products $u_1 \wedge \ldots \wedge u_{p+q}$ with $u_j \in \C T_x^*\Omega$ for $j = 1, \ldots, p+q$ and at least $p$ of these factors belonging to $T'_x$. Notice that $T^{p+1,q-1}_x \subset T^{p,q}_x$ and so we can define $\Lambda^{p,q}_x \doteq  T^{p,q}_x / T^{p+1,q-1}_x$ and $\Lambda^{p,q} = \bigcup_{x \in \Omega} \Lambda^{p,q}_x $ is a smooth vector bundle over $\Omega$. Since $\mathcal{V}$ is involutive we can easily verify that the exterior derivative take smooth sections of $T^{p,q}$ into smooth sections of $T^{p,q+1}$ and there exist a unique operator $\dext^{p,q}$ such that the diagram
$$
\xymatrix{
 T^{p,q} \ar[r]^{\dext} \ar[d]_{\pi_{p,q}}& T^{p,q+1} \ar[d]^{\pi_{p,q+1}} \\
\Lambda^{p,q} \ar[r]_{\dext^{p,q}} & \Lambda^{p,q+1}
}
$$
is commutative, with $\pi_{p,q} : T^{p,q} \to \Lambda^{p,q}$ being the quotient map.

When there is no risk of confusion, we will simplify the notation and write only $\dext '$ for the operator $\dext^{p,q}$, or $\dext'_{\mathcal V}$ when it is necessary to emphasize the associated involutive structure.

We denote by $\mathcal C^\infty(\Omega; \Lambda^{p,q})$ %, or $\Lambda^{p,q}(\Omega)$,
the space of sections of $\Lambda^{p,q}$ with smooth coefficients. % in the sheaf $\mathcal F$. To emphasize the associated involutive structure, we again use a subindex and we write $\Lambda^{p,q}_{\mathcal V}$. % or $\Lambda^{p,q}_{\mathcal V}(\Omega)$.
Notice that the operator $\dext'$ maps smooth sections of $\Lambda^{p,q}$ into smooth sections of $\Lambda^{p,q+1}$ and it also holds that $\dext' \circ \dext' = 0$. Therefore, for each $p \geq 0$ the operator $\dext'$ defines a complex of $\C$-linear mappings with coefficients in $\mathcal C^\infty$.
\begin{equation}
\label{h_complex}
 \mathcal C^\infty(\Omega; \Lambda^{p,0}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,1})  \xrightarrow{\dext'} ... \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \xrightarrow{\dext'} \ldots
\end{equation}

% Of course we also have a complex for the sheave of distributions $\mathcal D'$ and $\mathcal F = \mathcal B$.

For each $p \geq 0$ we denote the set of the $(p,q)$-cocycles elements by
$$ Z^{p,q} (\Omega; \mathcal V) = \ker \left( \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \right),$$
the set of $(p,q)$-coboundaries by
 $$ B^{p,q} (\Omega; \mathcal V) = \img \left( \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q-1}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q}) \right),$$
and the $(p,q)$-cohomology classes by
 $$  H^{p,q} (\Omega; \mathcal V) = \frac{Z^{p,q} (\Omega; \mathcal V)}{B^{p,q} (\Omega; \mathcal V)}.$$


Given any open set $V \subset \Omega$ we can restrict the involutive structure $\mathcal V$ to $V$, which we still denote by $\mathcal V$, and construct a complex $\left( \mathcal C^\infty(V; \Lambda^{p,q}), \dext' \right)$. And, by restriction, we have a complex homomorphism
$$ \left( \mathcal C^\infty(\Omega; \Lambda^{p,q}), \dext' \right) \to \left( \mathcal C^\infty(V; \Lambda^{p,q}), \dext' \right).$$ For a given $x \in V$, we define $$ \mathcal H^{p,q} (\{x\}; \mathcal V) = \varinjlim_{V \ni x} H^{p,q}(V; \mathcal V) $$ the inductive limit of $H^{p,q}(V; \mathcal V)$ with $V \ni x$. We can also construct the complex with coefficients being distributions over $V$, in this case we denote the cohomology space by
$   H^{p,q}_{\mathcal D'} (V; \mathcal V).$ In general, if $F(V) \subset \mathcal D'(V)$ is a convenient subspace, we denote by $F(\Omega; \Lambda^{p,q})$ %, or $\Lambda^{p,q}(\Omega)$,
the space of sections of $\Lambda^{p,q}$ with coefficients in $F$ and we denote the cohomology of $\dext'$ with coefficients in $F(V)$ by $ H^{p,q}_{F} (V; \mathcal V).$


\begin{exa}
By taking $\mathcal V = \C T \Omega$ we have the simplest involutive structure. In this case the operator $\dext'$ is just the usual exterior derivative. In this case, the space $H^p_{\mathcal C^\infty} (\Omega; \mathcal V)$ is just the de Rham cohomology space.
\end{exa}


\begin{exa}
Suppose that $J : T \Omega \to T \Omega$ is a vector bundle isomorphism satisfying $J \circ J = -\operatorname{Id}$ and
\begin{equation}
\label{chp:inv:j_complex}[JX, JY] = [X,Y] + J[JX, Y] + J[X,JY].
\end{equation} We extend $J$ complex-linearly to the complexified tangent bundle $\C T \Omega$ and we take $\mathcal V = \ker(J - i{\operatorname{Id}})$. The condition \eqref{chp:inv:j_complex} implies that  $\mathcal V$ is involutive. This structure is called a \emph{complex structure} over $\Omega$ and in this case, the operator $\dext'$ is the Doubeault operator $\delbar$.
\end{exa}

The structure $\mathcal V$ is always going to be considered to be locally integrable. We recall the standard coordinates and the generators associated to $\mathcal V$. For a detailed discussion on this topic we refer to \cite{treves1992hypo}.
Each point in $p \in \Omega$ is the center of a coordinate system $(x,t) = (x_1, \ldots, x_m, t_1, \ldots, t_n)$ defined on an open neighborhood of $p$ denoted by $U$ such that $(x(p),t(p)) = (0,0) \in \R^m \times \R^n$.
On $U$ it is defined a smooth function $\phi(x,t) = (\phi_1(x,t), \ldots, \phi_m(x,t))$ satisfying $\phi(0,0) = 0$ and $\phi_x(0,0) = 0$ such that the differentials of the functions
\begin{equation}
\label{chp:inv:first_integrals}
Z_k(x,t) = x_k + i\phi_k(x,t), \quad k = 1, \ldots, m
\end{equation}
 are linearly independent and span $T'$ over $U$. If we define the vector fields $$M_k = \sum_{j=1}^m \mu_{kj}(x,t) \frac{ \del }{ \del x_j}, \quad k = 1, \ldots, m,$$
characterized by the rule $M_kZ_j = \delta_{k,j}$ for $k,j = 1, \ldots, m$, then the complex vector fields
$$ L_j = \frac{ \del }{ \del t_j} - i\sum_{k=1}^m \frac{ \del \phi_k }{ \del t_j }(x,t)M_k, \quad j = 1, \ldots, n, $$
span $\mathcal V$ over $U$. The vector fields $L_j$ and $M_k$ are pairwise commutative.

The differentials $\dext t_k$, for $k = 1, \ldots, n$, span a bundle over $U$ which is, in a sense, supplementary to $T'$. Therefore we can adjoin them with $\dext Z_k$, for $k = 1, \ldots, m$, to get a smooth basis for $\C T^* \Omega$. So if $f$ is a smooth section of $\Lambda^{p,q}$ over $U$ we have the following unique representation for $f$
$$ f = \sum_{|J| = p} \sum_{|K| = q} f_{J,K}(x,t) \dext Z_J \wedge \dext t_K.$$

The standard representation of $\dext'f$ over $U$ is
$$ \dext' f = \sum_{|J| = p} \sum_{|K| = q} \sum_{l=1}^n \left( L_l  f_{J,K} \right) (x,t) \dext t_l \wedge \dext Z_J \wedge \dext t_K. $$


%%%%%%%%%%%%%%%%%
%%% LEVI FORM %%%
%%%%%%%%%%%%%%%%%

Let $T^0_x =  T'_x \cap \C T^*_x \Omega$. The \emph{Levi form} at a point $\xi \in T^0_x$ is the Hermitian form on $\mathcal V_x$ defined by $$\mc L_{(x,\xi)}(v,w) = (-i/2)\xi([L,\overline{M}]_x), \quad v,w \in \mathcal V_x$$ in which $L$ and $M$ are any smooth local sections of $\mathcal V$ in a neighborhood of $x$ such that $L_x = v$ and $M_x = w$. We shall say that $\mc L$ is \emph{nondegenerate} if given any point $\xi \in T^0_x$, with $ \xi \neq 0$, and any $v \in \mathcal V_x$, with $v \neq 0$, there is some $w \in \mathcal V_x$ such that
$ \mc L_{(x,\xi)}(v,w) \neq 0.$ % If the involutive structure $\mathcal V$ has nondegenerate Levi form, under some conditions about the eigenvalues of the Levi form, the associated Hodge Laplacian is subelliptic \cite{hanges1995involutive}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HODGE DECOMPOSITION %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Hodge decomposition}
\label{sec:hodge_theory}

In this section we are going to explain how to use the Hodge decomposition for the operator $\dext'$. With this decomposition we are going to find some simple conditions so that the cohomology is finite dimensional on a specific degree. Usually, Hodge decomposition is introduced in the context of elliptic differential operators between Hermitian vector bundles. Here we made a small improvement, we assumed that the operator is subelliptic. See Definition \ref{dfn:subellipticity_and_stuff}.

Suppose that $\Omega$ is a compact manifold with a positive $\mathcal C^\infty$-density $\mu$ and let $E_j$, for $j = 1, 2, 3$ be three Hermitian vector bundles over $\Omega$. We denote by $\ip{,}_j$ the hermitian inner product on $E_j$. Let $$A_j : \mathcal C^\infty(\Omega; E_j) \to \mathcal C^\infty(\Omega; E_{j+1}), \qquad j = 1, 2$$ be partial differential operators of order $m$ satisfying $A_2 \circ A_1 = 0$. That is we have
$$ \mathcal C^\infty(\Omega; E_1) \xrightarrow{A_1}{} \mathcal C^\infty(\Omega; E_{2})  \xrightarrow{A_2}{}  \mathcal C^\infty(\Omega; E_3).$$

We endow $\mathcal C^\infty(\Omega; E_j)$ with the inner product
$$\iip{u,v}_j \doteq \int_\Omega \ip{u(x),v(x)}_j \dint \mu(x),$$
for $u, v \in \mathcal C^\infty(\Omega; E_j)$ and we  define the operators $A_j^* : \mathcal C^\infty(\Omega; E_{j+1}) \to \mathcal C^\infty(\Omega; E_{j})$ by
$$ \iip{A_j u, v }_{j+1} = \iip{u, A^*_j v}_{j+1}$$
for $u \in \mathcal C^\infty(\Omega; E_{j})$ and $v \in \mathcal C^\infty(\Omega; E_{j+1}).$

Now we have everything we need to introduce the Hodge operator:

\begin{dfn}
For $u \in \mathcal C^\infty(\Omega; E_2)$ we define $\Box u \doteq (A_1 A_1^* + A_2^* A_2) u$, and, in the sense of distributions, we define $$D(\Box) = \{u \in L^2(\Omega; E_2): \Box u \in L^2(\Omega; E_2) \}$$ and $$\Box : D(\Box) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ is a densely defined operator called \emph{Hodge operator}, \emph{Hodge Laplacian} or just \emph{Box operator}.
\end{dfn}

% because $\mathcal C^\infty(\Omega; E_2) \subset D(\Box)$ is a dense subset of $L^2(\Omega; E_2)$.

The operator $\Box$ has closed graph. In fact, let $u_j, v_j \in L^2(\Omega; E_2)$ be a sequence satisfying $\Box u_j = v_j$ and suppose that $u_j \to u \in L^2(\Omega; E_2)$ and $v_j \to v \in L^2(\Omega; E_2)$. We want to show that $u \in D(\Box)$ and $\Box u = v$. Since $u_j \to u$ and $v_j \to v$ in $L^2(\Omega; E_2)$ we have have this convergence in $\mc D'(\Omega; E_2)$ and since $\Box$ is a differential operator it is continuous in $\mc D'(\Omega; E_2)$ so we can apply the closed graph theorem and conclude that $\Box u = v$ in the sense of distributions. By hypothesis we have $u,v \in L^2(\Omega; E_2)$ and so $u \in D(\Box)$.

We also remark that
$$
\begin{aligned}
\iip{\Box u, u}
	& = \iip{A_1 A_1^*u, u} + \iip{A_2^* A_2u, u} \\
	& = \iip{A_1^*u, A_1^*u} + \iip{A_2 u, A_2 u} \\
	& = \|A_1^*u\|_1^2 + \|A_2 u\|_3^2
\end{aligned}
$$
and so we have the following result:

\begin{prp}
\label{prp:kernel_Box_decomposition} The kernel of the operator $\Box$ is
$$ \ker \Box = \{u \in L^2(\Omega; E_2): A_1^*u = 0 \text{ and } A_2 u = 0\}. $$
\end{prp}

In the following definition we introduce two concepts regarding the regularity of differential operators. Under certain conditions, these concepts provide sufficient conditions so that the kernel of the differential operator has finite dimension.

\begin{dfn}
\label{dfn:subellipticity_and_stuff} Let $E$ be a vector bundle over $\Omega$ and consider a linear partial differential operator $P : \mc D' (\Omega; E) \to \mc D'(\Omega; E)$. For an $\epsilon > 0$, the operator $P$ is said to be \emph{$\epsilon$-subelliptic} if $Pu \in H^s(\Omega;E)$ implies that $u \in H^{s+\epsilon}(\Omega; E)$ for all $u \in H^s(\Omega; E)$. The operator $P$ is said to be \emph{globally hypoelliptic} if, given $u \in \mc D'(\Omega; E)$ such that $Pu \in \mathcal C^\infty(\Omega;F)$ it holds that $u \in \mathcal C^\infty(\Omega;E)$. Notice that subellipticity implies global hypoellipticity.
\end{dfn}

On the above definition it is not necessary to assume that the manifold $\Omega$ is compact.

The following proposition is a well known result about differential operators on compact manifolds.

\begin{prp} If $P : \mc D' (\Omega; E) \to \mc D'(\Omega; F)$ is global hypoelliptic, then $\dim \ker P < \infty.$
\end{prp}

\begin{proof}
Since $P$ is globally hypoelliptic we have that $\ker P \subset \mathcal C^\infty(\Omega; E)$. Consider $\ker P$ with the topology induced by $L^2(\Omega; E)$. Notice that this induced topology agrees with the topology induced by $H^s(\Omega; E)$ for any $s \in \R$ and take $B = \{ u \in \ker P: \|u\|_1 \leq 1 \}$ and note that $B$ is closed and bounded. By the Rellich lemma, we know that the inclusion $H^1(\Omega; E) \to H^0(\Omega; E) = L^2(\Omega; E)$ is compact and so $B$ is compact.
\end{proof}

In this work we are interested in the case in which $P$ is the Hodge operator. Therefore, we need to establish some conditions so that the Hodge operator is globally hypoelliptic. But first we need to finish our decomposition. We need the next lemma which is a basic result on Hilbert spaces.

\begin{lem}
Let $H_1$ and $H_2$ be Hilbert spaces with norms $\|.\|_1$ and $\|.\|_2$. If $T : H_1 \to H_2$ is a linear, closed and densely defined operator such that there is a constant $C > 0$ such that
$$\|f\|_1 \leq C \|Tf\|_2$$
for all $ f \in D(T) \cap \overline{\img(T^*)}$,
then $\img(T)$ is closed.
\end{lem}

\begin{proof}
Let $f_k \in \img(T)$ such that $f_k \to f$ in $H_2$. We want to show that there exist $g \in D(T)$ satisfying $Tg = f$. Let $g_k \in D(T)$ with $Tg_k = f_k$. Since $\ker T^\perp = \overline{\img(T^*)}$, we can assume that $g_k \in \overline{\img (T^*)}$. Notice that we have
$$\|g_k - g_l\|_1 \leq C\|Tg_k - Tg_l \|_2 = C\|f_k - f_l\|_2.$$
Since $\{f_k\}$ is a convergent sequence, it is a Cauchy sequence and so also is $\{g_k\}$. Therefore there exists $g \in H_1$ with $g_k \to g$. Since $T$ has closed graph we have that $(g_k, f_k) \to (g,f) \in \{(x, Tx): x \in H_1\}$ and so $f = Tg$.
\end{proof}

This next proposition shows another important result regarding subellipticity of the Hodge operator. By itself this proposition is interesting, but it is also necessary for the decomposition.

\begin{prp} If the operator $\Box$ is $\epsilon$-subelliptic, then $\img(\Box)$ is closed in $L^2(\Omega; E_2).$
\end{prp}

\begin{proof} We already know that $\Box$ is a linear, densely defined and closed operator. Since $\Box$ is $\epsilon$-subelliptic, we have that if $u \in D(\Box)$ then $u \in H^\epsilon(\Omega; E_2)$ and there exists a constant $C > 0$ such that
$$ \|u\|_\epsilon \leq C (\|\Box u\|_0 + \|u\|_0)$$
for all $u \in H^\epsilon(\Omega; E_2)$. So, if $u \in (\ker \Box)^\perp \cap D(\Box)$, we have that $$\|u\|_\epsilon \leq C \|\Box u\|_0$$
and clearly
$$\|u\|_0 \leq C \|\Box u\|_0.$$
The result follows from the preceding lemma.
\end{proof}

Now we are going to see that even with weaker conditions, the Hodge Laplacian still has some nice properties.

\begin{prp}
Suppose that $\Box$ is $\epsilon$-subelliptic. Let $D(T) = H^{\epsilon}(\Omega; E_2)$ and define $$T : D(T) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ by $Tu = \Box u$ for $u \in D(T)$. Then $T$ is a self-adjoint operator. Particularly, we have $$L^2(\Omega;E_2) = \ker T \oplus \img T.$$
\end{prp}

\begin{proof}
 Notice that $$\iip{\Box u, v}_2 = \iip{u, \Box v}_2$$
for all $u, v \in \mathcal C^\infty(\Omega; E_2).$ Since $\mathcal C^\infty(\Omega; E_2)$ is a dense subset of $H^{\epsilon}(\Omega; E_2)$, given $u, v \in H^{\epsilon}(\Omega; E_2)$ there exist sequences $\{u_j\}$ and $\{v_j\}$ in $\mathcal C^\infty(\Omega; E_2)$ such that $u_j \to u$ and $v_j \to v$ in $H^{\epsilon}(\Omega; E_2)$ and so
$\Box u_j \to \Box u$ and $\Box v_j \to \Box v$ in $L^2(\Omega; E_2)$ and since $$\iip{\Box u_j, v_j}_2 = \iip{u_j, \Box v_j}_2$$
for all $j$. Therefore we conclude that $\iip{\Box u, v}_2 = \iip{u, \Box v}_2$ and so $\iip{T u, v}_2 = \iip{u, T v}_2$ and $T$ is a symmetric operator.

To conclude we have to show that $D(T) = D(T^*)$. Let $v \in D(T^*)$. The operator $$ u \in D(T) \mapsto \iip{Tu, v}_2 $$ is continuous in $D(T)$ and so there exists a constant $C > 0$ such that
$$ |\iip{Tu, v}_2 | \leq C\|u\|_2, \qquad \forall u \in D(T).$$
Particularly, if we define $S \in \mc D'(M; E_2)$ by $S(\phi) = \iip{T\phi, u}$ for $\phi \in \mathcal C^\infty(\Omega; E_2)$, we have that there exists $w \in L^2(\Omega; E_2)$ such that $\iip{T \phi, u}_2 = \iip{\phi,w}_2$ and so $$ \overline{w}(\phi) = \overline{u}(\Box \phi)$$ for all $\phi \in \mathcal C^\infty(\Omega; E_2)$, that is $\Box \overline{u} = \overline{w}$ in $\mc D'(\Omega;E_2)$ and since $w \in L^2(\Omega;E_2)$ we have $w \in H^{\epsilon}(\Omega;E_2) = D(T)$.
\end{proof}

Assume that $\Box$ is $\epsilon$-subelliptic. We have that there exists $C > 0$ satisfying
$$ \|u\|_0 \leq C\|\Box u\|_0$$
for all $u \in D(\Box) \cap \ker \Box^\perp$ and according to Lemma 4.1.1 in \cite{hormander1973introduction} given any $f \in \ker \Box^\perp$ there is $u \in L^2(\Omega; E_2)$, $\|u\|_0 \leq C \|f\|_0$ such that $\Box u = f$. Let $\Pi$ denote the orthogonal projection on $\ker \Box^\perp$ and, for $f \in L^2(\Omega; E_2)$ let $Gf$ be the unique solution to $\Box u = \Pi f$ which is orthogonal to the kernel of $\Box$ in $L^2(\Omega; E_2)$. Then $G : L^2(\Omega; E_2) \to L^2(\Omega; E_2)$ is bounded, with norm $ \leq C$, and $\Box G = \Pi$ in $L^2(\Omega; E_2)$. We shall refer to $G$ as the Green operator of $\Box$.

And we have everything we need to prove the main result of this section.

\begin{prp} If $\Box$ is $\epsilon$-subelliptic, then
we have the Hodge decomposition
\begin{equation}
	\label{eq:hodge_decomposition}
	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box(\mathcal  C^\infty(\Omega;E_2) ) .
\end{equation}
and
\begin{equation}
	\label{eq:hodge_decomposition_isomorphism}
	\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.
\end{equation}

\end{prp}

\begin{proof} Let $f \in \mathcal C^\infty(\Omega; E_2)$. We write $f = f_1 + f_2$ with $f_1 \in \ker \Box $ and $f_2 \in \img(T)$. Since $f_2 \in \img(\Box)$ we can write $f_2 = \Box u$ for some $u \in H^\epsilon(\Omega; E_2)$. Notice that since $\Box f_1 = 0$ we have $f_1 \in \mathcal C^\infty(\Omega;E_2)$ and so $f_2 = f - f_1 \in \mathcal C^\infty(\Omega;E_2)$ and since $f_2 = \Box u$ we have $u \in \mathcal C^\infty(\Omega;E_2)$ and we obtained the Hodge decomposition:
$$ \mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box( \mathcal C^\infty(\Omega;E_2) ) .$$

If $u \in \mathcal C^\infty(\Omega;E_2)$ such that $A_2u=0$, then we can write $u = u_1 + \Box u_2$ with $\Box u_1 = 0$ and $u_2 \in \mathcal C^\infty(\Omega;E_2).$ We have $u = u_1 + A^*_2 A_2 u_2 + A_1 A^*_1 u_2$. Applying $A_2$ on both sides of this equality and using Proposition \ref{prp:kernel_Box_decomposition} we conclude that
$$ A_2 A^*_2 A_2 u_2 = 0.$$
We have $A_2^*A_2 u_2 = 0$ because $\iip{A_2^* A_2 u_2, A_2^* A_2 u_2} = \iip{A_2 u_2, A_2 A_2^* A_2 u_2} = 0$ and then $u = u_1 + A_1 A^*_1 u_2,$ that is $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.$$
\end{proof}

The following version of the decomposition is more suitable for the application in this work.

\begin{prp} If $\Box$ is $\epsilon$-subelliptic, then
we have the decomposition
\begin{equation}
	\label{eq:second_hodge_decomposition}
	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus A_1 ( \mathcal C^\infty(\Omega;E_1) ) \oplus A_2^* (\mathcal C^\infty(\Omega;E_3)).
\end{equation}
The space $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} $$ is isomorphic to $\ker \Box$ with each equivalence class in the former having a unique representative in the latter.
\end{prp}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HYPOANALYTIC STRUCTURES %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Hypocomplex structures}

In this section we are going to introduce the concept of hypocomplex structures, a class of structures with some good analytical properties very similar to the class of holomorphic functions. Such analytical properties are going to be used to find conditions so that the operator $\dext'$ has closed range. The main applications of this condition are Theorem \ref{thm:li:thm:duality_of_left} and Theorem \ref{thm:left_invariance_on_degree}.

Let $x \in \Omega$. We denote by $\mathcal S(x)$ the ring of germs of solutions of $\mathcal V$ at $x$, that is
$$ \mathcal S(x) = \{ f \in \mathcal C^\infty(x) : \dext' f = 0 \}$$
and we denote by $\mathcal O^m_0$ the ring of germs holomorphic functions defined in a neighborhood of $0$ in $\C^m$.

Now, consider the integrals $Z_1, \ldots, Z_m$ as in \eqref{chp:inv:first_integrals} defined in an open neighborhood of $p$ and denote by $Z$ the map $Z(x) = (Z_1(x), \ldots, Z_m(x))$ for $x$ in a neighborhood of $p$. We define a ring homomorphism
$$ \Lambda : h\in \mathcal O^m_0 \mapsto  h \circ Z \in  \mathcal S(p). $$
% defined by $$ \Lambda (h) = h \circ Z.$$
 We say that $\mathcal V$ is \emph{hypocomplex} at $p$ if $\Lambda$ is surjective, that is, if for every $f \in \mathcal S(p)$ there exist a holomorphic function $h \in \mathcal O^m_0$ such that $f = h \circ Z$. % We say that $\Omega$ is a \emph{hypocomplex manifold} if the involutive structure is
Notice that the map $x \mapsto Z(x) = x + i\phi(x, 0)$ defines the germ at 0 of a maximally real submanifold $\Sigma \subset \C^m$ and since for $h \in \mathcal O^m_0$, if $h|_\Sigma = 0$ then we have $h = 0$. This implies that $\Lambda$ is an injective homomorphism.

The following definition is going to be useful in the next section.

\begin{dfn}
We shall say that the locally integrable structure $\mathcal V$ satisfies the \emph{unique continuation property} if given any $u \in \mathcal D'(\Omega; \Lambda^{p,q})$ satisfying $\dext' u = 0$ in a non-empty open subset $U \subset \Omega$, then $u$ vanishes identically in $\Omega$.
\end{dfn}

It follows directly from the definition that hypocomplex structures satisfies the unique continuation property.

%\begin{dfn} Let $\Omega$ be a manifold endowed with a locally integrable structure $\mathcal{V}$. We denote by $N$ the dimension of $\Omega$,  by $n$ the rank of $\mathcal V$, and we write $m = N - n$. We say that  $\mathcal V$ is \emph{hypocomplex} if for each point $p \in \Omega$ there exist a neighborhood $U$ of $p$ and a smooth map $Z = (Z_1, \ldots, Z_m) : U \to \C^m$ whose components are solutions of the involutive structure $\mathcal V$. These coordinates have the following property: to any distributional solution $h$ of $\mathcal V$ in some open neighborhood of $p$ there is an holomorphic function $\tilde h$ in a neighborhood of $Z(p)$ in $\C^m$ such that $h = \tilde h \circ Z$..
%\end{dfn}

We will use the terminology FS to refer to the class of Fréchet-Schwartz spaces (cf. \cite{bourbaki2007espaces}). We will recall some stability properties of this class: if $E$ is an FS space and $F \subset E$ is a closed subspace then $F$ and $E/F$ are FS spaces. If $\{E_n\}$ is a sequence of FS spaces then the topological product $\prod_n E_n$ also is a FS space. Moreover, every FS space is a Montel space and consequently it is reflexive.

We shall use the terminology DFS to denote the class of strong duals of FS spaces. It follows that the space in this class are also Montel spaces and that closed subspaces and quotients by closed subspaces of DFS spaces also are DFS spaces. If ${E_n}$ is a sequence of DFS spaces, then the topological direct sum $\bigoplus_n E_n$ is a DFS space. Every DFS space is the inductive limit of an increasing sequence $E_n \subset E_{n+1}$ of Banach spaces, the injection maps being compact (cf. \cite{morimoto1993introduction}). We also suggest the reader to consult \cite{komatsu1967projective} and the references therein for an exposition on this subject.

For each open set $U \subset \Omega$ and for integers $p = 0, 1, \ldots, m$ we denote by $ \mathcal S^p(U)$ the set of all $u \in \mathcal C^\infty(U; \Lambda^{p,0})$ satisfying $\dext' u = 0$ on $U$. The space $\mathcal S^p(U)$ of sections of $\mathcal S^p$ over $U$ is %a closed subspace of $\mathcal C^\infty(U; \Lambda^{p,0})$ and thus is
an FS space. % It is possible to show that the space $\mathcal S^p(U)$ is a Montel space \cite{treves2016topological}.

The following basic result will be useful.

\begin{lem}
\label{hypocomplex_compact_restriction} Let $U$ and $V$ be open subsets of $\Omega$ and suppose that $\overline V \subset U$ and that $U$ is small enough so we have the standard coordinates introduced in the beginning of this chapter, then the mapping $\rho^U_V : \mathcal S^p(U) \to \mathcal S^p(V) $
is compact.
\end{lem}

\begin{proof}
We denote by $\Phi_{\mathcal S^p(U)}(0)$ the system of open neighborhoods of the origin defining the topology of $\mathcal S^p(U)$. Let $\epsilon > 0$ and consider $W \in \Phi_{\mathcal S^p(U)}(0)$ be given by
$$ W = \{ u \in \mathcal S^p(U) : u = \sum_{|I| = p} u_I \dext t_I \text{ and } \sup_{\overline{V}} |u_I| < \epsilon \text{ for } |I| = p\}.$$ The image of $W$ under $\rho^U_V$ is bounded and so it is relatively compact.
\end{proof}


If $K \subset \Omega$ is a compact set then $\mathcal S^p(K)$ will be the inductive limit of the spaces $\mathcal S^p(U)$ when $U$ runs over the set of all open neighborhoods of $K$. This is a DFS space. If $K'$ is a compact subset of the interior of $K$ then the restriction map $\mathcal S^p(K) \to \mathcal S^p(K')$ also is compact. The space $\mathcal S^p(K)$ is a DFS space.








\subsection{Sheaf cohomology}

In this section we will always be assuming that $\mathcal V$ is hypocomplex. Let $\mathcal S^p$ be the sheaf $(p,0)$-forms which are solutions of solutions of $\mathcal V$ over $\Omega$ and denote by $\Phi$ a paracompactifying family of supports in $X$. We denote by $H^q_\Phi(\Omega; \mathcal S^p)$ the \emph{cohomology group over $\Omega$ with coefficients in $\mathcal S^p$ and support in $\Phi$}. We are interested in the familty of supports consisting of all compacts subsets of $\Omega$ which is going to be denoted by $c$. % We are interested particularly in the topological properties of $H^1_c(\Omega; \mathcal S^p)$.

Following \cite{gunning1965analytic}, we will recall some notions related to \v Cech cohomology of a covering with values in a sheaf which will allow us to use functional analysis to study the operator $\dext'$ and the space $H^1_c(\Omega; \mathcal S^p)$. % The main reason for using \v Cech cohomology in this work is to be able to study cohomology of the operator $\dext'$ using tools from functional analysis. % But first we need the following:

This sheaf cohomology can be related to the cohomology introduced in the beginning of this chapter  via spectral sequence (cf. \cite{godement1958topologie} Théorème 5.2.4). A particular case of this can be done in locally trivial cohomologies which is the case of elliptic structures, for example. In fact, if the involutive structure $\mathcal V$ is elliptic, by the Poincaré Lemma for elliptic structures \cite{berhanu2008introduction} Theorem VIII.3.1, we know that $\dext'$ is locally exact, so we have a fine resolution of $\mathcal S$. Therefore we have for $q > 0$

$$ H^q(\Omega; \mathcal S^p) = \frac { \ker \left[ \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \right] }{ \img \left[ \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q-1}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q}) \right] } $$
and
$$ H^0(\Omega; \mathcal S^p) =  \ker \left[ \dext' :\mathcal  C^\infty(\Omega; \Lambda^{p,0}) \to \mathcal  C^\infty(\Omega; \Lambda^{p,1}) \right]. $$

That is, $H^q(\Omega; \mathcal S^p)$ is isomorphic to $H^{0,q}_{\mathcal C^\infty}(\Omega; \mathcal V)$. We note that in this context, we also have that $\dext' : \mathcal E' (\Omega; \Lambda^{p,q}) \to \mathcal E' (\Omega; \Lambda^{p,q+1})$ has closed range. What we are going to do now is show that under certain conditions we have similar results in the context of hypocomplex structures. In order to do this, we need some technical results.

Let $\frk K$ be a cover of $\Omega$ satisfying the following properties:

\begin{itemize}
\item $\frk K$ is countable, with elements indexed as $\frk K = \{K_j\}_{j \in \N}$;
\item $\frk K$ is locally finite;
\item Each $K \in \frk K$ is a compact set of $\Omega$.
\end{itemize}

For $q \in \Z_+$, let $\sigma = (K_{j_0}, \ldots, K_{j_q})$ be a $q$-simplex of $\frk K$, that is, an ordered collection of $q+1$ sets of $\frk K$ such that $|\sigma| \doteq K_{j_0} \cap \ldots \cap K_{j_q} \neq \emptyset.$ Sometimes we will denote the simplex $\sigma$ just by the indexes, that is $\sigma = (j_0, \ldots, j_q)$.% The set $|\sigma|$ is called the \textit{support} of $\sigma$.

We denote by $N^q(\frk K)$ the set of all $q$-simplexes and by $N(\frk K) = \bigcup_{q \in \Z_+} N^q(\frk K)$ the nerv of $\frk K$. %We denote by $\mathcal F$ a sheaf over $\Omega$.
We recall that for each $q \in \Z_+$, a $q$-cochain of $N(\frk K)$ with values in $\mathcal S^p$ is a function $f$ such that to each $q$-simplex $\sigma$ it is associated a local section $f_\sigma \in \mathcal S^p(|\sigma|)$. We denote by $C^q(\frk K, \mathcal S^p)$ the set of all $q$-cochains with values in $\mathcal S^p$.

The coboundary operators $\delta^q : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)$, $q \in \Z_+$, are defined by
$$ (\delta^q f)_\sigma = \sum_{j=0}^{q+1}(-1)^j \rho^{|\sigma_j|}_{|\sigma|} f_{\sigma_j}$$
in which $\sigma_j \doteq (U_0, \ldots, \hat {U_j}, \ldots, U_{q+1} )$ and the mapping $\rho^{|\sigma_j|}_{|\sigma|}$ associates each $p$-form in $|\sigma_j|$ to its restriction to $|\sigma|$. By definition we have that $\delta^{q+1} \circ \delta^{q} = 0$ for all $q \in \Z_+.$

We define the cohomology of the complex $\delta^q : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)$, $q \in \Z_+$ as
$$ \check H^q(\frk K, \mathcal S^p) = \frac{ \ker \left[ \delta : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)\right] }{ \img \left[ \delta : C^{q-1}(\frk K, \mathcal S^p) \to C^{q}(\frk K, \mathcal S^p)\right] }$$
for $q \geq 1$ and for $q = 0$ we define $$\check H^0(\frk K, \mathcal S^p) = \ker \left[ \delta : C^0(\frk K, \mathcal S^p) \to C^{1}(\frk K, \mathcal S^p)\right] = \mathcal S^p(\Omega).$$ We just defined the \emph{\v Cech cohomology of $\frk K$ with values in $\mathcal S^p$}.

We denote by $\mathcal C^q_c(\frk K, \mathcal S^p)$ the set of all \emph{finite} $q$-cochains with values in $\mathcal S^p$, that is, for a given $f \in \mathcal C^q_c(\frk K, \mathcal S^p)$ there is only a finite number of $q$-simplexes of $\frk K$ such that $f_\sigma$ is non-zero. We clearly have $\delta^q( C^q_c(\frk K, \mathcal S^p) ) \subset C^{q+1}_c(\frk K, \mathcal S^p)$ for all $q \in \Z_+$, and so we have a complex whose cohomology will be denoted by $\check H^q_c(\frk K, \mathcal S^p)$ for all $q$. And now we have what we call \emph{\v Cech cohomology of $\frk K$ with values in $\mathcal S^p$ with compact support}.

We note that $C^q_c(\frk K; \mathcal S^p)$ is a closed subspace of a direct sum of DFS spaces and so it is also a DFS space. Moreover, since $\delta^q$ is a linear continuous map between DFS spaces each $\ker \delta^q$ is also a DFS space.


% \subsection{Application of \v Cech cohomology}

% \begin{dfn} Let $\{X_l, Z_l\}$ be a hypo-analytic structure over a connected smooth manifold $\Omega$. We denote by $\mathcal S$ the sheaf over $\Omega$ of distribution solutions to $d' u = 0$ and by $\mathcal A$ the subsheaf of $\Omega$ of hypoanalytic functions on $\Omega$.
% \end{dfn}

% \begin{dfn} The hypo-analytic structure is said to be hypocomplex in an open subset $Y \subset \Omega$ is the sheaf $\mathcal A$ and $\mathcal S$ agree over $Y$.
% \end{dfn}

% We denote by $\mathcal A^p$ the sheaf of germs of sections of u $\mathcal D'(U; \Lambda^{p,0})$ which satisfy $\dext'u = 0$.



% Let $\frk K = \{K_j\}_{j \in \N}$ be a locally finite and countable covering of $\Omega$ with $K_j$ compact for all $j \in \N$. % We are going to consider the cohomology spaces $C^q_c(\frk K; \mathcal S^p)$.

Let $A \subset \N$ be a finite subset. We denote by $C^q_A(\frk K; \mathcal S^p)$ the set of all cochains $s \in C^q_c(\frk K; \mathcal S^p)$ such that $s_{j_0 j_1 \ldots j_q} = 0$ if $\{j_0, j_1, \ldots, j_q\} \cap A = \emptyset.$

Since $\delta^q( C^q_A(\frk K; \mathcal S^p)) \subset C^{q+1}_A(\frk K; \mathcal S^p)$ we have a well defined \emph{complex of cochains with supports contained in $A$}. The corresponding cohomology spaces are denoted by $H^q_A(\frk K; \mathcal S^p)$ with $q = 0, 1, \ldots$. We have natural homomorphisms
$$ H^q_A(\frk K; \mathcal S^p) \to H^q_B(\frk K; \mathcal S^p) $$ if $A \subset B$ and clearly $$ H^q_A(\frk K; \mathcal S^p) \to H^q_c(\frk K; \mathcal S^p).$$

\begin{prp}
\label{hypo:aprime} Suppose that $\Omega$ is endowed with a involutive structure $\mathcal V$ satisfying the unique continuation property. For every finite subset $A$ of $\N$ there is another finite subset $A'$ of $\N$ with $A \subset A'$ such that the kernel of the homomorphism $H^1_A(\frk K; \mathcal S^p) \to H^1_c(\frk K; \mathcal S^p)$ is contained in the kernel of the homomorphism $H^1_A(\frk K; \mathcal S^p) \to H^1_{A'}(\frk K; \mathcal S^p)$.
\end{prp}

\begin{proof}
Let $L \subset \Omega$ be a compact such that $Y \doteq \Omega \bs L$ is connected and $\bigcup_{j \in A} K_j \subset L$. We define
$ A' = \{ j \in \N : K_j \cap L \neq \emptyset \}.$
Since $\frk K$ is locally finite we have that $A'$ is finite. We also have, by the choice of $L$, that $A \subset A'$.

Let $s \in C^1_A(\frk K; \mathcal S^p)$ be such that $\delta^1 u = s$ for some $u \in C^0_c(\frk K; \mathcal S^p)$.
We write $u = \{u_j\}$ with $u_j \in \mathcal S^p(K_j)$.
We have $u_j - u_k = s_{jk}$ as elements in $\mathcal S(K_j \cap K_k)$ if $K_j \cap K_k \neq \emptyset.$ Let $p \in Y$ and assume that $p \in K_j \cap K_k$. Notice that $\{j,k\} \cap A = \emptyset$  implies $s_{jk} = 0$ and consequently the germs of $u_j$ and $u_k$ coincide at $p$. By the unique continuation property, we have that there is $f \in \mathcal S^p(Y)$ such that the germs of $f$ and $u_j$ coincide at $p$ if $p \in K_j$. Since all but a finite number of the $u_j$'s are zero, it follows from the unique continuation that $f$ vanishes in an open neighborhood of $\del \Omega$ and thus in $Y$. In particular $u_j = 0$ if $K_j \subset Y$, that is $u_j =0$ if $j \notin A'$. % \todo[inline]{Is it here that it is necessary to assume that $\Omega$ is not compact?}
\end{proof}


\begin{prp}
\label{hypo:rho1_injective} Let $\frk L = \{L_j\}$ be a countable and locally finite refinement of $\frk K$ with each $L_j$ compact. Then the refinement homomorphism
$$ \rho^q : C^q_c(\frk K; \mathcal S^p) \to C^q_c(\frk L; \mathcal S^p), \qquad q = 0, 1, 2 \ldots $$
induces homomorphisms
$$ \rho^q_* : H^q_c(\frk K; \mathcal S^p) \to H^q_c(\frk L; \mathcal S^p), \qquad q = 0, 1, 2 \ldots $$
and $\rho^1_*$ is injective.
\end{prp}

% \begin{que} Can I prove that $\rho^q_*$ is injective for $q > 1$?
% \end{que}

\begin{proof}
Let $ \gamma : \N \to \N$ be such that $L_j \subset K_{\gamma(j)}$ for every $j$. Let $ s = \{s_{jk}\} \in C^1_c(\frk K; \mathcal S^p)$ satisfying $\delta^1 s = 0$ and suppose that $\rho^1 s = \delta^0 v$ for some $v = \{v_j\} \in C^0_c(\frk L; \mathcal S^p).$ Then
$ v_k - v_j = s_{\gamma(j) \gamma(k)}$
as elements of $ \mathcal S^p(L_j \cap L_k) $ and since $s$ is a cocycle we have that $s_{kr} - s_{jr} + s_{jk} = 0$ as elements of $\mathcal S^p(K_j \cap K_k \cap K_r)$ and consequently
$$ v_k + s_{\gamma(k)r} = v_j + s_{\gamma(j)r}$$
as elements of $\mathcal S^p(L_j \cap L_k \cap K_r)$. Notice that the left hand side does not depend on $j$ and the right hand side does not depend on $k$. By varying $j$ and $k$ we see that there is $u_r \in \mathcal S^p(K_r)$ such that $u_r = v_j + s_{\gamma(j)r}$ as elements of $\mathcal S^p(L_j \cap K_r)$ whenever $K_j \cap K_r \neq \emptyset.$

Let $I,J \subset \N$ be such that $v_j = 0$ unless $j \in I$ and $s_{jk} = 0$ unless $j$ and $k$ belong to $J$. The set $I' \doteq J \cup \left\{ r \in \N : \left( \bigcup_{j \in I} L_j \right) \cap K_r \neq \emptyset\right\}$
is finite and $u_r = 0$ if $r \notin I'$. Indeed, if $r \notin I'$ then $r \notin J$ and if $j$ is such that $L_j \cap K_r \neq \emptyset$ then $j \notin I$. These two facts imply $u_r = 0$ in $K_r \cap L_j $. Thus $u \doteq \{u_j\}$ belongs to $C^0_c(\frk K; \mathcal S^p)$. Finally, as elements of $\mathcal S^p(L_j \cap K_r \cap K_t)$ we have
$$ u_r - u_t = (v_j + s_{\gamma(j)r}) - (v_j + s_{\gamma(j)t}) = s_{\gamma(j)r} - s_{\gamma(j)t} = - s_{tr}.$$ And the proof is completed. \end{proof}

From now on we assume that $\frk K$ and $\frk L$ satisfy the following properties:

\begin{equation}
\label{hypo:p1} L_j \subset \operatorname{int}(K_j) \text{ for all } j \in \N.
\end{equation}
\begin{equation}
\label{hypo:p2}
\text{\parbox{.85\textwidth}{ If $(j_0, j_1)$ is a 1-simplex for $\frk K$ then it is also a 1-simplex for $\frk L$. And if $(j_0, j_1, j_2)$ is a 2-simplex for $\frk K$ then it is also 2-simplex for $\frk L$.}}
\end{equation}

For this it suffices to take $\frk L$ to be a locally finite countable covering of $\Omega$ such that each $K_j$ is compact and $\frk K = \{K_j\}$ is the covering defined by
$$ K_j = \{ p \in \Omega : \operatorname{dist}(p, L_j) \leq \epsilon_j\}.$$

It is clear that $\frk K$ also is locally finite and countable and that each $K_j$ is compact if $\epsilon_j > 0$ is chosen suitable small.


% In order to prove this result we need some intermediate results.

% We are going to assume that $\Omega$ is not compact.



Notice that property \eqref{hypo:p2} above guarantees that the maps $\rho^p$ are injective for $p = 0, 1, 2$. Moreover, if $A \subset \N$ is finite, then $A$ induces homomorphisms
$$ \rho^p_A : C^p_A(\frk K; \mathcal S^p) \to C^p_A(\frk L; \mathcal S^p)$$
which are now, thanks to property \eqref{hypo:p1}, compact operators.



\begin{thm}
\label{hypo:thm:dfstop} Assume that $\Omega$ is endowed with a hypocomplex structure. The map $\delta^0 : C^0_c(\frk K; \mathcal S^p) \to C^1_c(\frk K; \mathcal S^p) $ has closed range. % and thus $H^1_c(\frk K, \mathcal S^p)$ has a natural topology of DFS spaces.
\end{thm}

\begin{proof} By Theorem 6' of \cite{komatsu1967projective}, it suffices to show that $\img(\delta^0) \cap C^1_A(\frk K; \mathcal S^p)$ is closed in $C^1_A(\frk K; \mathcal S^p)$ for all finite subsets $A \subset \N.$

Let $A \subset \N$ be finite and let $A'$ be as in Proposition \ref{hypo:aprime}. We define the following DFS spaces:
$$ V \doteq \{ (u,s) \in C^0_{A'}(\frk K; \mathcal S^p) \times C^1_{A}(\frk K; \mathcal S^p): \delta^0 u = s\},$$
$$ W \doteq \{ (u,s) \in C^0_{A'}(\frk L; \mathcal S^p) \times C^1_{A}(\frk K; \mathcal S^p): \delta^0 u = \rho^1s\},$$
and let $\sigma : V \to W$ be the linear map given by $ \sigma(u, s) = (\rho^0_{A'}u, s).$

We need the following lemma:

\begin{lem}  Assume that $\Omega$ is endowed with a hypocomplex structure. The map $\sigma$ is a bijection.
\end{lem}
\begin{proof}
Since $\delta^0$ is injective we have that $\sigma$ is injective. In fact, if $\sigma(u,s) = (0,0)$ then $s = 0$ and since $(u,s) \in V$ we have $\delta^0u = 0$.

Now we are going to prove that $\sigma$ is surjective. Let $(v,s) \in W$. We have that $\delta^1(\rho^1 s) = \delta^1(\delta^0 v) = 0$ and since $\rho^2(\delta^1 s) = \delta^1(\rho^1 s) = 0 $ and $\rho^2$ is injective if follows that $\delta^1 s = 0$. Hence the class of $s$ defines an element in $H^1_A(\frk K; \mathcal S^p)$ which belongs to the kernel of $\rho^1_*$. By Proposition \ref{hypo:rho1_injective} the class of $s$ vanishes in $H^1_c(\frk K; \mathcal S^p)$ and so Proposition \ref{hypo:aprime} implies that the class of $s$ vanishes in $H^1_{A'}(\frk K; \mathcal S^p)$. In other words, there is $u \in C^1_{A'}(\frk K; \mathcal S^p)$ such that $(u,s) \in V$. To complete the proof we need to show that $\sigma(u,s) = (v,s)$ and this follows from $\delta^0(v - \rho^0_{A'}u) = 0$ and the fact that $\delta^0$ is injective.
\end{proof}
We denote by $E$ the DFS space $C^0_{A'}(\frk L; \mathcal S^p) \times C^1_A(\frk K; \mathcal S^p)$; we remark that $W$ is a closed subspace of $E$ and thus also a DFS space. Let $\imath$ be the inclusion map $W \subset E$. It follows that $\imath \circ \sigma : V \to E$ is a topological embedding.

We introduce the following continuous linear maps
 $$ \tau_1(u,s) = (\rho^0_{A'}, 0), \qquad \tau_2(u,s) = (0,s).$$

Since $\tau_1$ is compact and $\tau_2 = \imath \circ \sigma - \tau_1$ it follows from Theorem 1 of \cite{schwartz1956} that $\tau_2$ has closed range in $E$. This is the same as saying that the map $p_2 : V \to C^1_A(\frk K; \mathcal S^p)$ given by the projection on the second factor has closed range, but according to Proposition \ref{hypo:aprime} we have
$$ \img{p_2} = \img(\delta^2) \cap C^1_A(\frk K; \mathcal S^p),$$
which completes the proof.
\end{proof}


% The most important technical result is the following one.

%\begin{thm}
%\label{hypo:thm:dfs} If $\Omega$ is a hypocomplex manifold then $H^1_c(\Omega; \mathcal S^p)$ has a natural topology of DFS space.
%\end{thm}

%\begin{proof}
% [Proof of Theorem \ref{hypo:thm:dfs}]
%We select two sequences $\frk L^r = \{L^r_j\}$ and $\frk K^r = \{K^r_j\}$ all being locally finite, countable with compact elements satisfying the following properties:

%\begin{enumerate}
%\item $L^r_j \subset int(K^r_j)$ for all $r, j \in \N$;
%\item If $r \in \N$ and if $(j_0, j_1)$ (resp. $(j_0, j_1, j_2)$) is a 1-simplex (resp. 2-simplex) for $\frk K^r$ it is also a 1-simplex (resp. 2-simplex) for $\frk L^r$;
%\item $\frk K^{r+1}$ is a refinement of $\frk K^r$ for all $r \in \N$;
%\item Given $D \subset \Omega$ open and $p_0 \in D$ there are $r_0 \in \N$ and a sequence $\{j_r\}_{r \geq r_0}$ such that $p_0 \in K^r_{jr} \subset D$ for all $r \geq r_0$.
%\end{enumerate}

%According to properties 1 and 2 above and due to Proposition \ref{hypo:prp:dfstop} it follows that each cohomology space $H^1_c(\frk K^r; \mathcal S^p)$ is a DFS space. Moreover, the natural homomorphisms
%$$ H^1_c(\frk K^r; \mathcal S^p) \to H^1_c(\frk K^{r+1}; \mathcal S^p)$$
%defined via the ``refinement mappings'' are continuous and in fact injective. Finally, by property 4 we have that the natural homomorphisms
%$$ \varinjlim H^1_c(\frk K^r; \mathcal S^p) \to H^1_c(\Omega; \mathcal S^p)$$
%is an isomorphism. Hence $H^1_c(\Omega;\mathcal S^p)$ has a natural topology of a DFS space. The proof is complete.

%\end{proof}

%Let $\mathcal F$ be the sheaves $\mathcal C^\infty$ or $\mathcal D'$ and we consider the complexes of sheaves
%$$ \dext' : \mathcal F(\Lambda^{p,q}) \to \mathcal F(\Lambda^{p,q+1}).$$

%whose cohomologies will be denoted by $\mathcal H^{p,q}(\mathcal F)$. In particular,
%$$ \mathcal H^{p,0}(\mathcal F) = \ker \left( \dext' :  \mathcal F(\Lambda^{p,0}) \to \mathcal F(\Lambda^{p,1}) \right) = \mathcal S^p.$$

%For each pair $p,q$, the sheaf $\mathcal F(\Lambda^{p,q})$ is a fine sheaf. Therefore, by applying Theorem 4.6.1 of \cite{godement1958topologie} there is a spectral sequence with
%$$ E^{r,s}_2 = H^r_\Phi(\Omega, \mathcal H^{p,r}(\mathcal F)) \implies H^{r+s}(\mathcal F_\Phi(\Omega; \Lambda^{p,*})).$$

%Here $\Phi$ is any family of supports of $\Omega$. Taking $\Phi$ as the family of all compact subsets if $\Omega$, that is $\Phi = c$, we obtain an exact sequence

%$$ 0 \to H^1_c(\Omega; \mathcal S^p) \to H^1(\mathcal F_c(\Omega;\Lambda^{p,*})) \to H^0_c(\Omega; \mathcal H^{p,1}(\mathcal F)).$$




%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RAGOGNETE'S THEOREM %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{prp}
\label{hypo:prp:equiv} Let $\Omega$ be endowed with a hypocomplex structure $\mathcal V$ and let $x \in \Omega$. The following properties are equivalent:
\begin{enumerate}
\item \label{hypo:prp:equiv1} $ \mathcal H^{0,1}_{\mathcal C^\infty} (\{x\}, \mathcal V) = 0$;
\item \label{hypo:prp:equiv2} $ \mathcal H^{0,1}_{\mathcal D'} (\{x\}, \mathcal V)= 0$;
\item $ \mathcal H^{p,1}_{\mathcal C^\infty} (\{x\}, \mathcal V) = 0$ for all $p = 0, 1, 2, \ldots$;
\item $ \mathcal H^{p,1}_{\mathcal D'} (\{x\}, \mathcal V)= 0$ for all $p = 0, 1, 2, \ldots$.
\end{enumerate}
\end{prp}

The proof of this result can be found in \cite{luis2018ultradifferential}.

%\begin{proof} We will prove only that \eqref{hypo:prp:equiv1} implies \eqref{hypo:prp:equiv2}. Let $\omega \subset \Omega$ be an open neighborhood of $x$. We define $Z$
%\end{proof}

\begin{thm}
\label{thm:closed_range} Let $\Omega$ be endowed with a hypocomplex structure $\mathcal V$. Assume that the equivalent conditions in Proposition \ref{hypo:prp:equiv} hold for every point of $\Omega$. Then % for each $p = 0, 1, \ldots, m$ the natural homomorphism
%$$ \alpha : H^1_c(\Omega; \mathcal S^p) \to H^{1}(\mathcal E'(\Omega; \Lambda^{p,*}))$$
%is an isomorphism and consequently
\begin{equation}
\label{hypo:eq:dprimecpctsupp} \dext' : \mathcal E' (\Omega; \Lambda^{p,0}) \to \mathcal E' (\Omega; \Lambda^{p,1})
\end{equation}
has closed range.
\end{thm}

For the proof we need to use Sobolev spaces and some technical results. For a coordinated open set $U \subset \Omega$, we denote by $W^{l,2}(U; \Lambda^{p,q})$ the Sobolev space over $U$ of order $l \in \Z$ and by $\|\cdot\|_{W^{l,2}(U)}$ its norm. Notice that $$\{u \in W^{-l,2}(U; \Lambda^{p,0}); \dext' u = 0\} \subset L^2_{loc}(U)$$ and this inclusion is continuous due to the closed graph theorem. It follows that if $K \subset U$ is compact, there exist a constant such that $\|u\|_{L^2(K)} \leq C\|u\|_{W^{-l,2}}$ and so the topology induced by the norms $C\|\cdot\|_{W^{-l,2}}$ is equivalent to the topology induced by $\|\cdot\|_{L^2(K)}$.

%Notice that if $u \in S^p(U)$ and $\|u\|_{W^{-l,2}(U)}$ for some integer $l \geq 0$ then $u = 0$. In fact, by Cauchy estimates, for any compact $K \subset U$ we have $$ \sup_K |M^\alpha v| \leq C_\alpha \|v\|_{L^2(U)} $$ for $v \in S^p(U)$ and so, by writing $\Delta_M = \sum_{j=0}^m M_j^2 $ we have $$ \sup_K |(I - \Delta_M)^p v| \leq C_p \|v\|_{L^2(U)}. $$ Therefore, by taking $u = (I - \Delta_M)^p v$ we obtain
%$$ \sup_K |u| \leq C_p \|(I - \Delta_M)^p u\|_{L^2(U)} = C_p \|u\|_{ W^{-2p,2}(U) }.$$ More details can be found in \cite{treves1992hypo}.

\begin{lem}
Let $\Omega$ be endowed with a hypocomplex structure $\mathcal V$. Assume that the equivalent conditions in Proposition \ref{hypo:prp:equiv} hold for a point $x \in \Omega$. Then for every open neighborhood $\omega \subset \Omega$ of $x$ and for every integer $M \in \Z_+$ we can find another open neighborhood $\omega' \subset \Omega$ of $x$ such that for any $ f \in \mathcal E'(\omega; \Lambda^{p,1}) \cap W^{-M,2}(\omega; \Lambda^{p,1})$ satisfying $\dext' f = 0$ on $\omega$ there exists an integer $L$, not depending on $f$, and $u \in \mathcal E'(\omega; \Lambda^{p,0}) \cap W^{-L,2}(\omega; \Lambda^{p,0})$ such that $\dext' u = f$ on $\omega'$.
\end{lem}

\begin{proof}

Let $\{U_l\}$ be a sequence of decreasing open neighborhoods of $x$ satisfying: $U_{l+1} \ssubset U_l$ and $\bigcap_l U_l = \{x\}$.
We write $$ Z_c^{p,1}(\omega) = \{ u \in \mathcal E'(\omega; \Lambda^{p,1}) : \dext' u = 0\}$$ and we define
$$ G_l = \{ (u, f) \in W^{-l,2}(U_l; \Lambda^{p,0}) \times Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1}) : \dext' u = f \}.$$

Notice that each $G_l$ is a closed subspace of $W^{-l,2}(U^l; \Lambda^{p,0}) \times  W^{-M,2}(\omega; \Lambda^{p,1})$ and so it is a Banach space. Notice that the projection $\pi_l : G_l \to Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1})$ is linear and continuous. Since we are assuming local solvability at $x$ we have $$ Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1}) = \bigcup_{l \in \Z} \pi_l (G_l).$$

By the Baire's category theorem, one of the spaces $\pi_l (G_l)$ must be of second category. Assume that $\pi_{l_0} (G_{l_0})$ is of second category. By the Banach open mapping theorem, the map $\pi_{l_0}: G_{l_0} \to Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1})$ must be surjective and open. The proof is finished by taking $\omega' = U_{l_0+1}$ and $L = l$.

\end{proof}

\begin{cor}
With the same assumptions and notations of the previous lemma we have that
% given a compact $K \subset \omega'$,
there exists a constant $C > 0$ such that for any $ f \in \mathcal E'(\omega; \Lambda^{p,1}) \cap W^{-M,2}(\omega; \Lambda^{p,1})$ satisfying $\dext' f = 0$ on $\omega$ there exist an integer $L$, not depending on $f$, and $u \in \mathcal E'(\omega; \Lambda^{p,0}) \cap W^{-L,2}(\omega; \Lambda^{p,0})$ such that $\dext' u = f$ on $\omega'$ having the following estimative
$$ \|u\|_{ W^{-L,2}(\omega') } \leq C \|f\|_{W^{-M,2}(\omega)}.$$
\end{cor}

\begin{proof}

By using the same notation from the previous proof, the map  $$\pi_{L}: G_{L} \to Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1})$$ is surjective and open.

Now
$$ U = \{(u, f) \in G_{L} : \|u\|_{ W^{-L,2}(U^l) } < 1\}$$
is an open neighborhood of the origin in $G_{L}$. Therefore $\pi_{L}(U)$ contains an open neighborhood $W$ of the origin in $Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1})$. Decreasing $W$ if necessary, we assume that $$ W = \{ f \in Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1}) : \|f\|_{W^{-M,2}(\omega)} < \epsilon \}$$
for some $\epsilon > 0$.

Let $f \in  Z^{p,1}_c(\omega) \cap W^{-M,2}(\omega; \Lambda^{p,1})$ and assume that $\|f\|_{ W^{-L,2}(\omega) } > 0$. We have $$(\epsilon/2)f/\|f\|_{W^{-M,2}(\omega)} \in W$$ and so we can find $w \in W^{-L,2}(\omega'; \Lambda^{p,0})$ such that $$(w, (\epsilon/2)f/\|f\|_{ W^{-L,2}(\Omega) }) \in U.$$ By setting $u = (2/\epsilon)\|f\|_{ W^{-L,2}(\omega) } w$ we have that $\dext' u = f$ on $\omega'$ and
$$ \|u\|_{ W^{-L,2}(\omega') } \leq \frac{2}{\epsilon} \|f\|_{W^{-M,2}(\omega)}.$$

If $f = 0$ in $\omega$ we take $u = 0$ and clearly

$$ \|u\|_{W^{-L,2}(\omega')} \leq \frac{2}{\epsilon} \|f\|_{W^{-M,2}(\omega) }.$$

The proof is complete by taking $C = 2/\epsilon$.
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:closed_range}]

Let $f^j \in \dext'(\mathcal E'(\omega; \Lambda^{p,0}))$ be a sequence of functions converging to $f \in \mathcal E'(\omega; \Lambda^{p,1})$. We write $u^j \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u^j = f^j$. We want to show that there exist $u \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u = f$.

Now we are going to construct a special covering for $\Omega$. Let $M$ be such that $f \in W^{-M,2}(\omega; \Lambda^{p,1})$. By following the same notation from the previous lemma, for each $x \in \Omega$ there exist a compact set $K(x) = \overline{U_{l_x + 1}(x)} \subset \omega'(x) \subset \omega(x)$ for every $w \in  Z^{p,1}_c(\omega(x)) \cap W^{-M,2}(\omega(x); \Lambda^{p,1})$ there exist a $u \in  \mathcal D'(\omega'(x); \Lambda^{p,0}) \cap W^{-l_x,2}(\omega'(x); \Lambda^{p,0})$ satisfying $$\dext' u = w$$ on $\omega'(x)$ and satisfying $$ \|u\|_{W^{-l_x,2}(\omega'(x))} \leq C(x) \|w\|_{W^{-M,2}(\omega(x))}.$$

Therefore, we have a covering $\frk U' = \{K(x)\}$ of $\Omega$ by compacts. We take a subcover $\frk U$ of $\frk U'$ being locally finite and countable. The elements of $\frk U$ will be denoted by $\frk U = \{K(x_j)\}$. We simplify the notation by writing $K_j = K(x_j)$, $\omega'_j = \omega'(x_j)$ and $\omega_j = \omega(x_j)$ and $C_j = C(x_j)$. Let $K$ be a compact such that $\operatorname{supp} f^j \in K$ for all $j$. Notice that only a finite number of elements of $\frk U$ intercept $K$ and so we take  $C = \max \{C_j: K_j \cap K \neq \emptyset \}$ and $L = \max \{l_{x_j} : K_j \cap K \neq \emptyset \}$.


% The space
% $$ Z_c^{p,1}(\Omega) = \{ u \in \mathcal E'(\Omega; \Lambda^{p,1}) : \dext' u = 0\}$$
% is a DFS space. Consider the map between DFS spaces
% $$ \theta : Z^{p,1}(\Omega) \xrightarrow{\pi} H^{p,1}(\Omega; \mathcal E') \xrightarrow{\alpha^{-1}} H^1_c(\Omega; \mathcal S^p),$$
%in which $\pi$ denotes the projection map over the quotient of $Z_c^{p,1}(\Omega)$ by the image of \eqref{hypo:eq:dprimecpctsupp}. We need to show that $\theta$ is continuous.


% In this context, the map $\theta$ has a very explicit expression. Let $f \in Z^ {p,1}_c(\Omega)$ and let $\mathfrak U$ be a covering of $\Omega$ by compacts. Assume that this covering is such that we have $H^{p,1}(U; \mathcal D') = 0$.

For each $k$ there exist $v^j_k \in \mathcal D'(\omega'_k; \Lambda^{p,0})$ such that $\dext' v^j_k = f^j|_{\omega_k}$ on $\omega'_k$ and satisfying the estimates
\begin{equation}
\label{hypo:ineq_sol}
 \| v^j_k \|_{W^{-L,2}(\omega'_k)} \leq C \|f^j\|_{W^{-M,2}(\omega_k)}.
\end{equation}

We take $v^j_k = 0$ if $f^j|_{\omega_k} = 0$.

If $k , l$ are such that $K_k \cap K_l \neq \emptyset$, then $\dext' [v^j_k - v^j_l] = 0$ in $K_k \cap K_l$ which means that $v^j_k - v^j_l \in \mathcal S^p(K_k \cap K_l)$. Therefore, it is defined a 1-cochain $g^j \in C^1(\mathfrak U; \mathcal S^p)$ such that for each 1-simplex $\sigma = (K_k, K_l)$, we have $g^j_\sigma = (v^j_k - v^j_l) $. % Notice that if $\sigma = (K_k, K_l, K_o)$ is a 2-simplex, we have $$(\delta^1 g)_\sigma = \sum_{j=0}^1 (-1)^j \rho^{|\sigma_j|}_{|\sigma|} g_{|\sigma_j|} = (g_{K_k} - g_{K_l}) - (g_{K_l} - g_{K_o}) + (g_{K_l} - g_{K_o}) = 0.$$

Notice that if we define $h^j_k = v^j_k - u^j$ then $h^j_k$ is in $\mathcal S^p(K_k)$ and then we have a 0-cochain $h^j \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$.

Since $f^j$ is convergent, and therefore a Cauchy sequence, by the inequality $\eqref{hypo:ineq_sol}$ the sequence $\{v^j_k\}$ also is a Cauchy sequence and so it converges to a function $v_{k}$ in $\mathcal S^p(K_k \cap K_l$ and so $g^j$ converge to a 1-cochain $g \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$. By Theorem \ref{hypo:thm:dfstop}, $\delta^0$ has closed range, and so there exist a 0-cochain $h \in C^0_c(\frk U; \mathcal S^p)$ such that $\delta^0(h) = g$. This means that $h_k - h_l = v_k - v_l$ in $K_k \cap K_l$. This mean that $v_k - h_k = v_l - h_l$ and so we can define $u \in \mathcal E'(\omega; \Lambda^{p,0})$ given by $u = v_k - h_k$ in $K_k$ for each $k$. Since $\dext' v^j_k = f^j$ for all $j$ we have $\dext' v_j = f$ and we also have $\dext' h_k = 0$ this means that $\dext' u = f$ in $K_k$ for every $k$.
\end{proof}

%Now suppose that if we have a different choice for solutions $\dext' u'_U = f|_U$ on $U$ then for each 1-simplex $\sigma = (U_0, U_1)$ $$(g - g')_\sigma = (u_j - u_k) - (u'_j - u'_k) = (u_j - u'_j) - (u_k - u_k') = (\delta^0 h)_\sigma $$ which $h_{U} = u_U - u'_U$, that is, $(g - g')$ is exact and so $g$ defines an element in $\check H(\mathfrak K; \mathcal S^p)$. Notice that, if $\mathfrak U'$ is another covering for $\Omega$ such that $H^{p,1}(U; \mathcal D') = 0$ for all $U \in \mathfrak U'$ and we construct $g'$ using this covering, we can consider a refinement $\mathfrak U''$ of $\mathfrak U$ and $\mathfrak U'$ and we easily see that $g - g'$ is exact on $C^1(\mathfrak U''; \mathcal S^p)$.

%Now we are going to construct a special covering for $\Omega$.
%We take $\mathcal U = \{ K(x) = \overline{U_{l_0 + 1}} : x \in \Omega \}$. This is a covering for $\Omega$ by compacts such that for each $K \in \mathcal U$ there exist an open neighborhood $U$ of $K$ in which $H^{p,1}(U; \mathcal D') = 0$ and such that, for every $f \in  Z^{p,q}_c(\Omega) \cap W^{-M,2}(\Omega; \Lambda^{p,1})$ there exist a $u \in  \mathcal D'(\Omega; \Lambda^{p,q}) \cap W^{-l_U,2}(\Omega; \Lambda^{p,0})$ satisfying $$ \|u\|_{W^{-l_U,2}(U)} \leq C_U \|f\|_{W^{-M,2}(\Omega)}.$$


%By taking a refinement of the covering, we can assume that $\mathcal U$ is locally finite and so, for a given $f \in W^{-M,2}(\Omega; \Lambda^{p,1})$ only a finite number of compacts $K$ of $\mathcal U$ intercepts the support of $f$. And, for each $K \in \mathfrak U$, by taking the corresponding covering $U$ of $K$ we have that the solution $u_{U} \in \mathcal D'(U; \Lambda^{p,0})$ of $\dext' u_U = f|_U$ belongs to $W^{-{L_U,2}}(U; \Lambda^{p,0})$ for some $L_U \in \Z_+$. % Let $L = \min \{L_j\}$. We have that $u_{U_j} \in H^{-L}(U_j; \Lambda^{p,0})$.
%We also assume that $u_U = 0$ if $U$ does not intercept the support of $f$.

%The topology of $C^1(\mathfrak U; \mathcal S^p)$ is given by the identification $$ C^1(\mathfrak U; \mathcal S^p) = \prod_{K \in U} \mathcal S^p(K)$$ with the latter endowed with the product topology. Now, take a sequence $\{f_j\} \subset Z^{p,1}_c(\Omega)$ converging to $0$. There exist a compact $K$ such that the support of all $f_j$ are contained in $K$. There exist a finite number of compacts from $\mathfrak U$ intercepting $K$, namely, $K_1, \ldots, K_k$ and we denote the corresponding open neighborhoods by $U_1, \ldots, U_k$ so
%$$ \sum_{j = 1}^k \|  u_K^j \|_{ W^{-L_K,2}(U_j) } \leq C_K \| f_j \|_{W^{-M,2}(\Omega)}.$$

%Therefore $\|  u_K^j \|_{ W^{-L_K,2}(\Omega) } \to 0$ when $j \to \infty$. Then $\theta$ is continuous. Since $H^1_c(\Omega;\mathcal S^p)$ is Hausdorff, the kernel of $\theta$ is closed in $Z^{p,1}_c(\Omega)$. Since $\alpha$ is an algebraic isomorphism it follows that this kernel is the image of \eqref{hypo:eq:dprimecpctsupp} which completes the proof.

\begin{cor} Let $\Omega$ be a non-compact manifold endowed with a hypocomplex structure $\mathcal V$. If one of the equivalent conditions in Proposition \ref{hypo:prp:equiv} hold then
$$   H^{p,n}_{\mathcal C^\infty}(\Omega) = 0,\qquad p = 0, 1, 2, \ldots$$
\end{cor}

\begin{proof} This property is equivalent to the surjectivity of the map
$$ \dext' : \mathcal C^\infty (\Omega; \Lambda^{p,n-1}) \to \mathcal C^\infty (\Omega; \Lambda^{p,n}) $$
its transpose is the map
$$ \dext' : \mathcal E' (\Omega; \Lambda^{m-p,0}) \to \mathcal E' (\Omega; \Lambda^{m-p,1}) $$
which is injective because $\mathcal V$ is hypocomplex and weakly closed thanks to Proposition \ref{hypo:prp:equiv}. The result is then a consequence of the homomorphism theorem for Fréchet-Montel spaces.
\end{proof}

\begin{cor} Let $\Omega$ be a compact manifold endowed with a hypocomplex structure $\mathcal V$. If one of the equivalent conditions in Proposition \ref{hypo:prp:equiv} hold then,
$$ \dim H^{p,n}_{\mathcal C^\infty}(\Omega) < \infty,\qquad p = 0, 1, 2, \ldots$$
\end{cor}

\begin{proof}
Since $\Omega$ is compact, it follows that $$\dim H^{p,0}_{\mathcal C^\infty}(\Omega) < \infty,\qquad p = 0, 1, 2, \ldots$$
The result is then a consequence of the homomorphism theorem for Fréchet-Montel spaces.
\end{proof}


The following is probably the simplest example of hypocomplex structure.

\begin{exa}
Let $\Omega \subset \R^2$ be an open neighborhood of the origin with coordinates $(s,t)$. Let $b : \Omega \to \R$ be a smooth function such that $b \geq 0$ and such that $b$ is not identically zero in any neighborhood of $s = 0$. In this case, the structure $\mathcal V$ spanned by the smooth vector field $L = \del_s + ib(s,t)\del_t$ is hypocomplex and the equivalent properties of Proposition \ref{hypo:prp:equiv} are valid at every point of $\Omega$. The proof of this fact can be found in \cite{treves1992hypo} Lemma III.6.2.
\end{exa}


In a sense, the example above is the ``only'' possible example at dimension 2. Now we make this statement precise: let $\Omega$ be a 2-dimensional manifold endowed with a hypocomplex structure $\mathcal V$. By Theorem III.6.2 \cite{treves1992hypo}, for each point $x \in \Omega$ there exist a smooth section $L$ of $\mathcal V$ in a neighborhood of $x$ and coordinates $(s,t)$ such that $L = \del_s + ib(s,t)\del_t$ in which $b$ is a smooth function satisfying $b(s,t) \geq 0$ near $x$ and such that $b(s,0)$ is not identically zero in any neighborhood of $s = 0$. In this case, the equivalent properties of Proposition \ref{hypo:prp:equiv} are valid at every point $x \in \Omega$.


The following example is a particular case of Example 2 from \cite{andreotti1981absence}. It shows that there are structures in which none of the equivalent properties of Proposition \ref{hypo:prp:equiv} hold.

\begin{exa}
In $\C^4$ we consider the coordinates $z \in \C$, $u \in \C$ and $w = (t_1 + i s_1, t_2 + i s_2) \in \C^2$ and consider the submanifold $\Omega \subset \C^4$ defined by the equations
$$
\left\{ \begin{aligned}
s_1 & = z \overline{z} - u \overline{u}; \\
s_2 & = z\overline{u} + u\overline{z}.
\end{aligned} \right.
$$
In this example, we can easily see that the signature of the Levi form is (1,1) at every point. Therefore this structure is hypocomplex, but by Theorem 3 of \cite{andreotti1981absence}, none of the equivalent properties of Proposition \ref{hypo:prp:equiv} hold.

\end{exa}

Using the same technique above we can prove a more general result. Basically, we needed to combine two results to prove global solvability at top degree was the vanishing. The first one was the vanishing of the cohomology $H^{p,1}_{\mathcal D'}(\Omega; \mathcal V)$, which in the case of hypocomplex structures follows from the unique continuation property. There are more examples structures having the unique continuation property. Consider, for example, the following definition.

\begin{dfn}
The structure $\mathcal V$ is said to be of \emph{finite type} if given any point $p \in \Omega$ the algebra spanned by $\{\Re L : L \text{ is a local section of } \mathcal V \text{ at p}\}$, when restricted to $p$, equals $T_p\Omega.$
\end{dfn}

If $\mathcal V$ is of finite type, the orbits of $\mathcal V$ in $\Omega$ are the connected components of $\Omega$ \cite{treves1992hypo} and thus, due to Theorem III.3.3 of \cite{treves1992hypo} it follows that every locally integrable structure of finite type posses the unique continuation property.

\begin{prp}
Let $\Omega$ be a non-compact connected manifold and suppose that $\mathcal V$ is a locally integrable structure over $\Omega$ having the unique continuation property. Then the kernel of the map
$$ \dext' : \mathcal E'(\Omega; \Lambda^{p,0}) \to \mathcal E'(\Omega; \Lambda^{p,1})$$
is trivial.
\end{prp}

\begin{thm}
\label{chp:inv:thm:stronger}
Suppose that $\Omega$ is a connected non-compact manifold and let $\mathcal V$ be a integrable involutive structure over $\Omega$ having the unique continuation property. If given any compact $K \subset \Omega$ and $s \in R$ there is $t \in \R$ such that if $u \in \mathcal E'(\Omega; \Lambda^{p,0})$ and $\dext' u \in H^{s}(\Omega; \Lambda^{p,1})$ then $u \in H^{t}(K; \Lambda^{p,0})$. Then $H^{p,n}_{\mathcal C^\infty}(\Omega; \mathcal V) = \{0\}$.
\end{thm}

\begin{cor}
Suppose that $\Omega$ is a non-compact connected component and that $\mathcal V$ is elliptic. Then $H^{p,n}_{\mathcal C^\infty}(\Omega; \mathcal V) = \{0\}$.
\end{cor}

\begin{cor}
Suppose that $\Omega$ is a connected non-compact manifold endowed with a locally integrable CR structure $\mathcal V$ of codimension $d > 0$ satisfying the following property: the levi form of $\mathcal V$ each each point $\xi \in \mathcal V^\perp_0$ has at least one negative eigenvalue. Then $H^{p,n}(\Omega; \mathcal V) = 0$.
\end{cor}

\begin{proof}
The property about the eigenvalues of the Levi form implies that the structure is hypocomplex. This is an application of Corollary 6.1 of \cite{baouendi1983microlocal}. Moreover, by Theorem 1 of \cite{shaw2005holder}, given $x \in \Omega$ and $s \in \R$ the following holds: if $u \in \mathcal D'(\Omega; \Lambda^{p,0})$ and $\dext' u \in \in H^{s}_{loc}(V_x; \Lambda^{p,1})$, in which $V_x$ is a neighborhood of x, then $\in H^{s+1/2}_{loc}(V'_x; \Lambda^{p,0})$. The conclusion follows from Theorem \ref{chp:inv:thm:stronger}.
\end{proof}

\begin{exa} Let $M$ be an real-analytic connected and oriented manifold of dimension $n \geq 1$ and let $\Omega \doteq \R \times M$. Given a real-analytic function $\Phi : M \to \R$ we consider the involutive structure $\mathcal V$ on $\Omega$ whose ortogonal $\mathcal V^\perp$ is spanned by the differential of the function $ Z : \Omega \to \C$ given by the rule $Z(x,t) = x + i \Phi(t)$ with $x \in \R$ and $t \in M$. Notice that if $t_1, \ldots, t_k$ are local coordinates on an open subset $U \subset \Omega$ then $\mathcal V$ is spanned over $R \times U$ by the vector fields
$$ L_j = \frac{\del}{\del t_j} - i \frac{\del \Phi}{\del t_j}(t) \frac{\del}{\del x}, \qquad j = 1, 2, \ldots, n. $$
According to Corollary III.5.3 of \cite{treves1992hypo}, the structure $\mathcal V$ is hypocomplex and since $\Phi$ is open we have that $\Omega$ is not compact. Moreover, from \cite{journe2006hypoellipticite} the following holds: Given $(x_0, t_0) \in \Omega$, if $u \in \mathcal D'(\Omega; \Lambda^{p,0})$ and $\dext' u \in H^s_{loc}(V_{(x_0, t_0)}; \Lambda^{p,1})$, in which $V_{(x_0, t_0)}$ is an open neighborhood of $(x_0, t_0)$, then $u \in H^s_{loc}(V'_{(x_0, t_0)}; \Lambda^{p,0})$, in which $V'_{(x_0, t_0)}$ is an open neighborhood of $(x_0, t_0)$. Again, from Theorem \ref{chp:inv:thm:stronger}, we have that $H^{p,n}_{\mathcal C^\infty}(\Omega; \mathcal V) = \{0\}$.
\end{exa}


==> chp-involutive-structures.tex <==




\chapter{Involutive structures}
\label{chp:involutive_structures}

In this chapter, we introduce the basic definitions regarding involutive structures along with some tools to study them. The main concepts introduced here are the concept of involutive structure, the associated differential operators, and their cohomology spaces, which are the main objects of study in this work.


\section{Preliminaries on functional analysis}

As pointed out before, we apply a suitable characterization of the homomorphisms with dense image defined between Fr\'echet-Schwartz spaces.
The advantage of this class relies on the fact that the strong dual of a Fr\'echet-Schwartz space is an inductive limit of a sequence of Banach spaces
with compact inclusions. The proof of the homomorphim theorem makes use of its well known version valid for the class of the Fr\'echet-Montel spaces, whose proof can be found in  \cite[Section 33]{kothe19679topological}:

\begin{thm}\label{thm:FM}
 Let $E$, $F$ be Fr\'echet-Montel spaces and let
$A:E\sra F$ be a continuous linear map with $A(E)$ dense in $F$. The following properties are equivalent:
\begin{enumerate}
\item $A$ is a homomorphism;
\item $A(E)=F$;
\item $\AT$ is a strong homomorphism;
\item $\forall {\cal{B}} \subset F'$,  $\AT({\cal{B}})\subset E'$  strongly bounded $\Rightarrow$ ${\cal{B}}$ strongly bounded;
\end{enumerate}\end{thm}

A particular class of Fr\'echet-Montel spaces is the class of the so-called Fr\'echet-Schwartz ({\bf FS}) spaces (cf. \cite{komatsu1967projective}).
When $E$ is a ({\bf FS}) space its strong dual is an inductive limit of a sequence of Banach spaces
$E'=\mbox{ind}\,( E'_p)$,
where, for each $p\in\N$, $E'_p$ is a subspace of $E'_{p+1}$, the injection map being compact.

\begin{thm}\label{thm:FS}
Let $E$, $F$ be Fr\'echet-Schwartz spaces and let
$A:E\sra F$ be a continuous linear map with dense image. Write the corresponding strong duals as inductive limits of Banach spaces
$E'=\mbox{ind}\,( E'_p)$, $F'=\mbox{ind}\,( F'_p)$,
where, for each $p$, the inclusions $E'_p\hookrightarrow E'_{p+1}$, $F'_p\hookrightarrow F'_{p+1}$ are compact. The following properties
are equivalent:
\begin{enumerate}
\item $A(E)=F$;
\item For each $p\in\N$, there is $q\in\N$ such that, if ${\cal{B}} \subset F'$ is such that $\AT({\cal{B}})$ is contained and bounded in $E'_p$,
then ${\cal{B}}$ is contained and bounded in $F'_q$;
\item For each $p\in\N$, there is $q\in\N$ such that, if $u\in F'$ is such that $\AT(u)\in E'_p$, then $u\in F'_q$.
\end{enumerate}
\end{thm}

\begin{proof} Since every strongly bounded subset of $E'$ is contained and
bounded in one of the Banach spaces $E'_p$ it is clear that (2) implies (4) of
Theorem \ref{thm:FM} and hence (1) holds. Conversely, if (1) holds then, by Theorem
\ref{thm:FM}, $\AT$ is a strong homomorphism. By \cite[Theorem 7']{komatsu1967projective},
$\AT(F')=\mbox{ind}\,(E'_p\cap \AT(F'))$, that is, $\AT(F')$ can also be described as the inductive limit of the sequence of Banach spaces
$G_p\doteq E'_p\cap \AT(F')$ with the corresponding compact inclusions $G_p\stackrel{\iota_p}{\hookrightarrow} G_{p+1}$. For each $p\in\N$, we set
$\lambda_p=(\AT)^{-1}|_{G_p}:G_p\sra F'$. Since $\lambda_p= \lambda_{p+1}\circ \iota_p$, it follows that each $\lambda_p$ is a compact linear map. Consequently,
if $U_p$ denotes the unit ball in $G_p$, then $\lambda_p(U_p)$ is strongly bounded in $F'$ and hence it is contained in $F'_q$ for some $q\in\N$
(and ``a fortiori'' $\lambda_p:G_p\sra F'_q$ is a continuous linear map between Banach spaces). We have
proved the following assertion: for each $p\in \N$, there is $q\in\N$ such that $(\AT)^{-1}|_{G_p} \in L(G_p, F'_q)$, from which (2) follows immediately.

Next, it is clear (2) implies (3) after taking ${\cal{B}}=\{u\}$. We are then left with the proof that (3) implies (2).
For this, it suffices so show that
the following strengthen form of (3) is satisfied (in the argument, we shall denote by $|\cdot|_p$ the norm in $E'_p$ and by $\|\cdot\|_p$ the norm in $F'_p$):
\begin{itemize}
 \item[($\bullet$)] {\sl Given $p\in\N$,  there are $q\in \N$ and $C>0$ such that,
if $u\in F'$ and $\AT u\in E'_p$, then $u\in F'_q$ and $\|u\|_q \leq C |\AT u|_p$}.
\end{itemize}

Indeed, for each $p\in \N$, take $q\in\N$ as in (3).
The space ${\mathfrak{E}}$ of all $u\in F'_{q+1}$ such that $\AT u\in E_p$
is a Banach space when we consider the norm $u \mapsto  \|u\|_{q+1} + |\AT u|_p$.
Property (3) gives ${\mathfrak{E}}\subset F'_q$ and the closed graph theorem implies the existence of a constant $\mu>0$ such that
$$   \|u\|_q \leq \mu \left( |\AT u|_p + \|u\|_{q+1}\right), \qquad u\in {\mathfrak{E}}. \leqno{(\sharp)} $$

If ($\bullet$) were not true, it would exist a sequence $\{u_j\}\subset F'_q$ such that $\{\AT u_j\}\subset E'_p$ and
$\|u_j\|_{q} > j|\AT u_j|_p$.
If we define $v_j=u_j/\|u_j\|_{q}$, then $\{v_j\}\subset E'_q$, $\|v_j\|_{q}=1$ for every $j$ and $\AT v_j\sra 0$ in $F'_p$. Since the inclusion
$F'_q\subset F'_{q+1}$ is compact, some subsequence $\{v_{j_k}\}$ of $\{v_j\}$ must converge in $F'_{q+1}$. Denoting by
$v\in F'_{q+1}$
the limit of this subsequence, we have $\AT v=0$, and hence $v=0$ since $A(E)$ is dense in $F$. On the other hand ($\sharp$) implies
$1 \leq \mu \left\{ |\AT v_{j_k}|_{p} + \|v_{j_k}\|_{q+1} \right \}$, $k=1,2,\ldots,$
and consequently $\|v\|_{q+1}\geq 1/\mu$, which is a contradiction. \end{proof}
\vspp







\section{The associated differential complex}

Let $\Omega$ be a smooth manifold and denote by $N$ its dimension. We always assume that $N \geq 2$. An involutive structure on $\Omega$ is a smooth subbundle $\mathcal V$ of the complexified tangent bundle $\C T \Omega$ of $\Omega$ that satisfies the involutive, or Frobenius, condition $[\mathcal V, \mathcal V] \subset \mathcal V$. We always denote the rank of $\mathcal V$ by $n$. We denote by $\Lambda^k$ the bundle $\Lambda^k \C T^* \Omega$ and by $\mathcal C^\infty(\Omega; \Lambda^k)$ the space of sections of $\Lambda^k$ with smooth coefficients. % in the sheaf $\mathcal F$. We are going to be using the following sheaves $\mathcal F = \mathcal D'$ and $\mathcal F = \mathcal C^\infty$.



% It is well known that to each involutive  structure is associated a complex  of differential  operators, and from that point of view, they are well studied in partial differential equations.

There is a natural differential complex associated to each involutive structure $\mathcal{V}$. We briefly recall the construction of such complexes. For each $x \in \Omega$, we define $$T'_x = \{ u \in \C T^*_x \Omega: u(X) = 0 ,~ \forall X \in \mathcal V_x \}$$ and we have that
$ T' = \bigcup_{x \in \Omega} T'_x $
is a vector subbundle of $\C T^*\Omega$. For each $p, q \in \Z_+$, we denote by $T^{p,q}_x$ the subspace of $\Lambda^{p+q} \C T_x^*\Omega$ consisting of linear combinations of exterior products $u_1 \wedge \ldots \wedge u_{p+q}$ with $u_j \in \C T_x^*\Omega$ for $j = 1, \ldots, p+q$ and at least $p$ of these factors belonging to $T'_x$.
Notice that $T^{p+1,q-1}_x \subset T^{p,q}_x$ and so we can define $\Lambda^{p,q}_x \doteq  T^{p,q}_x / T^{p+1,q-1}_x$ and consequently $\Lambda^{p,q} = \bigcup_{x \in \Omega} \Lambda^{p,q}_x $ is a smooth vector bundle over $\Omega$. Since $\mathcal{V}$ is involutive, we can easily verify that the exterior derivative take smooth sections of $T^{p,q}$ into smooth sections of $T^{p,q+1}$ and hence there exist a unique operator $\dext'_{p,q}$ such that the diagram
$$
\xymatrix{
 T^{p,q} \ar[r]^{\dext} \ar[d]_{\pi_{p,q}}& T^{p,q+1} \ar[d]^{\pi_{p,q+1}} \\
\Lambda^{p,q} \ar[r]_{\dext'_{p,q}} & \Lambda^{p,q+1}
}
$$
is commutative, with $\pi_{p,q} : T^{p,q} \to \Lambda^{p,q}$ being the quotient map.

When there is no risk of confusion, we simplify the notation and write simply $\dext '$
for the operator $\dext'_{p,q}$. We refer as $\dext'_{\mathcal V}$ when it is necessary to emphasize the associated involutive structure.

We denote by $\mathcal C^\infty(\Omega; \Lambda^{p,q})$ %, or $\Lambda^{p,q}(\Omega)$,
the space of sections of $\Lambda^{p,q}$ with smooth coefficients. % in the sheaf $\mathcal F$. To emphasize the associated involutive structure, we again use a subindex and we write $\Lambda^{p,q}_{\mathcal V}$. % or $\Lambda^{p,q}_{\mathcal V}(\Omega)$.
Notice that the operator $\dext'$ maps smooth sections of $\Lambda^{p,q}$ into smooth sections of $\Lambda^{p,q+1}$ and also that $\dext' \circ \dext' = 0$. Therefore, for each $p \geq 0$, the operator $\dext'$ defines a complex of $\C$-linear mappings
\begin{equation}
\label{h_complex}
 \mathcal C^\infty(\Omega; \Lambda^{p,0}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,1})  \xrightarrow{\dext'} ... \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \xrightarrow{\dext'} \ldots
\end{equation}

% Of course we also have a complex for the sheave of distributions $\mathcal D'$ and $\mathcal F = \mathcal B$.

Of course we obtain another differential complex after replacing $\mathcal C^\infty$ by $\mathcal C^\infty_c$, where $c$ stands for compact supports.

For each $p \geq 0$, we denote the set of the $(p,q)$-cocycles elements by
$$ Z^{p,q} (\Omega; \mathcal V) = \ker \left( \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \right),$$
the set of $(p,q)$-coboundaries by
 $$ B^{p,q} (\Omega; \mathcal V) = \img \left( \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q-1}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q}) \right),$$
and the $(p,q)$-cohomology classes by
 $$  H^{p,q} (\Omega; \mathcal V) = \frac{Z^{p,q} (\Omega; \mathcal V)}{B^{p,q} (\Omega; \mathcal V)}$$
 (we set $B^{p,0}(\Omega)=\{0\}$).

Given any open set $V \subset \Omega$ we can restrict the involutive structure $\mathcal V$ to $V$, which we still denote by $\mathcal V$, and construct a complex $\left( \mathcal C^\infty(V; \Lambda^{p,q}), \dext' \right)$. And, by restriction, we have a homomorphism of differential complexes
$$ \left( \mathcal C^\infty(\Omega; \Lambda^{p,q}), \dext' \right) \to \left( \mathcal C^\infty(V; \Lambda^{p,q}), \dext' \right).$$ This then  allows us to define, for a given $x \in V$,  $$ \mathcal H^{p,q} (\{x\}; \mathcal V) = \varinjlim_{V \ni x} H^{p,q}(V; \mathcal V) $$ the inductive limit of $H^{p,q}(V; \mathcal V)$ taken when  $V$ varies in the set of all open neighborhoods of $x$.

\begin{exa}
By taking $\mathcal V = \C T \Omega$, we have the simplest involutive structure. In this case, the operator $\dext'$ is just the usual exterior derivative. The space $H^p_{\mathcal C^\infty} (\Omega; \mathcal V)$ is just the de Rham cohomology space.
\end{exa}


\begin{exa}
Suppose that $J : T \Omega \to T \Omega$ is a vector bundle isomorphism satisfying $J \circ J = -\operatorname{Id}$ and
\begin{equation}
\label{chp:inv:j_complex}[JX, JY] = [X,Y] + J[JX, Y] + J[X,JY].
\end{equation} We extend $J$ complex-linearly to the complexified tangent bundle $\C T \Omega$ and we take $\mathcal V = \ker(J - i{\operatorname{Id}})$. The condition \eqref{chp:inv:j_complex} implies that  $\mathcal V$ is involutive. This structure is called a \emph{complex structure} over $\Omega$ and, in this case, the operator $\dext'$ is the Doubeault operator $\delbar$.
\end{exa}
It is also important to consider the preceeding complexes with more general coefficients. In order to do so, we assume from now on that
$$   \mbox{$\Omega$ is orientable.} $$
Under this hypothesis, we can also construct a complex similar to \eqref{h_complex}
where now the coefficients are distributions over $V$. In this case, we denote the cohomology space by
$   H^{p,q}_{\mathcal D'} (V; \mathcal V).$ In general, if $F(V)$  is a subspace
of $\Dli(V)$, we denote by $F(\Omega; \Lambda^{p,q})$ %, or $\Lambda^{p,q}(\Omega)$,
the space of sections of $\Lambda^{p,q}$ with coefficients in $F$ and we denote the cohomology of $\dext'$ with coefficients in $F(V)$ by $ H^{p,q}_{F} (V; \mathcal V).$
Furthermore, by \cite[Propositions VIII.1.2 and VIII.1.3]{treves1992hypo}, there is a natural bracket
which turn the spaces
$$ \mathcal C_c^\infty(V;\Lambda^{p,q})\mbox{ and } \Dli(V;\Lambda^{m-p,n-q})
\,\, (\mbox{resp. }   \mathcal C^\infty(V;\Lambda^{p,q})\mbox{ and }
\mathcal{E}'(V;\Lambda^{m-p,n-q})) $$
into the dual of one another and in such a way that the transpose of $\dd'$ is also $\dd'$ (up to a sign).

We can endow each space $\mathcal C^\infty(V;\Lambda^{p,q})$ with a locally convex structure of an ({\bf{FS}}) space. Its dual $\mathcal{E}'(V;\Lambda^{m-p,n-q})$ is then a ({\bf{DFS}}) space and a sequence of definition for its topology can be taken by the  sequence
$$     \GG_j(V;\Lambda^{m-p,n-q}) := \{u\in H^{-j}_{\tiny{\mbox{loc}}}(V,\Lambda^{m-p,n-q}): \,\mbox{supp}\, u \subset K_j \}, $$
where $\{K_j\}$ is an exhaustion of $V$ by compact sets (with the inclusions $$\GG_j(V;\Lambda^{m-p,m-q}) \hookrightarrow \GG_{j+1}(V;\Lambda^{m-p,m-q})$$ being compact by the Relich lemma).

We conclude this section by stating a direct consequence of Theorem \ref{thm:FS}.

\begin{thm}\label{thm:main}
Let $\Omega$ be an orientable differentiable manifold endowed with a formally integrable structure. Assume that
\begin{equation}\label{density}
\dd' : \mathcal{E}'(\Omega;\Lambda^{m-p,0}) \lra \mathcal{E}'(\Omega;\Lambda^{m-p,1})
\end{equation}
is injective. Then the map
\begin{equation}\label{1}
 \dd':  \mathcal C^\infty(\Omega;\Lambda^{p,n-1}) \lra \mathcal C^\infty(\Omega;
\Lambda^{p,n}) \end{equation}
is surjective (which is the same as saying that $H^{p,n}(\Omega; \VV)=0$) if and only if the following property holds:
\begin{itemize}
\item[$(\dagger)$] Given $K\subset \Omega$ compact and $s\in \R$, there are
 $K_1\subset \Omega$  compact and  $t\in \R$ such that the following holds for an arbitrary $u\in \mathcal{E}'(\Omega;\Lambda^{m-p,0})$:
$$ \mathrm{supp}\,\dd'u \subset K,\,\, \dd' u \in H^s_{\tiny{\mathrm{loc}}}(\Omega,\Lambda^{m-p,1}) \Longrightarrow  \mathrm{supp}\, u\subset K_1,\,\, u\in H^t_{\tiny{\mathrm{loc}}}(\Omega,\Lambda^{m-p,1}). $$
\end{itemize}
\end{thm}

Indeed, Property \eqref{density} is equivalent to the fact that \eqref{1} has dense image and hence Theorem \ref{thm:FS} applies immediately.

Under an additional property, we can strength the result stated in Theorem \ref{thm:main}. We introduce the following definition:

\begin{dfn}\label{dfn:contun} We shall say that $\VV$ satisfies property $(\star)$ if given $V\subset \Omega$ open and $u\in \Dli(V;\Lambda^{p,0})$ satisfying $\dd' u=0$ in a nonempty  connected open subset
$\omega$ of $V$ then $u$ vanishes identically in the component of $V$ that contains $\omega$.
\end{dfn}


\begin{prp}\label{prp:imp} Let $\Omega$ be an orientable differentiable manifold endowed with a formally integrable structure. Suppose that $\Omega$ has no compact connected component and that $\VV$ satisfies $(\star)$. Then
\begin{enumerate}
 \item  The kernel of the map $\dd':\mathcal E'(\Omega;\Lambda^{m-p,0})\sra \mathcal E'(\Omega;\Lambda^{m-p,1})$ is trivial;
\item If $K\subset \Omega$ is compact and if $u\in \Eli(\Omega;\Lambda^{m-p,0})$ is such that $\mbox{supp}\,\dd 'u\subset K$ then $\mbox{supp}\, u\subset \tilde K$,
where $\tilde K$ is the compact set obtained as the union of $K$ with the relatively compact components of $\Omega\setminus K$.
\end{enumerate}
\end{prp}

The proof is immediate.
\vspp

From Theorem \ref{thm:main} and Proposition \ref{prp:imp} we obtain:

\begin{cor}\label{cor:Main} Let $\Omega$ be an orientable differentiable manifold endowed with a formally integrable structure. Suppose that $\Omega$ has no compact connected component and that $\VV$ satisfies $(\star)$.
If for a given $K\subset \Omega$ compact
and for a given $s\in \R$ there is $t\in \R$ such that
$$ u\in \mathcal E'(\Omega,\Lambda^{m-p,0}),~ \supp\, \dext' u\subset K,~ \dext' u\in H^s_{\tiny\mathrm{loc}}(\Omega;\Lambda^{m-p,1}) \Longrightarrow u\in
H^t_{\tiny\mathrm{loc}}(\Omega;\Lambda^{m-p,0}) $$
then $H^{p,n}(\Omega;\VV)=0$.
\end{cor}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HYPOCOMPLEX STRUCTURES %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Hypocomplex structures}

From now on, we assume the stronger property that the structure $\mathcal V$ is {\sl locally integrable}. This means that, in a neighborhood of an arbitrary point $\pp\in \Omega$, there are defined $m=N-n$ smooth functions whose differentials span
$T'$ at each point in a neighborhood of $\pp$. Notice that each of these functions is annihilated by the operator  $\dd'$, that is, they are solutions for $\VV$.
In this section, we are going to introduce the concept of hypocomplex structures, a class of structures with some
good analytical properties, similar to the class of holomorphic functions. Such analytical properties are going to
be used to find conditions so that the operator $\dext'$ in maximum degree has closed range.

Let $\pp \in \Omega$. We denote by $\mathcal S(\pp)$ the ring of germs of solutions of $\mathcal V$ at $\pp$, that is,
$$ \mathcal S(\pp) = \{ f \in \mathcal C^\infty(\pp) : \dext' f = 0 \},$$
and we denote by $\mathcal O^m_0$ the ring of germs holomorphic functions defined in a neighborhood of $0$ in $\C^m$.

Now, consider $Z_1, \ldots, Z_m$ solutions for $\VV$, defined in an open neighborhood of $\pp$ with linearly independent differentials, and denote by $Z$ the map $Z = (Z_1, \ldots, Z_m)$ defined in a neighborhood of $\pp$. Of course, we assume that $Z(\pp)=0$.

We define a ring homomorphism
$$ \lambda : h\in \mathcal O^m_0 \mapsto  h \circ Z \in  \mathcal S(\pp). $$
% defined by $$ \Lambda (h) = h \circ Z.$$
It is not difficult to prove that $\lambda$ is injective. We shall say that $\mathcal V$ is \emph{hypocomplex} at $\pp$ if $\lambda$ is surjective, that is, if for every $f \in \mathcal S(\pp)$ there exist a holomorphic function $h \in \mathcal O^m_0$ such that $f = h \circ Z$. % We say that $\Omega$ is a \emph{hypocomplex manifold} if the involutive structure is
%Notice that the map $x \mapsto Z(x) = x + i\phi(x, 0)$ defines the germ at 0 of a maximally real submanifold $\Sigma \subset \C^m$ and since for $h \in \mathcal O^m_0$, if $h|_\Sigma = 0$ then we have $h = 0$. This implies that $\Lambda$ is an injective homomorphism.

The next result follows directly from the definitions:

\begin{prp}\label{prp:hypoxstar}
If $\VV$ is hypocomplex at each point, then $\VV$ satisfies Property $(\star)$.
 \end{prp}

A particular but important class of hypocomplex structures is that of the elliptic structures. Recall that the {\sl characteristic set of} $\VV$ is the set $C(\VV) = \VV^\perp \cap T^*\Omega$ and
that the structure is {\sl elliptic} if $C(\VV)=0$. Every elliptic structure, being hypocomplex ([T4, Proposition III.5.1]),
satisfies Property ($\star$) and, moreover,
given $\pp\in\Omega$ and $s\in\R$, the following is true:
if $u\in{\cal{D}}'(\Omega,\Lambda^{m-p,0})$ and $\dd' u\in H^s_{\loc}(\{\pp\};\Lambda^{m-p,1})$
then $u\in H^{s+1}_{\loc}(\{\pp\},\Lambda^{m-p,0})$. From Corollary \ref{cor:Main} follows:

\begin{thm}
Suppose that $\Omega$ has no compact connected component and that $\VV$ is elliptic.
Then $H^{p,n}(\Omega;\VV)=0$.
\end{thm}

Another important class of hypocomplex structures is the one described in the following. Assume that $\Omega$ is endowed with a locally integrable structure $\VV$. Let
 $T^0=  T' \cap \C T^* \Omega$ denote the characteristic set of $\VV$. Given $(\pp,\xi)\in T^0$, $\xi\neq 0$, the \emph{Levi form} at  $(\pp,\xi) \in T^0$ is the Hermitian form on $\mathcal V_x$ defined by $$\mc L_{(\pp,\xi)}(v,w) = (1/2i)\xi([L,\overline{M}]_\pp), \quad v,w \in \mathcal V_\pp,$$
 in which $L$ and $M$ are any smooth local sections of $\mathcal V$ in a neighborhood of $\pp$ such that $L_\pp = v$ and $M_\pp = w$. We shall say that $\mc L$ is \emph{nondegenerate} if given any point $(\pp,\xi) \in T^0$, with $ \xi \neq 0$, the hermitian form $\mc L_{(\pp,\xi)}$ is nondegenerate.

The following result is due to Baouendi-Chang-Treves \cite{baouendi1983microlocal}:

\begin{thm}\label{thm:BCT}
Let $\Omega$ be endowed with a locally integrable structure for which the Levi form at
each $(\pp,\xi)\in T^0$, $\xi\neq 0$, has one positive and one negative eigenvalue. Then
$\VV$ is hypocomplex.
\end{thm}

Assume now that the locally integrable structure $\VV$ has rank $N-1$, that is, $T'$ is a complex line bundle. For such, structures hypocomplexity is completely characterized \cite{treves1992hypo}:

\begin{thm}\label{thm:open}
If the locally integrable structure $\VV$ has rank $N-1$, then $\VV$ is hypocomplex if and only if given any $\pp\in \Omega$ and given any local solution $Z$ for $\VV$ near
$\pp$ with $\dd'Z_\pp\neq 0$ then $Z$ is open at $\pp$.
\end{thm}








%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% RAGOGNETE'S THEOREM %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section {A remark on local solvability}

Let $\Omega$ be endowed with a locally integrable structure $\VV$. We shall now make use of the local representation for $\VV$ as described in \cite{treves1992hypo}, \cite{berhanu2008introduction}. Any point $\pp\in\Omega$ is the center of a coordinate system $(x,t) = (x_1, \ldots, x_m, t_1, \ldots, t_n)$ defined on an open neighborhood of $p$ denoted by $U$ such that $(x(\pp),t(\pp)) = (0,0) \in \R^m \times \R^n$.
On $U$ it is defined a smooth function $\phi(x,t) = (\phi_1(x,t), \ldots,$ $\phi_m(x,t))$ satisfying $\phi(0,0) = 0$ and $\phi_x(0,0) = 0$ such that the differentials of the functions
\begin{equation}
\label{chp:inv:first_integrals}
Z_k(x,t) = x_k + i\phi_k(x,t), \quad k = 1, \ldots, m
\end{equation}
 are linearly independent and span $T'$ over $U$. If we define the vector fields $$M_k = \sum_{j=1}^m \mu_{kj}(x,t) \frac{ \del }{ \del x_j}, \quad k = 1, \ldots, m,$$
characterized by the rule $M_kZ_j = \delta_{k,j}$ for $k,j = 1, \ldots, m$, then the complex vector fields
$$ L_j = \frac{ \del }{ \del t_j} - i\sum_{k=1}^m \frac{ \del \phi_k }{ \del t_j }(x,t)M_k, \quad j = 1, \ldots, n, $$
span $\mathcal V$ over $U$. The vector fields $L_j$ and $M_k$ commute pairwise.

The differentials $\dext t_k$, for $k = 1, \ldots, n$, span a bundle over $U$, which is supplementary to $T'|_U$. Therefore we can adjoin them with $\dext Z_k$, for $k = 1, \ldots, m$, to get a smooth basis for $\C T^* \Omega$. So, if $f$ is a smooth section of $\Lambda^{p,q}$ over $U$, we have the following unique representation for $f$:
$$ f = \sum_{|J| = p} \sum_{|K| = q} f_{J,K}(x,t) \dext Z_J \wedge \dext t_K.$$

The standard representation of $\dext'f$ over $U$ is then given by
$$ \dext' f = \sum_{|J| = p} \sum_{|K| = q} \sum_{l=1}^n \left( L_l  f_{J,K} \right) (x,t) \dext t_l \wedge \dext Z_J \wedge \dext t_K. $$


The goal of this section is to prove the following result:

\begin{prp}
\label{prp:equiv} Let $\Omega$ be endowed with a locally integrable structure $\mathcal V$ and let $\pp \in \Omega$. The following properties are equivalent, for a fixed $q\in\{1,\ldots,n\}$:
\begin{enumerate}
\item \label{hypo:prp:equiv1} $ \mathcal H^{0,q}_{\mathcal C^\infty} (\{\pp\}, \mathcal V) = 0$;
\item \label{hypo:prp:equiv2} $ \mathcal H^{0,q}_{\mathcal D'} (\{\pp\}, \mathcal V)= 0$;
\item $ \mathcal H^{p,q}_{\mathcal C^\infty} (\{\pp\}, \mathcal V) = 0$ for all $p = 0, 1, 2, \ldots, m$;
\item $ \mathcal H^{p,q}_{\mathcal D'} (\{\pp\}, \mathcal V)= 0$ for all $p = 0, 1, 2, \ldots,m$.
\end{enumerate}
\end{prp}

\begin{proof} From the discussion that precedes, it is clear that it suffices to prove the equivalence between (1) and (2).
We first prove that \eqref{hypo:prp:equiv1} implies \eqref{hypo:prp:equiv2} by using in part an argument in \cite{andreotti1981absence}. We keep the notation just established
and apply the well known Grothendieck argument as in \cite[Theorem VII.6.1]{berhanu2008introduction}:
given $U_0\subset U$ an open neighborhood of the origin, there corresponds another open neighborhood $V_0\ssubset U_0$ such that, if we set
$$    \EE := \{(f,u)\in Z^{0,q}(U_0)\times C^\infty(V_0,\Lambda^{0,q-1}) :
\dd' u =f|_{V_0} \},$$
then the projection map $\pi:\EE \sra Z^{0,q}(U_0)$ (a continuous linear map between Fréchet spaces) is surjective and hence open. If we follow \cite{andreotti1981absence}, we can ensure:

\begin{itemize}
\item Given $K'\subset V_0$ compact and $\nu'$ a positive integer, there are $K\subset
U_0$ compact, $\nu$ a positive integer and $C>0$ such that the following is true: if $f\in Z^{0,q}(U_0)$, there is $u\in C^\infty(V_0,\Lambda^{0,q-1})$ such that
$$     \|u\|_{\nu',K'}\leq C\|f\|_{\nu,K}. $$
\end{itemize}
We obtain
$$ \|f\|_{\nu,K} \doteq \sup_{|\alpha| \leq \nu} \sup_K |D^\alpha f|. $$

In order to conclude (2), we make use of \cite[Theorem II.5.2]{treves1992hypo}. It suffices to establish the following solvability property:

\begin{itemize}
\item Given an open neighborhood $U_1$ of the origin, there is $\mu$ such that, if $f\in \mc C^\mu(U_1;\Lambda^{0,q})$ satisfies $\dd'f=0$, we can find $u\in \Dli(\{0\};\Lambda^{0,q-1})$ solving $\dd'u =f$.
\end{itemize}

We first apply the approximate Poincaré lemma \cite[Section II.6]{treves1992hypo}: there is
an open neighborhood $U_0\ssubset U_1$ of the origin such that the conclusion of \cite[Theorem II.6.1]{treves1992hypo} holds. Now we refer to the discussion presented before: taking a sufficiently small closed ball
$K_0$ centered at the origin, there are $\mu$ and $C>0$ such that, for every
$g\in Z^{0,q}(\overline{U_0};\Lambda^{0,q})$, there is
$v\in C^\infty(K_0,\Lambda^{0,q-1})$ such that $\dd' v = g$ in $K_0$
and
$$       \|v\|_{K_0,0}\leq C \|g\|_{\overline{U_0},\mu}. $$
This defines our sought $\mu$. Given $f\in C^\mu(U_1,\Lambda^{0,q})$, we can find $f_j\in Z^{0,q}(\overline{U_0})$ such that
$f_j\sra f$ in $\mc C^\mu (\overline{U_0};\Lambda^{0,q})$. Let $u_j \in C^\infty(K_0,\Lambda^{0,q-1})$ such that $\dd' u_j = f_j$ in $K_0$
and
$$       \|u_j\|_{K_0,0}\leq C \|f_j\|_{\overline{U_0},\mu}. $$
This shows that $u_j$ is bounded in $L^\infty(K_0;\Lambda^{0,q-1})$ and hence some subsequence of $u_j$ converges weakly to some $u$ defined in the interior of $K_0$, which a fortiori satisfies $\dd'u=f$.

For the proof that (2) implies (1), we again start by applying the Grothendieck argument, this time in the following way. Let $U_0$ be a neighborhood of the origin, let
$\omega_j\ssubset U_0$ be a fundamental system of neighborhoods of the origin
and define
$$    \EE_j \doteq \{(f,u)\times Z^{0,q}(U_0)\times H^{-j}_{\mbox{\small loc}}(\omega_j):
 \dd 'u=f|_{\omega_j} \}. $$
By the standard argument, we can find $V_0\subset U_0$ an open neighborhood of the origin and $\sigma\in\R$ such that the following is true:
\begin{itemize}
\item Given $f\in Z^{0,q}(U_0)$, there is $u\in H^{-\sigma}_{\mbox{\small loc}}(V_0,\Lambda^{0,q-1})$ such that $\dd'u=f|_{V_0}$.
\end{itemize}

The proof completes  after applying the argument presented in the proof of  \cite[Theorem VIII.9.1]{treves1992hypo}
\end{proof}


\begin{rmk}\label{rmk:1}
Inspection of the proof of Proposition \ref{prp:equiv} shows that Properties (1) to (4)
in Proposition \ref{prp:equiv} are still equivalent to the following one:
\begin{itemize}
\item[5.] Given $s\in\R$, there is $t\in\R$ such that, if $f\in H^{s}_{\mbox{\small loc}}(\{\pp\},\Lambda^{p,q})$ satisfies $\dd'f=0$, then there is $u\in H^{t}_{\mbox{\small loc}}(\{\pp\},\Lambda^{p,q-1})$ such that $\dd' u=f$, $p=0,1,\ldots,m$.
\end{itemize}
\end{rmk}



Next, we state the main theorem of this chapter:

\begin{thm}\label{thm:first}  Let $\Omega$ be orientable with no compact connected component. Assume also that $\Omega$ is endowed with a hypocomplex structure $\mathcal V$. If the equivalent conditions in Proposition \ref{prp:equiv} hold for $q=1$, then
$$   H^{p,n}_{\mathcal C^\infty}(\Omega) = 0,\qquad p = 0, 1, 2, \ldots.$$
\end{thm}

\begin{proof} We apply Corollary \ref{cor:Main}. Let $K\subset \Omega$ be compact, $s\in\R$ and assume that $u \in \mc E '(\Omega;\Lambda^{m-p,0})$
satisfies $\supp~ u\subset K$, $\dd'u \in H^{s}_{\mbox{\small loc}}(\Omega;\Lambda^{m-p,1})$. By Remark \ref{rmk:1}, for each $\pp\in \supp~ u$ we can find $t\in \R$ and $v_\pp\in
H^{t}_{\mbox{\small loc}}(\{\pp\},\Lambda^{p,0})$ with $\dd'v_\pp= \dd'u$ near $\pp$.
By compactness, we can select $t$ independent of the choice of $\pp$. Furthermore, since $\VV$ is hypocomplex, it follows that $u-v_\pp$ is smooth near $\pp$ and hence
$u\in  H^{t}_{\mbox{\small loc}}(\{\pp\},\Lambda^{p,0})$. Since $\pp$ is arbitrary, Corollary \ref{cor:Main} gives the result. \end{proof}




\section{Examples}

We now apply Corollary \ref{cor:Main} and Theorem \ref{thm:first} to derive some examples:

%\begin{exa}\label{exa:1}
%Suppose that $\Omega$ has no compact connected component and that $\VV$ is a locally integrable
%CR structure of codimension $d>0$ satisfying the following property:
%$$
% \mbox{\sl The Levi form of $\VV$ at each $\theta\in T^0\setminus 0$ has at least one negative eigenvalue.}$$
%Then $H^{p,n}_{\mc C^\infty}(\Omega;\VV)=0$.
%\end{exa}

%\begin{proof} The hypothesis on the Levi form implies that $\VV$ is hypocomplex [BCT, Corollary 6.1]. Moreover from
%[SW, Theorem 1] our hypothesis also implies the following one: given $\pp\in\Omega$, if $u\in{\cal{D}}'(\Omega;\Lambda^{p,0})$
%and $\dd' u\in H^s_{\loc}(\{\pp\};\Lambda^{p,1})$
%then $u\in H^{s+1/2}_{\loc}(\{\pp\};\Lambda^{p,0})$. The conclusion follows from Corollary \ref{cor:Main}. \end{proof}

\begin{exa}\label{exa:2}
Let ${\cal{M}}$ be an oriented, real-analytic manifold of dimension $n\geq 1$ and set
$\Omega\doteq \R\times{\cal{M}}$. Given a real-analytic function $\Phi:{\cal{M}}\sra \R$, we shall consider the locally
integrable structure $\VV$ on $\Omega$ whose orthogonal $T'$ is spanned by the differential of the function $Z:\Omega\sra \C$,
$Z(x,\qq)=x+i\Phi(\qq)$, $x\in\R$, $q\in {\cal{M}}$. Notice that, if $(t_1,\ldots,t_n)$ are local coordinates on an open subset
$W$ of ${\cal{M}}$, then $\VV$ is spanned, over $\R\times W$, by the vector fields
$$ \LLl_j = \frac{\partial}{\partial t_j}-i\frac{\partial \Phi}{\partial t_j}(t)\frac{\partial}{\partial x}, \quad j=1,\ldots, n.$$
We show that, under these conditions, if $\Phi$ is an open map then $H^{q,n}_{\mc C^\infty}(\Omega;\VV)=0$.
\end{exa}

\begin{proof}
 According to Theorem \ref{thm:open}, the structure $\VV$ is hypocomplex. Moreover, from
[JT, Theorem 1.5], the following property holds: given $(x_0,\qq_0)\in\Omega$,
if $u\in{\cal{D}}'(\Omega;\Lambda^{q,0})$ and $\dd' u\in H^s_{\loc}(\{(x_0,\qq_0\};\Lambda^{q,1})$,
then $u\in H^{s-n/2}_{\loc}(\{x_0,\qq_0\};\Lambda^{p,0})$. The conclusion follows again from Corollary \ref{cor:Main}.
\end{proof}

\begin{exa} Let $\Omega$ be orientable with no compact connected component. Suppose that $m = 1$ and suppose that $\mathcal V$ satisfies:
\begin{enumerate}
    \item $\VV$ is hypocomplex (cf. Theorem \ref{thm:open});
    \item $\VV$ satisfies Condition $(\star)_0$ (as discussed in \cite{cordaro2001local}) at every point.
\end{enumerate}
Then $H^{p,n}(\Omega; \VV) = 0$.
\end{exa}

\begin{exa}
\label{exa:2'}
Let $\Omega$ be an analytic orientable manifold with no compact connected component. Suppose that $\VV$ is analytic and suppose that, for $(\pp, \xi) \in T^0$ with $\xi \neq 0$, we have that $\mc L_{\pp, \xi}$ is non-degenerate and has signature different from $n$ and $n-2$. Then $H^{p,n}(\Omega; \VV) = 0$.
\end{exa}

The following example is a particular case of Example \ref{exa:2'}.

\begin{exa}\label{exa:3}
Let $\mc Q : \C^k \times \C^k \to \C^d$ be a quadratic form and consider the (non compact, connected) quadric submanifold $\Omega = \{(x + iy, w) \in \C^d \times \C^k : y = \mc Q(w, \overline{w})\}$. We endow $\Omega$ with the involutive structure $\mc V$ generated by the vector fields
$$ L_j =  \frac{\del}{\del w_j} + 2i \sum_{l=1}^d \frac{ \del \mc Q_l}{ \del w_j} \frac{\del}{\del z}, \qquad 1 \leq j \leq k.$$ This involutive structure is a CR structure (we refer to \cite{boggess1991cr} to a detailed description of this class of CR manifolds and the computation of its Levi form). Since the characteristic set of $\VV$ is a real line bundle, it suffices to compute it at $(\pp,\xi)$, with $\xi \in T^0_0$.
Up to a sign, this Levi form equals $\mc Q$. If $\mc Q$ is non-degenerate and has at least one positive and one negative eigenvalue, then $\mc V$ is hypocomplex. Furthermore,
 if its signature is different from $n-2$, then the equivalent conditions in Proposition \ref{prp:equiv} hold when $q=1$. Hence, we can infer that $H^{p,n}(\Omega;\VV)=0$ when the signature of $\mc Q$ is different from $n$ and $n-2$. In Chapter 3, we shall see that this example corresponds to a left-invariant hypocomplex CR structure defined in a suitable Lie group.
 \end{exa}

\section{Sheaf cohomology}

In this section, we are going to be assuming that $\mathcal V$ is hypocomplex, but we make no restrictions to the manifold, that is, $\Omega$ can have compact connected components. Let $\mathcal S^p$ be the sheaf $(p,0)$-forms which, are solutions of $\mathcal V$ over $\Omega$, and denote by $\Phi$ a paracompactifying family of supports in $X$. We denote by $H^q_\Phi(\Omega; \mathcal S^p)$ the \emph{cohomology group over $\Omega$ with coefficients in $\mathcal S^p$ and support in $\Phi$}. We are interested in the family of supports consisting of all compacts subsets of $\Omega$ which is going to be denoted by $c$. % We are interested particularly in the topological properties of $H^1_c(\Omega; \mathcal S^p)$.

Following \cite{gunning1965analytic}, we recall some notions related to \v Cech cohomology of a covering with values in a sheaf which allows us to use functional analysis to study the operator $\dext'$ and the space $H^1_c(\Omega; \mathcal S^p)$. % The main reason for using \v Cech cohomology in this work is to be able to study cohomology of the operator $\dext'$ using tools from functional analysis. % But first we need the following:

This sheaf cohomology can be related to the cohomology introduced in the beginning of this chapter  via a spectral sequence (cf. \cite{godement1958topologie} Théorème 5.2.4). A particular case of this can be done in locally trivial cohomologies, which is the case of elliptic structures, for example. In fact, if the involutive structure $\mathcal V$ is elliptic, by the Poincaré Lemma for elliptic structures (cf.  \cite{berhanu2008introduction} Theorem VIII.3.1), we know that $\dext'$ is locally exact, so we have a fine resolution of $\mathcal S$. Therefore, we have, for $q > 0$,

$$ H^q(\Omega; \mathcal S^p) = \frac { \ker \left[ \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q+1}) \right] }{ \img \left[ \dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q-1}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q}) \right] } $$
and
$$ H^0(\Omega; \mathcal S^p) =  \ker \left[ \dext' :\mathcal  C^\infty(\Omega; \Lambda^{p,0}) \to \mathcal  C^\infty(\Omega; \Lambda^{p,1}) \right]. $$

That is, $H^q(\Omega; \mathcal S^p)$ is isomorphic to $H^{p,q}_{\mathcal C^\infty}(\Omega; \mathcal V)$. We note that, in this context, we also have that $\dext' : \mathcal E' (\Omega; \Lambda^{p,q}) \to \mathcal E' (\Omega; \Lambda^{p,q+1})$ has closed range. We are going to show that, under certain conditions, we have similar results in the context of hypocomplex structures. In order to do this, we need some technical results.

We start with some remarks. If $Y \subset \Omega$ is open, the space $S^q(Y)$ of sections over $Y$ is a closed subspace of $\mc C^q(Y)$ and thus an ({\bf{FS}}) space. If $Y'\subset Y$ is also open and with compact closed contained in $Y$, then the restriction map $S^q(Y) \to S^q(Y')$ is compact: this is a consequence of \cite[Corollary III.5.5]{treves1992hypo}. If now $K \ssubset \Omega$ is compact, then $S^q(K)$ denotes the inductive limit of the spaces $S^q(Y)$ when $Y$ runs over the set of all open neighborhoods of $K$. This is a ({\bf{DFS}}) space. If $K'$ is a compact subset of the interior of $K$, then the natural map $S^q(K) \to S^q(K')$ is also compact.

Let $\frk K$ be a cover of $\Omega$ satisfying the following properties:

\begin{itemize}
\item $\frk K$ is countable, with elements indexed as $\frk K = \{K_j\}_{j \in \N}$;
\item $\frk K$ is locally finite;
\item Each $K \in \frk K$ is a compact set of $\Omega$.
\end{itemize}

For $q \in \Z_+$, let $\sigma = (K_{j_0}, \ldots, K_{j_q})$ be a $q$-simplex of $\frk K$, that is, an ordered collection of $q+1$ sets of $\frk K$ such that $|\sigma| \doteq K_{j_0} \cap \ldots \cap K_{j_q} \neq \emptyset.$ Sometimes we denote the simplex $\sigma$ just by the indexes, that is $\sigma = (j_0, \ldots, j_q)$.% The set $|\sigma|$ is called the \textit{support} of $\sigma$.

We denote by $N^q(\frk K)$ the set of all $q$-simplexes and by $N(\frk K) = \bigcup_{q \in \Z_+} N^q(\frk K)$ the nerv of $\frk K$. %We denote by $\mathcal F$ a sheaf over $\Omega$.
We recall that for each $q \in \Z_+$, a $q$-cochain of $N(\frk K)$ with values in $\mathcal S^p$ is a function $f$ such that, for each $q$-simplex $\sigma$, there is an associated local section $f_\sigma \in \mathcal S^p(|\sigma|)$. We denote by $C^q(\frk K, \mathcal S^p)$ the set of all $q$-cochains with values in $\mathcal S^p$.

The coboundary operators $\delta^q : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)$, $q \in \Z_+$, are defined by
$$ (\delta^q f)_\sigma = \sum_{j=0}^{q+1}(-1)^j \rho^{|\sigma_j|}_{|\sigma|} f_{\sigma_j},$$
in which $\sigma_j \doteq (U_0, \ldots, \hat {U_j}, \ldots, U_{q+1} )$ and the mapping $\rho^{|\sigma_j|}_{|\sigma|}$ associates each $p$-form in $|\sigma_j|$ to its restriction to $|\sigma|$. By definition, we have that $\delta^{q+1} \circ \delta^{q} = 0$ for all $q \in \Z_+.$

We define the cohomology of the complex $\delta^q : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)$, $q \in \Z_+$, for $q \geq 1$, as

\begin{equation}
\label{eq:chech_coho}
\check H^q(\frk K, \mathcal S^p) = \frac{ \ker \left[ \delta^q : C^q(\frk K, \mathcal S^p) \to C^{q+1}(\frk K, \mathcal S^p)\right] }{ \img \left[ \delta^{q-1} : C^{q-1}(\frk K, \mathcal S^p) \to C^{q}(\frk K, \mathcal S^p)\right] },
\end{equation} and, for $q = 0$, as
\begin{equation}
\label{eq:chech_coho_}
\check H^0(\frk K, \mathcal S^p) = \ker \left[ \delta^0 : C^0(\frk K, \mathcal S^p) \to C^{1}(\frk K, \mathcal S^p)\right] = \mathcal S^p(\Omega).
\end{equation} We defined in \eqref{eq:chech_coho} and \eqref{eq:chech_coho_} the \emph{\v Cech cohomology of $\frk K$ with values in $\mathcal S^p$}.

We denote by $\mathcal C^q_c(\frk K, \mathcal S^p)$ the set of all \emph{finite} $q$-cochains with values in $\mathcal S^p$, that is, for a given $f \in \mathcal C^q_c(\frk K, \mathcal S^p)$, there is only a finite number of $q$-simplexes of $\frk K$ such that $f_\sigma$ is non-zero. We clearly have $\delta^q( C^q_c(\frk K, \mathcal S^p) ) \subset C^{q+1}_c(\frk K, \mathcal S^p)$ for all $q \in \Z_+$, and so we have a complex whose cohomology is denoted by $\check H^q_c(\frk K, \mathcal S^p)$ for all $q$. And now we have what we call \emph{\v Cech cohomology of $\frk K$ with values in $\mathcal S^p$ with compact support}.

We note that $C^q_c(\frk K; \mathcal S^p)$ is a closed subspace of a direct sum of ({\bf DFS}) spaces and so it is also a ({\bf DFS}) space. Moreover, since $\delta^q$ is a linear continuous map between ({\bf DFS}) spaces, each $\ker \delta^q$ is also a ({\bf DFS}) space.



Let $A \subset \N$ be a finite subset. We denote by $C^q_A(\frk K; \mathcal S^p)$ the set of all cochains $s \in C^q_c(\frk K; \mathcal S^p)$ such that $s_{j_0 j_1 \ldots j_q} = 0$ if $\{j_0, j_1, \ldots, j_q\} \cap A = \emptyset.$

Since $\delta^q( C^q_A(\frk K; \mathcal S^p)) \subset C^{q+1}_A(\frk K; \mathcal S^p)$ we have a well defined \emph{complex of cochains with supports contained in $A$}. The corresponding cohomology spaces are denoted by $H^q_A(\frk K; \mathcal S^p)$ with $q = 0, 1, \ldots$. We have natural homomorphisms
$$ H^q_A(\frk K; \mathcal S^p) \to H^q_B(\frk K; \mathcal S^p) $$ if $A \subset B$ and clearly $$ H^q_A(\frk K; \mathcal S^p) \to H^q_c(\frk K; \mathcal S^p).$$

\begin{prp}
\label{hypo:aprime} Suppose that $\Omega$ is endowed with a hypocomplex involutive structure $\mathcal V$. For every finite subset $A$ of $\N$, there is another finite subset $A'$ of $\N$ with $A \subset A'$ such that the kernel of the homomorphism $H^1_A(\frk K; \mathcal S^p) \to H^1_c(\frk K; \mathcal S^p)$ is contained in the kernel of the homomorphism $H^1_A(\frk K; \mathcal S^p) \to H^1_{A'}(\frk K; \mathcal S^p)$.
\end{prp}

\begin{proof}
Let $L \subset \Omega$ be a compact such that $Y \doteq \Omega \bs L$ is connected and $\bigcup_{j \in A} K_j \subset L$. We define
$ A' = \{ j \in \N : K_j \cap L \neq \emptyset \}.$
Since $\frk K$ is locally finite, we have that $A'$ is finite. We also have, by the choice of $L$, that $A \subset A'$.

Let $s \in C^1_A(\frk K; \mathcal S^p)$ be such that $\delta^1 u = s$ for some $u \in C^0_c(\frk K; \mathcal S^p)$.
We write $u = \{u_j\}$ with $u_j \in \mathcal S^p(K_j)$.
We have $u_j - u_k = s_{jk}$ as elements in $\mathcal S(K_j \cap K_k)$ if $K_j \cap K_k \neq \emptyset.$ Let $p \in Y$ and assume that $p \in K_j \cap K_k$.
Notice that $\{j,k\} \cap A = \emptyset$  implies $s_{jk} = 0$ and consequently the germs of $u_j$ and $u_k$ coincide at $p$. Since $\VV$ is hypocomplex, we have that there is $f \in \mathcal S^p(Y)$ such that the germs of $f$ and $u_j$ coincide at $p$ if $p \in K_j$. Since all but a finite number of the $u_j$'s are zero, it follows that $f$ vanishes in an open neighborhood of $\del \Omega$ and thus in $Y$.
In particular, $u_j = 0$ if $K_j \subset Y$, that is, $u_j =0$ if $j \notin A'$. % \todo[inline]{Is it here that it is necessary to assume that $\Omega$ is not compact?}
\end{proof}


\begin{prp}
\label{hypo:rho1_injective} Let $\frk L = \{L_j\}$ be a countable and locally finite refinement of $\frk K$ with each $L_j$ compact. Then, the refinement homomorphism
$$ \rho^q : C^q_c(\frk K; \mathcal S^p) \to C^q_c(\frk L; \mathcal S^p), \qquad q = 0, 1, 2 \ldots $$
induces homomorphisms
$$ \rho^q_* : H^q_c(\frk K; \mathcal S^p) \to H^q_c(\frk L; \mathcal S^p), \qquad q = 0, 1, 2 \ldots $$
and $\rho^1_*$ is injective.
\end{prp}

% \begin{que} Can I prove that $\rho^q_*$ is injective for $q > 1$?
% \end{que}

\begin{proof}
Let $ \gamma : \N \to \N$ be such that $L_j \subset K_{\gamma(j)}$ for every $j$. Let $ s = \{s_{jk}\} \in C^1_c(\frk K; \mathcal S^p)$ satisfying $\delta^1 s = 0$ and suppose that $\rho^1 s = \delta^0 v$ for some $v = \{v_j\} \in C^0_c(\frk L; \mathcal S^p).$ Then
$ v_k - v_j = s_{\gamma(j) \gamma(k)}$
as elements of $ \mathcal S^p(L_j \cap L_k) $ and, since $s$ is a cocycle, we have that $s_{kr} - s_{jr} + s_{jk} = 0$ as elements of $\mathcal S^p(K_j \cap K_k \cap K_r)$ and consequently
$$ v_k + s_{\gamma(k)r} = v_j + s_{\gamma(j)r}$$
as elements of $\mathcal S^p(L_j \cap L_k \cap K_r)$. Notice that the left hand side does not depend on $j$ and the right hand side does not depend on $k$. By varying $j$ and $k$, we see that there is $u_r \in \mathcal S^p(K_r)$ such that $u_r = v_j + s_{\gamma(j)r}$ as elements of $\mathcal S^p(L_j \cap K_r)$ whenever $K_j \cap K_r \neq \emptyset.$

Let $I,J \subset \N$ be such that $v_j = 0$ unless $j \in I$ and $s_{jk} = 0$ unless $j$ and $k$ belong to $J$. The set $I' \doteq J \cup \left\{ r \in \N : \left( \bigcup_{j \in I} L_j \right) \cap K_r \neq \emptyset\right\}$
is finite and $u_r = 0$ if $r \notin I'$. Indeed, if $r \notin I'$, then $r \notin J$ and, if $j$ is such that $L_j \cap K_r \neq \emptyset$, then $j \notin I$. These two facts imply $u_r = 0$ in $K_r \cap L_j $. Thus $u \doteq \{u_j\}$ belongs to $C^0_c(\frk K; \mathcal S^p)$. Finally, as elements of $\mathcal S^p(L_j \cap K_r \cap K_t)$, we have
$$ u_r - u_t = (v_j + s_{\gamma(j)r}) - (v_j + s_{\gamma(j)t}) = s_{\gamma(j)r} - s_{\gamma(j)t} = - s_{tr}.$$ And the proof is completed. \end{proof}

From now, on we assume that $\frk K$ and $\frk L$ satisfy the following properties:

\begin{equation}
\label{hypo:p1} L_j \subset \operatorname{int}(K_j) \text{ for all } j \in \N.
\end{equation}
\begin{equation}
\label{hypo:p2}
\text{\parbox{.85\textwidth}{ If $(j_0, j_1)$ is a 1-simplex for $\frk K$, then it is also a 1-simplex for $\frk L$. And if $(j_0, j_1, j_2)$ is a 2-simplex for $\frk K$, then it is also 2-simplex for $\frk L$.}}
\end{equation}

For this, it suffices to take $\frk L$ to be a locally finite countable covering of $\Omega$ such that each $K_j$ is compact and $\frk K = \{K_j\}$ is the covering defined by
$$ K_j = \{ p \in \Omega : \operatorname{dist}(p, L_j) \leq \epsilon_j\}.$$

It is clear that $\frk K$ also is locally finite and countable and that each $K_j$ is compact if $\epsilon_j > 0$ is chosen suitable small.


% In order to prove this result we need some intermediate results.

% We are going to assume that $\Omega$ is not compact.



Notice that Property \eqref{hypo:p2} guarantees that the maps $\rho^p$ are injective for $p = 0, 1, 2$. Moreover, if $A \subset \N$ is finite, then $A$ induces homomorphisms
$$ \rho^p_A : C^p_A(\frk K; \mathcal S^p) \to C^p_A(\frk L; \mathcal S^p)$$
which are now, thanks to Property \eqref{hypo:p1}, compact operators.



\begin{thm}
\label{hypo:thm:dfstop} Assume that $\Omega$ is endowed with a hypocomplex structure. The map $$ \delta^0 : C^0_c(\frk K; \mathcal S^p) \to C^1_c(\frk K; \mathcal S^p) $$ has closed range. % and thus $H^1_c(\frk K, \mathcal S^p)$ has a natural topology of DFS spaces.
\end{thm}

\begin{proof} By Theorem 6' of \cite{komatsu1967projective}, it suffices to show that $\img(\delta^0) \cap C^1_A(\frk K; \mathcal S^p)$ is closed in $C^1_A(\frk K; \mathcal S^p)$ for all finite subsets $A \subset \N.$

Let $A \subset \N$ be finite and let $A'$ be as in Proposition \ref{hypo:aprime}. We define the following ({\bf DFS}) spaces:
$$ V \doteq \{ (u,s) \in C^0_{A'}(\frk K; \mathcal S^p) \times C^1_{A}(\frk K; \mathcal S^p): \delta^0 u = s\},$$
$$ W \doteq \{ (u,s) \in C^0_{A'}(\frk L; \mathcal S^p) \times C^1_{A}(\frk K; \mathcal S^p): \delta^0 u = \rho^1s\},$$
and let $\sigma : V \to W$ be the linear map given by $ \sigma(u, s) = (\rho^0_{A'}u, s).$

We need the following lemma:

\begin{lem}  Assume that $\Omega$ is endowed with a hypocomplex structure. The map $\sigma$ is a bijection.
\end{lem}
\begin{proof}
Since $\delta^0$ is injective, we have that $\sigma$ is injective. In fact, if $\sigma(u,s) = (0,0)$, then $s = 0$ and, since $(u,s) \in V$ we have $\delta^0u = 0$.

Now we are going to prove that $\sigma$ is surjective. Let $(v,s) \in W$. We have that $\delta^1(\rho^1 s) = \delta^1(\delta^0 v) = 0$ and, since $\rho^2(\delta^1 s) = \delta^1(\rho^1 s) = 0 $ and $\rho^2$ is injective, it follows that $\delta^1 s = 0$. Hence, the class of $s$ defines an element in $H^1_A(\frk K; \mathcal S^p)$ which belongs to the kernel of $\rho^1_*$.
By Proposition \ref{hypo:rho1_injective}, the class of $s$ vanishes in $H^1_c(\frk K; \mathcal S^p)$ and so Proposition \ref{hypo:aprime} implies that the class of $s$ vanishes in $H^1_{A'}(\frk K; \mathcal S^p)$. In other words, there is $u \in C^1_{A'}(\frk K; \mathcal S^p)$ such that $(u,s) \in V$.
To finish the proof, we need to show that $\sigma(u,s) = (v,s)$. This follows from the facts that $\delta^0(v - \rho^0_{A'}u) = 0$ and that $\delta^0$ is injective.
\end{proof}
We denote by $E$ the ({\bf DFS}) space $C^0_{A'}(\frk L; \mathcal S^p) \times C^1_A(\frk K; \mathcal S^p)$; we remark that $W$ is a closed subspace of $E$ and thus also a ({\bf DFS}) space. Let $\imath$ be the inclusion map $W \subset E$. It follows that $\imath \circ \sigma : V \to E$ is a topological embedding.

We introduce the following continuous linear maps
 $$ \tau_1(u,s) = (\rho^0_{A'}, 0), \qquad \tau_2(u,s) = (0,s).$$

Since $\tau_1$ is compact and $\tau_2 = \imath \circ \sigma - \tau_1$, it follows from Theorem 1 of \cite{schwartz1956} that $\tau_2$ has closed range in $E$. This is the same as saying that the map $p_2 : V \to C^1_A(\frk K; \mathcal S^p)$, given by the projection on the second factor, has closed range, but according to Proposition \ref{hypo:aprime} we have
$$ \img{p_2} = \img(\delta^2) \cap C^1_A(\frk K; \mathcal S^p),$$
which completes the proof.
\end{proof}



\begin{thm}
\label{thm:closed_range} Let $\Omega$ be orientable and endowed with a hypocomplex structure $\mathcal V$. Assume that the equivalent conditions in Proposition \ref{prp:equiv} hold for every point of $\Omega$. Then % for each $p = 0, 1, \ldots, m$ the natural homomorphism
%$$ \alpha : H^1_c(\Omega; \mathcal S^p) \to H^{1}(\mathcal E'(\Omega; \Lambda^{p,*}))$$
%is an isomorphism and consequently
\begin{equation}
\label{hypo:eq:dprimecpctsupp} \dext' : \mathcal C^\infty (\Omega; \Lambda^{p,n-1}) \to \mathcal C^\infty (\Omega; \Lambda^{p,n})
\end{equation}
has closed range.
\end{thm}

We emphasize that we are not precluding that $\Omega$ has compact connected components.



\begin{proof}
According to \cite[Page 18]{kothe19679topological}, it suffices to show that $\dext' : \mathcal E' (\Omega; \Lambda^{m-p,0}) \to \mathcal E' (\Omega; \Lambda^{m-p,1})$ has strongly sequentially closed range. The argument follows by the conjunction of Remark \ref{rmk:1}, the proof of Theorem \ref{thm:first}, and Theorem \ref{hypo:thm:dfstop}.

Let $\{u_j\} \subset \mathcal E'(\omega; \Lambda^{m-p,0})$ be such that $\dext' u_j \to f$ in $E'(\omega; \Lambda^{m-p,1})$. Hence, there are a compact set $K \subset \Omega$ and a real number $s \in \R$ such that $\dext' u_j \in H^s(K, \Lambda^{m-p,1})$, for all $j$.

By the hypothesis and by Remark \ref{rmk:1}, there exists a covering $\frk U = \{K_j\}$ of $\Omega$ by compact sets such that $\{K_1, \ldots, K_\nu\}$ is a covering of $K$ and there exists an $s \in \R$ such that the following is true:

For every $l=1, \ldots, \nu$, there are $U_l \supset K_l$ open and $v_{l,j} \in H^t_{\tiny{loc}}(U_l; \Lambda^{m-p,0})$ such that $\dext' v_{l,j} = \dext' u_j$ in $U_l$ and $\{v_{l,j}\}_{j=1}^\infty$ is a Cauchy sequence if $H^t_{\tiny{loc}}(U_l; \Lambda^{m-p,0})$ (this last property follows from the proof of Proposition \ref{prp:equiv}).
We define $v_l = \lim_j v_{l,j} \in H^t_{\tiny{loc}}(U_l; \Lambda^{m-p,0}).$ For $l > \nu$ we have $\dext' u_j = 0$ for all $j$ and so we take $v_{l,j} = 0$.

Now, suppose that $K_{l_1} \cap K_{l_2} \neq \emptyset$. Then $\dext' (v_{l_1,j} - v_{l_2,j}) = 0$ in a neighborhood of $K_{l_1} \cap K_{l_2}$ and so $V_j = \{v_{l_1,j} - v_{l_2,j}\}$ defines, for each $j$, an element in $C^1(\frk U; \mathcal S^{m-p})$.

Moreover, a standard argument of comparison of topologies, taking into account the property of hypocomplexity, shows that $V_j \to V$ in $C^1(\frk U; \mathcal S^{m-p})$. We have that $V = \{v_{l_1} - v_{l_2}\}_{l_1, l_2}$. On the other hand, $W_j = \{v_{lj} - u_j\}_l \in C^0(\frk U; \mathcal S^{m-p})$ and $\delta_0 W_j = V_j \to V$.

By Theorem \ref{hypo:thm:dfstop}, there is $W \in C^0(\frk U; \mathcal S^{m-p})$ such that $\delta_0 W = V$. Now we write $W = \{w_l\} \in C^0(\frk U; \mathcal S^{m-p})$, and then we obtained
$w_{l_1} - w_{l_2} = v_{l_1} - v_{l_2}$ near $K_{l_1} \cap K_{l_2}$. Now we define $u$ by setting $u = v_l - w_l$ near $K_l$ and we have $d'u = d'v_l = f$ near $K_l$. By construction, $u$ has compact support and the proof is completed.
% Let $f^j \in \dext'(\mathcal E'(\omega; \Lambda^{m-p,0}))$ be a sequence converging to $f \in \mathcal E'(\omega; \Lambda^{p,1})$. We write $u^j \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u^j = f^j$. We want to show that there exists $u \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u = f$.
%
% Now we are going to construct a special covering for $\Omega$. Let $M$ be such that $f \in H^{-M}(\omega; \Lambda^{p,1})$. By following the same notation from the previous lemma, for each $x \in \Omega$, there exists a compact set $K(x) = \overline{U_{l_x + 1}(x)} \subset \omega'(x) \subset \omega(x)$ such that, for every $w \in  Z^{p,1}_c(\omega(x)) \cap H^{-M}(\omega(x); \Lambda^{p,1})$, there exists a $u \in  \mathcal D'(\omega'(x); \Lambda^{p,0}) \cap H^{-l_x}(\omega'(x); \Lambda^{p,0})$ satisfying
% $$\dext' u = w$$ on $\omega'(x)$ and satisfying $$ \|u\|_{H^{-l_x}(\omega'(x))} \leq C(x) \|w\|_{H^{-M}(\omega(x))}.$$
%
% Therefore, we have a covering $\frk U' = \{K(x)\}$ of $\Omega$ by compacts. We take a subcover $\frk U$ of $\frk U'$ being locally finite and countable. The elements of $\frk U$  be denoted by $\frk U = \{K(x_j)\}$. We simplify the notation by writing $K_j = K(x_j)$, $\omega'_j = \omega'(x_j)$, $\omega_j = \omega(x_j)$, and $C_j = C(x_j)$. Let $K$ be a compact such that $\operatorname{supp} f^j \in K$ for all $j$. Notice that only a finite number of elements of $\frk U$ intercept $K$.
% Therefore, we take  $C = \max \{C_j: K_j \cap K \neq \emptyset \}$ and $L = \max \{l_{x_j} : K_j \cap K \neq \emptyset \}$.
%
%
%
%
% For each $k$, there exists $v^j_k \in \mathcal D'(\omega'_k; \Lambda^{p,0})$ such that $\dext' v^j_k = f^j|_{\omega_k}$ on $\omega'_k$ and satisfying the estimates
% \begin{equation}
% \label{hypo:ineq_sol}
%  \| v^j_k \|_{H^{-L}(\omega'_k)} \leq C \|f^j\|_{H^{-M}(\omega_k)}.
% \end{equation}
%
% We take $v^j_k = 0$ if $f^j|_{\omega_k} = 0$.
%
% If $k , l$ are such that $K_k \cap K_l \neq \emptyset$, then $\dext' [v^j_k - v^j_l] = 0$ in $K_k \cap K_l$ which means that $v^j_k - v^j_l \in \mathcal S^p(K_k \cap K_l)$. Therefore, it is defined a 1-cochain $g^j \in C^1(\mathfrak U; \mathcal S^p)$ such that, for each 1-simplex $\sigma = (K_k, K_l)$, we have $g^j_\sigma = (v^j_k - v^j_l) $. % Notice that if $\sigma = (K_k, K_l, K_o)$ is a 2-simplex, we have $$(\delta^1 g)_\sigma = \sum_{j=0}^1 (-1)^j \rho^{|\sigma_j|}_{|\sigma|} g_{|\sigma_j|} = (g_{K_k} - g_{K_l}) - (g_{K_l} - g_{K_o}) + (g_{K_l} - g_{K_o}) = 0.$$
%
% Notice that if we define $h^j_k = v^j_k - u^j$, then $h^j_k$ is in $\mathcal S^p(K_k)$ and then we have a 0-cochain $h^j \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$.
%
% Since $f^j$ is convergent, and therefore a Cauchy sequence, by the inequality $\eqref{hypo:ineq_sol}$, the sequence $\{v^j_k\}$ is also a Cauchy sequence and so it converges to a function $v_{k}$ in $\mathcal S^p(K_k \cap K_l$ and so $g^j$ converges to a 1-cochain $g \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$. By Theorem \ref{hypo:thm:dfstop}, $\delta^0$ has closed range and so there exists a 0-cochain
% $h \in C^0_c(\frk U; \mathcal S^p)$ such that $\delta^0(h) = g$. This means that $h_k - h_l = v_k - v_l$ in $K_k \cap K_l$ and that $v_k - h_k = v_l - h_l$. Thus, we can define $u \in \mathcal E'(\omega; \Lambda^{p,0})$ given by $u = v_k - h_k$ in $K_k$ for each $k$. Since $\dext' v^j_k = f^j$ for all $j$, we have $\dext' v_j = f$ and we also have $\dext' h_k = 0$. This means that $\dext' u = f$ in $K_k$ for every $k$.
\end{proof}


% To close this section, we state a Corollary from Proposition \ref{prp:equiv} that is going to be useful on the next chapter.

%\begin{thm}
%\label{thm:closed_range} Let $\Omega$ be endowed with a hypocomplex structure $\mathcal V$. Assume that the equivalent conditions in Proposition \ref{prp:equiv} hold for every point of $\Omega$. Then % for each $p = 0, 1, \ldots, m$ the natural homomorphism
%$$ \alpha : H^1_c(\Omega; \mathcal S^p) \to H^{1}(\mathcal E'(\Omega; \Lambda^{p,*}))$$
%is an isomorphism and consequently
%\begin{equation}
%\label{hypo:eq:dprimecpctsupp} \dext' : \mathcal E' (\Omega; \Lambda^{p,0}) \to \mathcal E' (\Omega; \Lambda^{p,1})
%\end{equation}
%has a strongly sequentially closed range.
%\end{thm}

% \begin{proof}[Proof of Theorem \ref{thm:closed_range}]

% Let $f^j \in \dext'(\mathcal E'(\omega; \Lambda^{p,0}))$ be a sequence of functions converging to $f \in \mathcal E'(\omega; \Lambda^{p,1})$. We write $u^j \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u^j = f^j$. We want to show that there exist $u \in \mathcal E'(\omega; \Lambda^{p,0})$ such that $\dext' u = f$.

% Now we are going to construct a special covering for $\Omega$. Let $M$ be such that $f \in H^{-M}(\omega; \Lambda^{p,1})$. By following the same notation from the previous lemma, for each $x \in \Omega$ there exist a compact set $K(x) = \overline{U_{l_x + 1}(x)} \subset \omega'(x) \subset \omega(x)$ for every $w \in  Z^{p,1}_c(\omega(x)) \cap H^{-M}(\omega(x); \Lambda^{p,1})$ there exist a $u \in  \mathcal D'(\omega'(x); \Lambda^{p,0}) \cap H^{-l_x}(\omega'(x); \Lambda^{p,0})$ satisfying $$\dext' u = w$$ on $\omega'(x)$ and satisfying $$ \|u\|_{H^{-l_x}(\omega'(x))} \leq C(x) \|w\|_{H^{-M}(\omega(x))}.$$

% Therefore, we have a covering $\frk U' = \{K(x)\}$ of $\Omega$ by compacts. We take a subcover $\frk U$ of $\frk U'$ being locally finite and countable. The elements of $\frk U$  be denoted by $\frk U = \{K(x_j)\}$. We simplify the notation by writing $K_j = K(x_j)$, $\omega'_j = \omega'(x_j)$ and $\omega_j = \omega(x_j)$ and $C_j = C(x_j)$. Let $K$ be a compact such that $\operatorname{supp} f^j \in K$ for all $j$. Notice that only a finite number of elements of $\frk U$ intercept $K$ and so we take  $C = \max \{C_j: K_j \cap K \neq \emptyset \}$ and $L = \max \{l_{x_j} : K_j \cap K \neq \emptyset \}$.




% For each $k$ there exist $v^j_k \in \mathcal D'(\omega'_k; \Lambda^{p,0})$ such that $\dext' v^j_k = f^j|_{\omega_k}$ on $\omega'_k$ and satisfying the estimates
% \begin{equation}
% \label{hypo:ineq_sol}
%  \| v^j_k \|_{H^{-L}(\omega'_k)} \leq C \|f^j\|_{H^{-M}(\omega_k)}.
% \end{equation}

% We take $v^j_k = 0$ if $f^j|_{\omega_k} = 0$.

% If $k , l$ are such that $K_k \cap K_l \neq \emptyset$, then $\dext' [v^j_k - v^j_l] = 0$ in $K_k \cap K_l$ which means that $v^j_k - v^j_l \in \mathcal S^p(K_k \cap K_l)$. Therefore, it is defined a 1-cochain $g^j \in C^1(\mathfrak U; \mathcal S^p)$ such that for each 1-simplex $\sigma = (K_k, K_l)$, we have $g^j_\sigma = (v^j_k - v^j_l) $. % Notice that if $\sigma = (K_k, K_l, K_o)$ is a 2-simplex, we have $$(\delta^1 g)_\sigma = \sum_{j=0}^1 (-1)^j \rho^{|\sigma_j|}_{|\sigma|} g_{|\sigma_j|} = (g_{K_k} - g_{K_l}) - (g_{K_l} - g_{K_o}) + (g_{K_l} - g_{K_o}) = 0.$$

% Notice that if we define $h^j_k = v^j_k - u^j$ then $h^j_k$ is in $\mathcal S^p(K_k)$ and then we have a 0-cochain $h^j \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$.

% Since $f^j$ is convergent, and therefore a Cauchy sequence, by the inequality $\eqref{hypo:ineq_sol}$ the sequence $\{v^j_k\}$ also is a Cauchy sequence and so it converges to a function $v_{k}$ in $\mathcal S^p(K_k \cap K_l$ and so $g^j$ converge to a 1-cochain $g \in C^1_c(\frk U; \mathcal S^p)$ such that $\delta^0(h^j) = g^j$. By Theorem \ref{hypo:thm:dfstop}, $\delta^0$ has closed range, and so there exist a 0-cochain $h \in C^0_c(\frk U; \mathcal S^p)$ such that $\delta^0(h) = g$. This means that $h_k - h_l = v_k - v_l$ in $K_k \cap K_l$. This mean that $v_k - h_k = v_l - h_l$ and so we can define $u \in \mathcal E'(\omega; \Lambda^{p,0})$ given by $u = v_k - h_k$ in $K_k$ for each $k$. Since $\dext' v^j_k = f^j$ for all $j$ we have $\dext' v_j = f$ and we also have $\dext' h_k = 0$ this means that $\dext' u = f$ in $K_k$ for every $k$.
% \end{proof}

% \begin{rmk}
% Notice that under the same hypothesis as Theorem \ref{thm:closed_range} we conclude that
% \begin{equation}
% \label{hypo:eq:dprimecpctsuppsmooth} \dext' : \mathcal C^\infty (\Omega; \Lambda^{p,0}) \to \mathcal C^\infty (\Omega; \Lambda^{p,1})
% \end{equation}
% has closed range for all $p$.
%
% \end{rmk}

%\subsection{Involutive structures on \texorpdfstring{$SU(3)$}{SU(3)}}

%\section{The compact case}




%\begin{cor}
%\label{prp:finite_dim} Let $\Omega$ be a compact manifold endowed with a %hypocomplex structure $\mathcal V$. Assume that the equivalent conditions in %Proposition \ref{prp:equiv} hold for every point of $\Omega$. Then the kernel %of the map % for each $p = 0, 1, \ldots, m$ the natural homomorphism
%%$$ \alpha : H^1_c(\Omega; \mathcal S^p) \to H^{1}(\mathcal E'(\Omega; %\Lambda^{p,*}))$$
%%is an isomorphism and consequently
%\begin{equation}
% \dext' : \mathcal E' (\Omega; \Lambda^{p,0}) \to \mathcal E' (\Omega; %\Lambda^{p,1})
%\end{equation}
%has finite dimension.
%\end{cor}




\section{Serre duality}

% In this section, we  recall some conditions under the involutive structure $\mathcal V$, which we assume to be hypocomplex, and the manifold $\Omega$ and for certain integers $p$ and $q$ so that we have the following isomorphisms
% $$  H^{p,q}_{\mathcal C^\infty}(\Omega; \mathcal V) \cong  H^{p,q}_{\mathcal D'}(\Omega; \mathcal V)$$
% and
% $$  H^{p,q}_{\mathcal C^\infty_c}(\Omega; \mathcal V) \cong  H^{p,q}_{\mathcal E'}(\Omega; \mathcal V). $$ The main reference for this section is \cite{serre1955theoreme}.

% First we suppose that $q = 0$ and that we have $u \in \mathcal D'(\Omega; \Lambda^{p,0})$  such that $\dext' u = 0$. Since we are assuming that $\mathcal V$ is hypocomplex we have that $u \in \mathcal C^\infty(\Omega; \Lambda^{p,0})$. Then:

% $$  H^{p,0}_{\mathcal D'}(\Omega; \mathcal V) = \mathcal S^p(\Omega) =   H^{p,0}_{\mathcal C^\infty}(\Omega; \mathcal V).$$

% If $\Omega$ is compact, then clearly $ \mathcal C^\infty_c =  \mathcal C^\infty$ and $\mathcal D' = \mathcal E'$ and we have the desired isomorphisms. If $\Omega$ is not compact, by using the analytic continuation property we also obtain:

% $$  H^{p,0}_{\mathcal E'}(\Omega; \mathcal V) = 0 =   H^{p,0}_{\mathcal C^\infty_c}(\Omega; \mathcal V).$$


%As we saw in the beginning of this chapter, the set $\mathcal C^\infty(\Omega;\Lambda^j)$ has a topology of a Fréchet space and its topological dual can be identified with $\mathcal E'(\Omega;\Lambda^{N-j})$. This identification is given by the following map:

% Let $u \in \mathcal E'(\Omega; \Lambda^{N-j})$ and $v \in \mathcal  C^\infty(\Omega; \Lambda^j)$. We have that $u \wedge v$ is a current of degree $N$ and so it can be integrated over $\Omega$. Therefore we can define

%$$T_u(v) = (u \wedge v)(1)$$
%and clearly if $u$ has smooth coefficients what we are doing is
%$$ T_u(v) = \int_\Omega  u \wedge v.$$

%We clearly can identify $\mathcal C^\infty(\Omega; \Lambda^{p,q})$ with a closed subspace of $\mathcal C^\infty(\Omega; \Lambda^{p+q})$ and therefore it also has a structure of a Fréchet space.

%By the Hahn-Banach Theorem we have that the map $$v \in \mathcal E'(\Omega; \Lambda^{N-p-q}) \mapsto T_v \in \mathcal C^\infty(\Omega; \Lambda^{p,q})^*$$ and since we can decompose $\mathcal E'(\Omega; \Lambda^{N-p-q}) = \bigoplus_{i+j = N - p - q} \mathcal E'(\Omega; \Lambda^{i,j})$ and $u \wedge v = 0$ when $u \in \mathcal E'(\Omega; \Lambda^{i,j})$ and $v \in \mathcal C^\infty(\Omega; \Lambda^{p,q}) $ and $(i,j) \neq (m-p, n - q)$ and so we obtain:

% \begin{prp}
% The map $v \in \mathcal E'(\Omega; \Lambda^{N-j}) \mapsto T_v \in \mathcal C^\infty(\Omega; \Lambda^j)^*$ is an isomorphism.
% \end{prp}

% Now we want to study the transpose of the operator $$\dext' : \mathcal C^\infty(\Omega; \Lambda^{p,q}) \to \mathcal C^\infty(\Omega; \Lambda^{p,q+1}).$$

% \begin{prp}
% The following diagram is commutative
% $$
% \xymatrix@+2pc{
%  \mathcal E'(\Omega; \Lambda^{m-p,n-q-1}) \ar[r]^{(-1)^{p+q}\dext'} \ar[d]_{}& \mathcal E'(\Omega; \Lambda^{m-p,n-q}) \ar[d]^{} \\
%  \mathcal C^\infty(\Omega; \Lambda^{p,q+1})^* \ar[r]_{\dext'^t} &  \mathcal C^\infty(\Omega; \Lambda^{p,q})^*
% }
% $$
% with the vertical arrows denoting the isomorphism $v \mapsto T_v.$
% \end{prp}

% \begin{proof} This is a simple application of Stokes' theorem.
% \end{proof}

We recall some basic facts about Fréchet spaces. We remember that, if $E$ and $F$ are Fréchet spaces and $u : E \to F$ is a linear continuous map, we say that $u$ is a homomorphism if $u(E)$ is closed. By the Open Mapping Theorem, we have that $u$ is a homomorphism if and only if $u': E / \ker u \to F$ is an isomorphism.

The following result is important for us:

\begin{prp}
\label{prp:finite_dim_and_closedness} Let $E$ and $F$ be Fréchet spaces and $u : E \to F$ be a linear continuous map. If the codimension of $u(E)$ is finite, then $u$ is a homomorphism.
\end{prp}

\begin{prp} Let $E$, $F$ and $G$ be Fréchet spaces. Consider the mappings
$$ E \xrightarrow{u} F \xrightarrow{v} G .$$ We assume that $u$ and $v$ are homomorphism and that $u(E) \subset \ker v$. Then $ \ker v / u(E) $ is a Fréchet space and we have a canonical isomorphism
$$ \left( \frac{\ker v}{u(E)} \right)^* \cong \frac{ \ker u^t}{v^t(G^*)} .$$
\end{prp}

Combining the results above with the discussion that precedes Theorem 2.2.3, we obtain the following version of Serre's duality theorem:

\begin{thm}
\label{chp:inv:thm:serre_duality}
Suppose that $\Omega$ is orientable and that the following linear maps are homomorphisms
$$ \mathcal C^\infty(\Omega; \Lambda^{p,q-1}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q}) \xrightarrow{\dext'} \mathcal C^\infty(\Omega; \Lambda^{p,q+1}).$$
Then $ H^{p,q}_{\mathcal C^\infty}(\Omega;\mathcal V)$ is a Fréchet space and there is a canonical isomorphism
$$  H^{p,q}_{\mathcal C^\infty}(\Omega; \mathcal V)^* \cong  H^{m-p,n-q}_{\mathcal E'}(\Omega; \mathcal V).$$
\end{thm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HODGE DECOMPOSITION %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Hodge decomposition}
\label{sec:hodge_theory}

In this section, we are going to explain how to use the Hodge decomposition for the operator $\dext'$. With this decomposition, we are going to find some simple conditions so that the cohomology is finite dimensional on a specific degree. Usually, Hodge decomposition is introduced in the context of elliptic differential operators between Hermitian vector bundles. Here we made a small improvement: we assumed that the operator is subelliptic. See Definition \ref{dfn:subellipticity_and_stuff}.

Suppose that $\Omega$ is a compact manifold with a positive $\mathcal C^\infty$-density $\mu$ and let $E_j$, for $j = 1, 2, 3$ be three Hermitian vector bundles over $\Omega$. We denote by $\ip{,}_j$ the hermitian inner product on $E_j$.
Let $$A_j : \mathcal C^\infty(\Omega; E_j) \to \mathcal C^\infty(\Omega; E_{j+1}), \qquad j = 1, 2$$ be partial differential operators of order $m$ satisfying $A_2 \circ A_1 = 0$. That is, we have
$$ \mathcal C^\infty(\Omega; E_1) \xrightarrow{A_1}{} \mathcal C^\infty(\Omega; E_{2})  \xrightarrow{A_2}{}  \mathcal C^\infty(\Omega; E_3).$$

We endow $\mathcal C^\infty(\Omega; E_j)$ with the inner product
$$\iip{u,v}_j \doteq \int_\Omega \ip{u(x),v(x)}_j \dint \mu(x),$$
for $u, v \in \mathcal C^\infty(\Omega; E_j)$, and we define the operators $A_j^* : \mathcal C^\infty(\Omega; E_{j+1}) \to \mathcal C^\infty(\Omega; E_{j})$ by
$$ \iip{A_j u, v }_{j+1} = \iip{u, A^*_j v}_{j+1},$$
for $u \in \mathcal C^\infty(\Omega; E_{j})$ and $v \in \mathcal C^\infty(\Omega; E_{j+1}).$

Now we have everything we need to introduce the Hodge operator:

\begin{dfn}
For $u \in \mathcal C^\infty(\Omega; E_2)$, we define $\Box u \doteq (A_1 A_1^* + A_2^* A_2) u$ and, in the sense of distributions, we define $$D(\Box) = \{u \in L^2(\Omega; E_2): \Box u \in L^2(\Omega; E_2) \}.$$ The operator $$\Box : D(\Box) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ is densely defined and is called \emph{Hodge operator}, \emph{Hodge Laplacian} or just \emph{Box operator}.
\end{dfn}

% because $\mathcal C^\infty(\Omega; E_2) \subset D(\Box)$ is a dense subset of $L^2(\Omega; E_2)$.

The operator $\Box$ has closed graph. In fact, let $u_j, v_j \in L^2(\Omega; E_2)$ be a sequence satisfying $\Box u_j = v_j$ and suppose that $u_j \to u \in L^2(\Omega; E_2)$ and $v_j \to v \in L^2(\Omega; E_2)$.
We want to show that $u \in D(\Box)$ and $\Box u = v$. Since $u_j \to u$ and $v_j \to v$ in $L^2(\Omega; E_2)$, we have this convergence in $\mc D'(\Omega; E_2)$ and, since $\Box$ is a differential operator, it is continuous in $\mc D'(\Omega; E_2)$. Thus, we can apply the Closed Graph Theorem and conclude that $\Box u = v$ in the sense of distributions. By hypothesis, we have $u,v \in L^2(\Omega; E_2)$ and so $u \in D(\Box)$.

We also remark that
$$
\begin{aligned}
\iip{\Box u, u}
	& = \iip{A_1 A_1^*u, u} + \iip{A_2^* A_2u, u} \\
	& = \iip{A_1^*u, A_1^*u} + \iip{A_2 u, A_2 u} \\
	& = \|A_1^*u\|_1^2 + \|A_2 u\|_3^2
\end{aligned}
$$
and so we have the following result:

\begin{prp}
\label{prp:kernel_Box_decomposition} The kernel of the operator $\Box$ is
$$ \ker \Box = \{u \in L^2(\Omega; E_2): A_1^*u = 0 \text{ and } A_2 u = 0\}. $$
\end{prp}

In the following definition, we introduce two concepts regarding the regularity of differential operators. Under certain conditions, these concepts provide sufficient conditions so that the kernel of the differential operator has finite dimension.

\begin{dfn}
\label{dfn:subellipticity_and_stuff} Let $E$ be a vector bundle over $\Omega$ and consider a linear partial differential operator $P : \mc D' (\Omega; E) \to \mc D'(\Omega; E)$. For an $\epsilon > 0$, the operator $P$ is said to be \emph{$\epsilon$-subelliptic} if $Pu \in H^s(\Omega;E)$ implies that $u \in H^{s+\epsilon}(\Omega; E)$ for all $u \in H^s(\Omega; E)$.
The operator $P$ is said to be \emph{globally hypoelliptic} if, given $u \in \mc D'(\Omega; E)$ such that $Pu \in \mathcal C^\infty(\Omega;F)$, it holds that $u \in \mathcal C^\infty(\Omega;E)$.
Notice that subellipticity implies global hypoellipticity.
\end{dfn}

On the above definition, it is not necessary to assume that the manifold $\Omega$ is compact.

The following proposition is a well known result about differential operators on compact manifolds.

\begin{prp} If $P : \mc D' (\Omega; E) \to \mc D'(\Omega; F)$ is globally hypoelliptic, then $$\dim \ker P < \infty.$$
\end{prp}

\begin{proof}
Since $P$ is globally hypoelliptic, we have that $\ker P \subset \mathcal C^\infty(\Omega; E)$. Consider $\ker P$ with the topology induced by $L^2(\Omega; E)$. Notice that this induced topology agrees with the topology induced by $H^s(\Omega; E)$ for any $s \in \R$. Take $B = \{ u \in \ker P: \|u\|_1 \leq 1 \}$ and note that $B$ is closed and bounded. By the Rellich lemma, we know that the inclusion $H^1(\Omega; E) \to H^0(\Omega; E) = L^2(\Omega; E)$ is compact and so $B$ is compact.
\end{proof}

In this work, we are interested in the case in which $P$ is the Hodge operator. Therefore, we need to establish some conditions so that the Hodge operator is globally hypoelliptic. But first we need to finish our decomposition. We need the next lemma which is a basic result on Hilbert spaces.

%\begin{lem}
%Let $H_1$ and $H_2$ be Hilbert spaces with norms $\|.\|_1$ and $\|.\|_2$. If $T : H_1 \to H_2$ is a linear, closed and densely defined operator such that there is a constant $C > 0$ such that
%$$\|f\|_1 \leq C \|Tf\|_2$$
%for all $ f \in D(T) \cap \overline{\img(T^*)}$,
%then $\img(T)$ is closed.
%\end{lem}
%
%\begin{proof}
%Let $f_k \in \img(T)$ such that $f_k \to f$ in $H_2$. We want to show that there exist $g \in D(T)$ satisfying $Tg = f$. Let $g_k \in D(T)$ with $Tg_k = f_k$. Since $\ker T^\perp = \overline{\img(T^*)}$, we can assume that $g_k \in \overline{\img (T^*)}$. Notice that we have
%$$\|g_k - g_l\|_1 \leq C\|Tg_k - Tg_l \|_2 = C\|f_k - f_l\|_2.$$
%Since $\{f_k\}$ is a convergent sequence, it is a Cauchy sequence and so also is $\{g_k\}$. Therefore there exists $g \in H_1$ with $g_k \to g$. Since $T$ has closed graph we have that $(g_k, f_k) \to (g,f) \in \{(x, Tx): x \in H_1\}$ and so $f = Tg$.
%\end{proof}

This next proposition shows another important result regarding subellipticity of the Hodge operator. By itself, this proposition is interesting, but it is also necessary for the decomposition.

\begin{prp} If the operator $\Box$ is $\epsilon$-subelliptic, then there exists $C > 0$  such that
\begin{equation}
    \|u\|_0 \leq C \|\Box u\|_0, \qquad u \in (\ker \Box)^\perp \cap D(\Box).
\end{equation}
%$\img(\Box)$ is closed in $L^2(\Omega; E_2).$
\end{prp}

\begin{proof} %Since $\Box$ is $\epsilon$-subelliptic, we have that if $u \in D(\Box)$ then $u \in H^\epsilon(\Omega; E_2)$ and by
Defining the norm $$ u \mapsto \left\{ \|u\|_0^2 + \|\Box u\|_0^2 \right\}^{1/2} $$ on $$ D(\Box) = \{ u \in L^2(\Box; E_2) : \Box u \in L^2(\Box; E_2) \}$$ gives a Hilbert space and subellipticity gives $D(\Box) \subset H^\epsilon(\Omega; E_2)$. By the Closed Graph Theorem, there exists a constant $C > 0$ such that
$$ \|u\|_\epsilon \leq C (\|\Box u\|_0 + \|u\|_0),$$
for all $u \in D(\Box)$. Hence, if $u \in (\ker \Box)^\perp \cap D(\Box)$, we have $$\|u\|_\epsilon \leq C \|\Box u\|_0.$$
Indeed, suppose that this last inequality is not valid. Then, for every $j$, there exist a $u_j$ such that $\|u\|_\epsilon \geq j\|\Box u _j\|_0$. Notice that, if we take $v_j = u_j/\|u\|_\epsilon\|$, we have $\|v_j\|_\epsilon = 1$ and $\|\Box v_j\| < 1/j$. There exists a subsequence $\{v_{j_k}\}$ such that $v_{j_k} \to v$ in $L^2(\Omega; E_2)$ and clearly $v \in \ker \Box \cap (\ker \Box)^\perp$. Notice that $$ 1 \leq C (\|\Box v_{j_k}\|_0 + \|v_{j_k}\|_0)$$ and so
$$ 1 \leq C \|v\|_0$$
which is a contradiction. The proof is completed.
\end{proof}

A standard argument, making use of 2.10 (see, for instance, Lemma 4.1.1 in \cite{hormander1973introduction}), shows the existence of a bounded linear operator $G : (\ker \Box)^\perp \to (\ker \Box)^\perp$ with $\|G\| \leq C$ such that $\Box G f = f$ for $f \in \ker \Box.$ Now, given $g \in L^2(\Omega; E_2)$, we can write $g = f + h$ with $h \in \ker \Box$ and $f \in (\ker \Box)^\perp$. Hence $g = \Box G f + h$.
Moreover, if $g \in \mc C^\infty(\Omega; E_2)$, both $f$ and $h$ also are in $\mc C^\infty(\Omega; E_2)$, and also $Gf \in \mc C^\infty(\Omega; E_2)$ because $\Box$ is hypoelliptic.
%Now we are going to see that even with weaker conditions, the Hodge Laplacian still has some nice properties.

%\begin{prp}
%Suppose that $\Box$ is $\epsilon$-subelliptic. Let $D(T) = H^{\epsilon}(\Omega; E_2)$ and define $$T : D(T) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ by $Tu = \Box u$ for $u \in D(T)$. Then $T$ is a self-adjoint operator. Particularly, we have $$L^2(\Omega;E_2) = \ker T \oplus \img T.$$
%\end{prp}

%\begin{proof}
% Notice that $$\iip{\Box u, v}_2 = \iip{u, \Box v}_2$$
%for all $u, v \in \mathcal C^\infty(\Omega; E_2).$ Since $\mathcal C^\infty(\Omega; E_2)$ is a dense subset of $H^{\epsilon}(\Omega; E_2)$, given $u, v \in H^{\epsilon}(\Omega; E_2)$ there exist sequences $\{u_j\}$ and $\{v_j\}$ in $\mathcal C^\infty(\Omega; E_2)$ such that $u_j \to u$ and $v_j \to v$ in $H^{\epsilon}(\Omega; E_2)$ and so
%$\Box u_j \to \Box u$ and $\Box v_j \to \Box v$ in $L^2(\Omega; E_2)$ and since $$\iip{\Box u_j, v_j}_2 = \iip{u_j, \Box v_j}_2$$
%for all $j$. Therefore we conclude that $\iip{\Box u, v}_2 = \iip{u, \Box v}_2$ and so $\iip{T u, v}_2 = \iip{u, T v}_2$ and $T$ is a symmetric operator.

%To conclude we have to show that $D(T) = D(T^*)$. Let $v \in D(T^*)$. The operator $$ u \in D(T) \mapsto \iip{Tu, v}_2 $$ is continuous in $D(T)$ and so there exists a constant $C > 0$ such that
%$$ |\iip{Tu, v}_2 | \leq C\|u\|_2, \qquad \forall u \in D(T).$$
%Particularly, if we define $S \in \mc D'(M; E_2)$ by $S(\phi) = \iip{T\phi, u}$ for $\phi \in \mathcal C^\infty(\Omega; E_2)$, we have that there exists $w \in L^2(\Omega; E_2)$ such that $\iip{T \phi, u}_2 = \iip{\phi,w}_2$ and so $$ \overline{w}(\phi) = \overline{u}(\Box \phi)$$ for all $\phi \in \mathcal C^\infty(\Omega; E_2)$, that is $\Box \overline{u} = \overline{w}$ in $\mc D'(\Omega;E_2)$ and since $w \in L^2(\Omega;E_2)$ we have $w \in H^{\epsilon}(\Omega;E_2) = D(T)$.
%\end{proof}

% Assume that $\Box$ is $\epsilon$-subelliptic. We have that there exists $C > 0$ satisfying
% $$ \|u\|_0 \leq C\|\Box u\|_0$$
% for all $u \in D(\Box) \cap \ker \Box^\perp$ and according to Lemma 4.1.1 in \cite{hormander1973introduction} given any $f \in \ker \Box^\perp$ there is $u \in L^2(\Omega; E_2)$, $\|u\|_0 \leq C \|f\|_0$ such that $\Box u = f$. Let $\Pi$ denote the orthogonal projection on $\ker \Box^\perp$ and, for $f \in L^2(\Omega; E_2)$ let $Gf$ be the unique solution to $\Box u = \Pi f$ which is orthogonal to the kernel of $\Box$ in $L^2(\Omega; E_2)$. Then $G : L^2(\Omega; E_2) \to L^2(\Omega; E_2)$ is bounded, with norm $ \leq C$, and $\Box G = \Pi$ in $L^2(\Omega; E_2)$. We shall refer to $G$ as the Green operator of $\Box$.

% And we have everything we need to prove the main result of this section.

We have proved:

\begin{prp} If $\Box$ is $\epsilon$-subelliptic, then
we have the Hodge decomposition
\begin{equation}
	\label{eq:hodge_decomposition}
	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box(\mathcal  C^\infty(\Omega;E_2) ) = \ker \Box \oplus A_1 ( \mathcal C^\infty(\Omega;E_1) ) \oplus A_2^* (\mathcal C^\infty(\Omega;E_3))
\end{equation}
and
\begin{equation}
	\label{eq:hodge_decomposition_isomorphism}
	\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.
\end{equation}

\end{prp}

% \begin{proof} Let $f \in \mathcal C^\infty(\Omega; E_2)$. We write $f = f_1 + f_2$ with $f_1 \in \ker \Box $ and $f_2 \in \img(T)$. Since $f_2 \in \img(\Box)$ we can write $f_2 = \Box u$ for some $u \in H^\epsilon(\Omega; E_2)$. Notice that since $\Box f_1 = 0$ we have $f_1 \in \mathcal C^\infty(\Omega;E_2)$ and so $f_2 = f - f_1 \in \mathcal C^\infty(\Omega;E_2)$ and since $f_2 = \Box u$ we have $u \in \mathcal C^\infty(\Omega;E_2)$ and we obtained the Hodge decomposition:
% $$ \mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box( \mathcal C^\infty(\Omega;E_2) ) .$$

% If $u \in \mathcal C^\infty(\Omega;E_2)$ such that $A_2u=0$, then we can write $u = u_1 + \Box u_2$ with $\Box u_1 = 0$ and $u_2 \in \mathcal C^\infty(\Omega;E_2).$ We have $u = u_1 + A^*_2 A_2 u_2 + A_1 A^*_1 u_2$. Applying $A_2$ on both sides of this equality and using Proposition \ref{prp:kernel_Box_decomposition} we conclude that
% $$ A_2 A^*_2 A_2 u_2 = 0.$$
% We have $A_2^*A_2 u_2 = 0$ because $\iip{A_2^* A_2 u_2, A_2^* A_2 u_2} = \iip{A_2 u_2, A_2 A_2^* A_2 u_2} = 0$ and then $u = u_1 + A_1 A^*_1 u_2,$ that is $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.$$
% \end{proof}

% The following version of the decomposition is more suitable for the application in this work.

% \begin{prp} If $\Box$ is $\epsilon$-subelliptic, then
% we have the decomposition
% \begin{equation}
% 	\label{eq:second_hodge_decomposition}
% 	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus A_1 ( \mathcal C^\infty(\Omega;E_1) ) \oplus A_2^* (\mathcal C^\infty(\Omega;E_3)).
% \end{equation}
% The space $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} $$ is isomorphic to $\ker \Box$ with each equivalence class in the former having a unique representative in the latter.
% \end{prp}


==> chp-lie-algebra-cogomology-and-botts-theorem.tex <==

\chapter{Lie algebra cohomology and Bott's theorem}

\input sec-cohomology-of-lie-algebras

\section{Bott's Theorem}

    On this section, we state a theorem by Bott that is useful when dealing with elliptic involutive structures on compact Lie groups. The following two lemmas are necessary for the statement of Bott's theorem:

\begin{lem}
    Let $G$ be a complex Lie group. If $f$ is (anti-)holomorphic then $Xf$ is (anti-)holomorphic for all left invariant vectors $X$.
\end{lem}

\begin{proof}
    First we assume that $X$ is a real vector field. By definition we have $$(Xf)(x) = \left. \frac{\dext}{\dext t} \right|_{t=0} f(x \exp(t X(e))) $$ we write $f_t(x) = f(x \exp(t X(e)))$ and since our complex structure is left invariant we have that left translations are holomorphic and so $f_t$ is holomorphic for every $t$. Now, let $(z_1, \ldots, z_N)$ be local coordinates in $U$ and let $x \in U$. We have that
    $$  \frac{\del}{\del \overline{z_j}} \frac{\dext}{\dext t} f_t(x) =  \frac{\dext}{\dext t} \frac{\del}{\del \overline{z_j}} f_t(x) = 0$$ and so $Xf$ is holomorphic. For a complex left invariant vector field $X$ we write $X = \Re X + i \Im X$ and so $Xf$ is just the sum of two holomorphic functions, $\Re X f$ and $i\Im X f$.

    With the obvious adaptation of this argument we have that if $f$ is anti-holomorphic then $Xf$ is anti-holomorphic.
\end{proof}


Let $U$ and $G$ be complex Lie groups with $U$ closed in $G$. Let $\Omega = G/U$ and suppose that $G$ is connected and $\Omega$ is compact and simply-connected.

By a theorem of Montgomery \cite{montgomery1950simply}, if $K$ is a maximal compact subgroup of $G$,  on the above conditions, $K$ will act transitively on $\Omega$ and therefore $\Omega$ has another description:
$$ \Omega = K/H$$
with $H = U \cap K$.

We denote by $\frk g, \frk u, \frk k, \frk h$ the complexified Lie algebra of $G$, $U$, $K$ and $H$. Since $G$ is a complex Lie group, we can decompose $\frk g$ into two ideals $\frk g = \frk g_\alpha \oplus \frk g_\beta$ in which $\frk g_\alpha$ is the set of all left-invariant vector fields annihilated by all anti-holomorphic differential forms on $G$ and $\frk g_\beta$ is the set of all left-invariant vector fields annihilated by all holomorphic differential forms on $G$.

The sets $\frk g_\alpha$ and $\frk g_\beta$ are ideals. They are obviously subalgebras, so we only need to prove the following:

\begin{lem}
    If $X \in \frk g_\alpha$ and $Y \in \frk g_\beta$, then $[X,Y] = 0$.
\end{lem}

\begin{proof}
    Let $f$ be holomorphic. By definition if $X \in \frk g_\alpha$ then $X$ annihilates every holomorphic function, so $Xf = 0$ and by the preceding lemma $Yf$ is also holomorphic so $$ [X,Y]f = X(Yf) - Y(Xf) = 0$$ and we conclude that $[X,Y] \in \frk g_\alpha$. By an analogous argument we have that $[X,Y] \in \frk g_\beta$ and so $[X,Y] = 0$.
\end{proof}


Let $\alpha : \frk g \to \frk g_\alpha$ be the projection and denote by $\imath : \frk k \to \frk g$ the inclusion of $\frk k$ into $\frk g$. Write $\frk u_* = (\alpha \imath)^{-1}(\frk u)$. Clearly $\frk u_* \subset \frk k$. In the case where $G$ is the complexification of $K$, which we can always assume by Montgomery's theorem, and also will be the case in which we will apply this theorem, $u_*$ can be identified with $\frk u_\R$, the real Lie algebra of $U$.

\begin{thm}[Bott's theorem]
Let $G$, $U$, $K$, $H$ and $\Omega$ with the conditions we just established and let $\mathscr O^p$ be the sheaf of local holomorphic $p$-forms on $\Omega$. Then
$$ H^q(\Omega; \mathscr O^p) = H^q(\frk u_*, \frk h, \Lambda^p(\frk k / \frk u_*)^*)$$
with $u_*$ acting on $\Lambda^p(\frk k / \frk u_*)^*$ via adjoint action.
\end{thm}

\subsection{Applications of Bott's theorem}

Now we are going to prove some propositions and lemma that are going to be useful when applying Bott' theorem.

% \subsection{Technical lemmas} %  useful when applying Bott's theorem}
% The technique on the next result was first suggested by Ben McKay on Math Overflow\footnote{https://mathoverflow.net/questions/268595/holomorphic-extension-of-an-action-by-a-compact-lie-group-on-a-complex-homogeneo} but since I could not understand his suggestion I found another proof based on a result by Kobayashi.

\begin{prp}
\label{prp:ext_act_complexified} Let $G$ be a connected compact Lie group acting transitively on a smooth manifold $\Omega$. If $\Omega$ is endowed with a complex structure invariant by the action of $G$, then this action extends to a transitive holomorphic action of $G_\C.$
\end{prp}

\begin{proof} We are assuming that the action of $G$ preserves the complex structure, so each automorphism $T_g : \Omega \to \Omega$ is holomorphic and we have a group homomorphism
\begin{equation}
\label{eq:cont_homo_of_groups}
	g \in G \mapsto T_g \in \Aut_\Ho(\Omega).
\end{equation}

Since $\Omega$ is compact, by \cite{kobayashi2012transformation} Theorem 1.1, chapter III, the set $\Aut_\Ho(\Omega)$ is a complex Lie group. The topology on $\Aut_\Ho(\Omega)$ is the compact open topology, and in this case it is uniform convergence over the compacts. Since $T : G \times \Omega \to \Omega$ is smooth, in particular it is uniformly continuous, we have that the map \eqref{eq:cont_homo_of_groups} is continuous and so it is automatically a Lie group homomorphism.

Let $(G_\C, \eta)$ be the universal complexification of $G$. By the universal property, there exist a complex Lie group homomorphism $g \in G_\C \mapsto T'_g \in \Aut_\Ho(\Omega)$ such that $T'_{\eta(g)} = T_g$ for all $g \in G$. Since $G$ is compact we have that $\eta$ is injective and $G$ can be identified with $\eta(G)$ and the action $T'$ can be considered an extension of $T$.
\end{proof}


\begin{lem}
\label{ss:lem:sctoss} Let $G$ be a semisimple compact Lie group and suppose that it is endowed with an elliptic involutive structure $\frk h \subset \frk g$. Then its universal covering group $G'$ also is compact and admits an elliptic involutive structure $\frk h'$ such that $H^{p,q}(G; \frk h) \cong H^{p,q}(G';\frk h')$.
\end{lem}

\begin{proof}
By Weyl's theorem (Theorem 4.26 of \cite{knapp2016representation}) the universal covering $G'$ is compact. We know that covering map $\pi : G' \to G$ gives an isomorphism between $\frk g$ and $\frk g'$ so via this isomorphism we define $\frk h' \subset \frk g'$.

We denote by $\mathcal S_{\frk h}$ the sheaf of local solutions of $\frk h$ and by $\mathcal S_{ \frk h'}$ the sheaf of local solutions of $\frk h'$. Let $\mathcal U'$ be a finite covering of $G'$ consisting of sets satisfying the following conditions: if $U' \in G'$ and $U = \pi(U')$ then $\pi|_{U'}: U' \to U$ is a diffeomorphism and $H^q(U'; \mathcal S_{\frk h'}) = 0$ for $q > 0.$ The condition about the diffeomorphism is possible because $\pi$ is a covering and the condition about the sheaf cohomology is possible because $\frk h'$ is elliptic. By taking $\mathcal U = { U = \pi(U'): U' \in U}$ we have a finite open covering for $G$ such that $H^q(U; \mathcal S_{\frk h}) = 0$.

Next construct a cochain isomorphism between $(C^q(\mathcal U', \mathcal S_{\frk h'}), \delta'^q)$ and $(C^q(\mathcal U', \mathcal S_{\frk h'}), \delta^q)$. Since $\mathcal U'$ is finite, we can enumerate its elements $U'_1, U'_2, \ldots$ and we have a one-to-one correspondence with elements of $\mathcal U$, $U_1, U_2, \ldots$, so for any simplex of $\sigma \in N(\mathcal U)$ there is a unique associated simplex $\sigma' \in N(\mathcal U')$ that is, if $\sigma = (i_0, \ldots, i_q)$ and $|\sigma| = U_{i_0} \cap \cdots \cap U_{i_q} $ then $\sigma' = (i_0, \ldots, i_q)$ and $|\sigma'| = U'_{i_0} \cap \cdots \cap U'_{i_q} $.

Let $f' \in (C^q(\mathcal U', \mathcal S_{\frk h'}), \delta'^q)$ and let $\sigma'$ be a $q$-simplex. We define $f_\sigma$ in $|\sigma|$ by $f_\sigma(x) = f'(\pi^{-1}(x))$. This function $f_\sigma$ is well defined because $\pi|_{\sigma'}$ is a diffeomorphism and is in $\mathcal S_{\frk h}$. So we define a map $\phi : C^q(\mathcal U', \mathcal S_{\frk h'}) \to C^q(\mathcal U', \mathcal S_{\frk h'})$ and which is obviously bijective and also commute with the restrictions, so we have that $\delta^q \phi(f') = \phi( \delta'^q f')$ so it induces an isomorphism in cohomology $H^q(\mathcal U',\mathcal S_{\frk h}) \cong H^q(\mathcal U;\mathcal S_{\frk h})$.

Now, by using Leray's Theorem \cite{gunning1965analytic} (Section D, Theorem 4), for every $q \geq 0$, we have that $H^q(G',\mathcal S_{\frk h'}) \cong H^q(\mathcal U';\mathcal S_{\frk h'})$ and $H^q(G,\mathcal S_{\frk h}) \cong H^q(\mathcal U;\mathcal S_{\frk h})$ and finally we have  $H^q(G',\mathcal S_{\frk h'}) \cong H^q(G,\mathcal S_{\frk h})$.
% Since $\pi$ is a proper finite-to-one map, by Corollary of \cite{demailly1997complex} we have that $H^p(G',\mathcal S_{\frk h'}) \cong H^p(G,q_*\mathcal S_{\frk h'}) = H^p(G,\mathcal S_{\frk h})$.
\end{proof}

% % \begin{thm} Let $G$ be a connected compact Lie group endowed with a involutive structure $\frk h \subset \frk g.$ Let $K \subset G$ be a connected closed subgroup of $G$ and take $\frk h' = \frk h \cap \frk k$. Let $\Omega = G / K$ and denote by $\pi : G \to \Omega$ the quotient map. Suppose that $\mathcal V = \pi_*(\frk h)$ is an involutive structure on $\Omega$. If the induced map $i^* : H^p(G; \mathcal S_{\frk h}) \to H^p(K; \mathcal S_{\frk h'}) $ is surjective, then
% % $$ H^p(G; \mathcal S_{\frk h}) \cong \sum_{r+s= p} H^r(\Omega; \mathcal S_{\mathcal V}) \otimes H^r(K; \mathcal S_{\frk h'}) $$
% % \end{thm}

% % \begin{proof} By \cite{hilgert2011structure} it is possible to find a covering $\{U_j\}$ of  $\Omega$ and smooth sections $\sigma_j$ of the quotient map $\pi : G \to \Omega$ such that $$ (u, k) \in U_j \times K \xmapsto{ m_j } \sigma_j(u)k \in \sigma_j(U_j)K$$
% % is a diffeomorphism onto an open subset of $G$ which we are going to denote by $V_j$. Notice that $\{V_j\}$ is a covering for $G$. In fact, let $g \in G$ and take $U_j$ such that $\pi(g) \in U_j$. Then $g = \sigma_j(\pi(g))e \in V_j$.

% % Let $\mathcal V_j = \pi_* \frk|_{U_j}$ be the restriction of the structure on $\Omega$ and we endow $U_j \times K$ with the structure given by the direct sum of $\mathcal V_j$ and $\frk h'$. Notice that each isomorphism $m_j$ preserve the structures of $U_j \times K$ and $V_j$, in fact if $Z \in \mathcal V_j \oplus \frk h'$ then we can write $Z = (X, Y)$ with $X \in \mathcal V_j$ and $Y \in \frk h'$. The map $m_j$ can be written as
% %  $$ m_j(u,k) = \mu(\sigma(u),k) $$
% % with $\mu : G \times G \to G$ the multiplication. Now $(m_j)_* (X,Y) = (\sigma_j)_*X + Y$. Clearly $Y \in \frk h' \subset \frk h$ and $(\sigma_j)_*X \in \frk h$ or $\sigma$ would not be a section for $\pi$. Since $\sigma_j$ is a diffeomorfism and both structures have the same rank, we have then that inverse of $m_j$ also preserves the structure. Therefore, by applying Künneth's formula, the cohomology of $H^p(V_j,\mathcal S_{\frk h})$ is isomorphic to $$ \sum_{r + s = q} H^r(U_j,\mathcal S_{W_j}) \otimes H^s(K,\mathcal S_{\frk h'}).$$

% % If $V_j \cap V_k \neq \emptyset$ we can use the same reasoning and compute the cohomology in $V_j \cap V_k$, therefore the proof can be completed by using a Mayer-Vietoris argument.


% % \end{proof}

% % \begin{lem} Let $G$ be a compact connected Lie group endowed with an elliptic involutive structure $\frk h \subset \frk g$. Let $\frk k_\R = \frk h \cap \overline{\frk h} \cap \frk g_\R$ and we assume that the group $K = \exp_G(\frk k_\R)$. We endow $K$ with the De Rham structure. Then the inclusion $ i : K \to G$ induces a surjective homomorphism in cohomology
% % $$ i^* : H^{q}_{\frk h} (G) \to H^q_{dR}(K). $$
% % \end{lem}

% % \begin{proof} Let $\mathcal U = \{U_j\}$ be a covering for $G$ such that each $U_j$ is connected and $ H^{q}_{\frk h} (|\sigma|) = \{0\} $ for all $q$-simples $\sigma$ in which $|\sigma| = U_{j_0} \cap \ldots \cap U_{j_q} \neq \emptyset$. By decreasing $U_j$ if necessary, we can assume that $V_j = K \cap U_j$ also satisfies $H^{q}_{dR} (|\sigma'|) = \{0\}$ with $|\sigma'| = V_{j_0} \cap \ldots \cap V_{j_q} \neq \emptyset$.

% %  By Leray's theorem we have that there is an isomorphism $\phi : H^q(\mathcal V, \C) \to H^q(K,\C)$ and an isomorphism $\psi : H^q(\mathcal U, \mathcal O_{\frk h}) \to H^q(G, \mathcal O_{\frk h})$. Now we are going to see that the map $i^*$ induces an surjection
% %  $$ j^* : H^q(\mathcal U, \mathcal O_{\frk h}) \to H^q(\mathcal V, \C)$$
% %  such that $i^* = \psi^{-1} \circ j^*\circ \phi$.

% % The inclusion $j : C^q(\mathcal U, \mathcal O_{\frk h}) \to C^q(\mathcal V, \C)$ is defined by $g_{\sigma'}(|\sigma'|) = f_{\sigma}(|\sigma|)$. It is well defined because each $f_\sigma$ is constant on $K$ and clearly defines an homomorphism in cohomology.

% % This homomorphism is surjective. Indeep, notice that if $g \in H^q(\mathcal V, \C)$ for each $\sigma$ we can define $f_\sigma (|\sigma|) = g_{\sigma'} $ if $|\sigma| \cap K \neq \emptyset$ and we define $f_\sigma (|\sigma|) = 0$ otherwise. Since $g_{\sigma'}$ is constant in $|\sigma'|$, we clearly have $f_\sigma \in \mathcal O_{\frk h}$.

% % Now we need to verify that $i^* = \psi^{-1} \circ j^*\circ \phi$...

% % \end{proof}




% \begin{proof}[Second proof of Theorem \ref{chp:homogeneous:homo_on_simply} (Spanier's proof adapted to our case)]

% %Since we are assuming that $G$ is simply-connected and by construction $K$ is always connected, by applying the long exact sequence of homotopy, we have that $\Omega$ is also simply-connected.

% % Furthermore, by Proposition \ref{prp:ext_act_complexified} we can extend the action of $G$ on $\Omega$ to an action $T$ on its universal complexification $G_\C$. Let $p \in \Omega$ be any point and consider $U$ the Lie group given by
% % $$ U = \{ g \in G_\C : T_g p = p\}.$$

% % The group $U$ is clearly closed and it follows from basic results on homogeneous spaces that $G_\C / U = \Omega$. By a Theorem 10.1.10 of \cite{hilgert2011structure} we have that the action is regular and so $U$ is a complex Lie subgroup of $G_\C$.


% Let $[\alpha] \in H^{p,r}_{\delbar}(\Omega)$ and $[\beta] \in H^s_d(K)]$. We can always choose $v$ left-invariant, so by the last lemma there exist an extension of $\beta$ to $G$, denoted here by $\beta'$,  such that $\dext' \beta' = 0$ and since  $\dext' (\pi^*u) = \pi^* (\delbar u) = 0$, we have that $\pi^*\alpha \wedge \beta'$ is $\dext'$-closed and its restriction to each fiber $gK$ is closed, so it is a cohomology extension and according to \cite{spanier1994algebraic} chapter 5 Theorem 9 the proof is completed.

% $$ ([\alpha],[\beta]) \in H^{p,r}_{\delbar}(\Omega) \times H^s_d(K)] \xmapsto{\phi} [\pi^*\alpha \wedge \beta'] \in H^{l,r+s}_{\dext'}(G).$$

% By the universal property of the tensor product this and sum over all $r$ and $s$ such that $r + s = q$ we have the following map that we are going to show that is an isomorphism:

% $$ \sum_{r+s=q} H^{p,r}_{\delbar}(\Omega) \times H^s_d(K)] \xmapsto{\phi}  \in H^{p,q}_{\dext'}(G)$$

% By \cite{hilgert2011structure} it is possible to find a covering $\{U_j\}$ of  $\Omega$ and smooth sections $\sigma_j$ of the quotient map $\pi : G \to \Omega$ such that $$ (u, k) \in U_j \times K \xmapsto{ m_j } \sigma_j(u)k \in \sigma_j(U_j)K$$
% is a diffeomorphism onto an open subset of $G$ which we are going to denote by $V_j$.

% Let $\mathcal W_j = \pi_* \frk|_{U_j}$ be the restriction of the complex structure on $\Omega$ and we endow $U_j \times K$ with the structure given by the direct sum of $\mathcal W_j$ and $\C TK$. Notice that each isomorphism $m_j$ preserve the structures of $U_j \times K$ and $V_j$, in fact if $Z \in \mathcal W_j \oplus \C TK$ then we can write $Z = (X, Y)$ with $X \in \mathcal W_j$ and $Y \in \C TM$. The map $m_j$ can be written as
%  $$ m_j(u,k) = \mu(\sigma(u),k) $$
% with $\mu : G \times G \to G$ the multiplication. Now $(m_j)_* (X,Y) = (\sigma_j)_*X + Y$. Clearly $Y \in \C T K \subset \frk h$ and $(\sigma_j)_*X \in \frk h$ or sigma would not be a section for $\pi$. Since $m_j$ is a diffeomorfism and both structures have the same rank, we have then that inverse of $m_j$ also preserves the structure. Therefore, by applying Künneth's formula, the cohomology of $H^{p,q}(V_j,\mathcal O_{\frk h})$ is isomorphic to $$ \sum_{r + s = q} H^{p,r}(U_j,\mathcal O_{W_j}) \otimes H^s(K,\C)$$
% and the isomorphism is given by the extension of the bilinear maps
% $$([\alpha],[\beta]) \in H^{p,r}(U_j,\mathcal O_{W_j}) \times H^s(K,\C) \xmapsto{\psi_j} [\pi_1^* \alpha \wedge \pi_2^* \beta] \in  H^{p,r+s}(V_j,\mathcal O_{\frk h})$$ to $$\sum_{r+s=q}H^{p,r}(U_j,\mathcal O_{W_j}) \otimes H^s(K,\C).$$

% With a simple computation we see that $m_j^* \phi_j = \psi_j$. In fact, let $([u], [v]) \in H^{p,r}_{\delbar}(U_j) \times H^s{K}$ and so $\phi_j([u], [v]) = [ \pi^*u \wedge v']$ and now we need to compute $m_j^* (\pi^*u \wedge v')$. Let $$(Z_1, T_1), \ldots, (Z_q, T_q) \in \C T U_j \times K$$ and notice that
% $$
% \begin{aligned} m_j^* (\pi^*u & \wedge v')((Z_1, T_1), \ldots, (Z_q, T_q))  = (\pi^*u \wedge v')( \sigma_*(Z_1) + T_1, \ldots, \sigma_*(Z_{p+q}) + T_{p+q} ) \\
% 	& = \frac{1}{(p+q)!} \sum_{\tau \in S_{p+q}} (\pi^*u)( \sigma_*(Z_{\tau(1)}) + T_{\tau(1)}, \ldots )v'(\sigma_*(Z_{\tau(p+q+1)}) + T_\tau(p+q+1), \ldots ) \\
%  & = \frac{1}{(p+q)!} \sum_{\tau \in S_{p+q}} u(Z_{\tau(1)}, \ldots, Z_{\tau(p+r)}))v(T_\tau(p+q+1), \ldots, T_{p+r+s})  \\  & = \psi_j(\pi_1^*u \wedge \pi_2^*v)((Z_1, T_1), \ldots, (Z_q, T_q)).
% \end{aligned}
% $$
% Therefore $\phi_j = (m_j^*)^{-1}\psi_j$ and so the restriction of $\phi$ to $U_j \times K$ is an isomorphism.

% If $V_j \cap V_k \neq \emptyset$ we can use the same reasoning and compute the cohomology in $V_j \cap V_k$, therefore the proof can be completed by using a Mayer-Vietoris argument and the Five Lemma. In fact, consider the following diagram with the column on the left being the Mayer Vietoris sequence of the cohomology of $H^{p,q}_{\dext'}(U_j \cup U_k \times K)$ and the maps of the right column being the only one making the diagram commutative and the sequence exact:

% $$\xymatrix{
% \vdots \ar[d] & \vdots \ar[d] \\
% 	H^{p,q-1}_{\dext'}(U_j \times K) \oplus H^{p,q-1}_{\dext'}(U_k \times K) \ar[d] \ar[r]^-{\psi_j \oplus \psi_k }  & \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_j) \otimes H^s(K) \oplus \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_k) \otimes H^s(K)  \ar[d] \\
%     H^{p,q-1}_{\dext'}(U_j \cap U_k \times K)  \ar[d] \ar[r]^-{\psi_{j \cap k} }  & \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_j \cap U_k) \otimes H^s(K) \ar[d] \\
%     H^{p,q}_{\dext'}(U_j \cup U_k \times K)  \ar[d] \ar[r]^-{\psi_{j \cup k} }  & \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_j \cup U_k) \otimes H^s(K) \ar[d] \\
%     H^{p,q}_{\dext'}(U_j \times K) \oplus H^{p,q}_{\dext'}(U_k \times K) \ar[d] \ar[r]^-{\psi_j \oplus \psi_k }  & \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_j) \otimes H^s(K)\oplus \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_k) \otimes H^s(K)  \ar[d] \\
%     H^{p,q}_{\dext'}(U_j \cap U_k \times K)  \ar[d] \ar[r]^-{\psi_{j \cap k} }  & \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_j \cap U_k) \otimes H^s(K) \ar[d] \\
%     \vdots & \vdots \\
% }$$

% Now consider the following diagram with the sequence of the left column being as defined above and the sequence on the right column being the Mayer-Vietoris sequence associated to for $H^{p,q-1}_{\dext'}(V_j \cup V_k)$:
% $$\xymatrix{
% \vdots \ar[d] & \vdots \ar[d] \\
%   \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_j) \otimes H^s(K) \oplus \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_k) \otimes H^s(K) \ar[r]^-{\ \phi_j \otimes \phi_k} \ar[d] & H^{p,q-1}_{\dext'}(V_j) \oplus H^{p,q-1}_{\dext'}(V_k) \ar[d] \\
%       \displaystyle \sum_{r + s = q-1} H^{p,r}_{\delbar}(U_j \cap U_k ) \otimes H^s(K)  \ar[r]^-{\phi_{j \cap k}} \ar[d] & H^{p,q-1}_{\dext'}(V_j \cap V_k) \ar[d] \\
%       \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_j \cup U_k ) \otimes H^s(K)  \ar[r]^-{\phi_{j \cup k}} \ar[d] & H^{p,q-1}_{\dext'}(V_j \cup V_k) \ar[d] \\
%       \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_j) \otimes H^s(K) \oplus \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_k) \otimes H^s(K)  \ar[r]^-{\ \phi_j \otimes \phi_k} \ar[d] & H^{p,q}_{\dext'}(V_j) \oplus H^{p,q}_{\dext'}(V_k) \ar[d] \\
%       \displaystyle \sum_{r + s = q} H^{p,r}_{\delbar}(U_j \cap U_k ) \otimes H^s(K)  \ar[r]^-{\phi_{j \cap k}} \ar[d] & H^{p,q}_{\dext'}(V_j \cap V_k) \ar[d] \\
%     \vdots & \vdots \\
% }$$

% This diagram is commutative and the maps $\phi_j \otimes \phi_k$ and $\phi_{j \cap k}$ are isomorphisms and so, by the Five Lemma, the map $\phi_{j \cap k}$ is an isomorphism. The proof finishes by induction.
% \end{proof}



\begin{thm}
\label{thm:homogeneous:homo_on_simply2} Let $G$ be a connected, simply-connected and compact Lie group and suppose that $\frk h \subset \frk g$ is an elliptic involutive structure. Let $\frk k = \frk h \cap \overline{\frk h}$ and take $\frk k_\R \subset \frk g_\R$ such that $\frk k = \frk k_\R \otimes \C$. Assume that the group $K = \exp_G(\frk k_\R)$ is closed. Assume that there exist an ideal $\frk z \subset \frk h$ such that $\frk k \oplus \frk z = \frk h$. Consider the homogeneous space $\Omega = G / K$ endowed with the complex structure $\pi_* \frk h$ induced by the quotient map $ \pi : G \to \Omega$. Then we have
$$ H^{p,q}(G; \frk h) \cong \sum_{r + s = q} H^r(\frk u_*, \frk k, \Lambda^p(\frk g / \frk u_*)) \otimes H^s(\frk k).$$
\end{thm}

\begin{proof}
Since $G$ is simply-connected and $K$ is connected by construction, we use the long exact sequence of homotopy groups gives and conclude that $\Omega$ is simply-connected. Since $G$ is compact we have that $\Omega$ is compact and so we can apply Bott's theorem.
\end{proof}

Notice that by applying Lemma \ref{ss:lem:sctoss} we have the same result by requiring only that $G$ is semisimple.

\begin{thm}
\label{thm:homogeneous:homo_on_simply3} Let $G$ be a connected, semisimple and compact Lie group and suppose that $\frk h \subset \frk g$ is an elliptic involutive structure. Let $\frk k = \frk h \cap \overline{\frk h}$ and take $\frk k_\R \subset \frk g_\R$ such that $\frk k = \frk k_\R \otimes \C$. Assume that the group $K = \exp_G(\frk k_\R)$ is closed. Assume that there exist an ideal $\frk z \subset \frk h$ such that $\frk k \oplus \frk z = \frk h$. Consider the homogeneous space $\Omega = G / K$ endowed with the complex structure $\pi_* \frk h$ induced by the quotient map $ \pi : G \to \Omega$. Then we have
$$ H^{p,q}(G; \frk h) \cong \sum_{r + s = q} H^r(\frk u_*, \frk k, \Lambda^p(\frk g / \frk u_*)) \otimes H^s(\frk k).$$
\end{thm}

\begin{cor}
    Let $G$ be a and semisimple Lie group compact Lie group and let $T \subset G$ be maximal torus.  Consider the following elliptic Lie algebra $ \frk h = \frk t \oplus \bigoplus_{\alpha \in \Delta_+} \frk g_\alpha$ with $\frk t$ being the complexification of the Lie algebra of the maximal torus $T$. Then we have $$ H^{0,q}(G) = H^{0,q}(T).$$
\end{cor}

\begin{proof}
    % Consider the following elliptic Lie algebra $$ \frk h = \frk t \oplus \bigoplus_{\alpha \in \Delta_+} \frk g_\alpha$$ with $\frk t$ being the complexification of the Lie algebra of the maximal torus $T$.

    We define the homogeneous manifold $\Omega \doteq G / T$ and we denote the quotient map by $\pi : G \to \Omega$. Notice that we have precisely the hypothesis of Theorem \ref{thm:homogeneous:homo_on_simply3}. Therefore we have
    $$ H^{0,q}(G) = \sum_{ r + s = q} H^{0,r}(T; \frk t) \otimes H^{0,s}_{\delbar}(\Omega) = H^{0,q}(T)$$ and the last equality follows from the fact $H^{p,q}_{\delbar}(\Omega) = 0$ if $p \neq q$ and $H^{0,0}_{\delbar}(\Omega) = \C$. In this case we can compute the $\dext'$-cohomology of $G$ using only algebraic methods.
\end{proof}

\subsection{Examples}

    Now we are going to show a few examples that are not a directly application of the theorems above, but with a left-invariant elliptic structure whose cohomology can be studied by techniques that are very closed to the ones used to prove the results discussed in this work.

    Let $G$ be a and semisimple Lie group compact Lie group and let $T \subset G$ be maximal torus. Let $\Omega \doteq G / T$ be a homogeneous manifold with quotient map denoted by $\pi : G \to \Omega$.

\begin{exa}
    Consider the following elliptic Lie algebra $$ \frk h = \frk e \oplus \bigoplus_{\alpha \in \Delta_+} \frk g_\alpha$$ with $\frk e$ being an elliptic structure on the maximal torus.

    The quotient map induces a complex structure on $\Omega$ which is known to be Kähler.

    Let $[u] \in H^{0,q}(T; \frk e)$. We know that we can choose $u$ to be a left-invariant form, so we can extend it to a cohomology extension and by the Leray-Hirsch theorem we have

    $$ H^{0,q}(G; \frk h) = \sum_{ r + s = q} H^{0,r}(; \frk eT) \otimes H^{0,s}(\Omega; \pi_*(\frk h)) = H^{0,q}(T; \frk e)$$ and the last equality follows from the fact $H^{p,q}(\Omega;  \pi_*(\frk h)) = 0$ if $p \neq q$ and $H^{0,0}_{\delbar}(\Omega) = \C$. In this case we can compute the cohomology of $G$ using only algebraic methods.

    Notice that if $\frk k = \frk h \cap \overline{\frk h}$ is closed then we can write $\frk h = \frk k \oplus \frk u$ with $\frk u = \frk e \cap \overline{\frk e} \oplus \bigoplus_{\alpha \in \Delta_+} \frk g_\alpha$ being an ideal. So, if we assume that the integral group of $\frk k_\R$ is closed we can also apply Theorem \ref{thm:homogeneous:homo_on_simply3}.
\end{exa}

\begin{exa}
    Now let $$ \frk h' = \frk e \oplus \bigoplus_{\alpha \in \Delta} \frk g_\alpha$$ again with $\frk e$ being an elliptic structure on the maximal torus.

    The projection map induces the usual De Rham cohomology on $\Omega$.

    Let $[u] \in H^{0,q}(T; \frk e)$.. Since we can choose $u$ to be a left-invariant form, we again extend it to define a cohomology extension and we have

    $$ H^{0,q}(G; \frk h') = \sum_{ r + s = q} H^{0,r}(T; \frk e) \otimes H^{s}(\Omega; \frk \C T \Omega).$$

    On the torus we proved that we can compute the cohomology using only algebraic methods and on the homogeneous manifold we know by the Chevalley Eilenberg theorem that it can also be computed using only algebraic methods, so the general cohomology also can be computed using algebraic methods.

    Notice that if $\frk k = \frk h \cap \overline{\frk h}$ is closed then we can write $\frk h = \frk k \oplus \frk u$ with $\frk u = \frk e \cap \overline{\frk e}$ being an ideal. So, if we assume that the integral group of $\frk k_\R$ is closed we can also apply Theorem \ref{thm:homogeneous:homo_on_simply3}.

\end{exa}


\begin{exa}
    Now let $$ \frk h'' = \frk e \oplus \frk f$$ with $\frk f + \overline{\frk f} = \bigoplus_{\alpha \in \Delta} \frk g_\alpha$ again with $\frk e$ being an elliptic structure on the maximal torus.

    The quotient map induces an elliptic structure invariant by the action of $G$ on $\Omega$. We are going to denote this structure by $\mathcal V_{\frk f}$.
    Here we also have a cohomology extension and so $$ H^{0,q}(G; \frk h'') = \sum_{ r + s = q} H^{0,r}(T; \frk e) \otimes H^{0,s}(\Omega; \pi_*(\frk h'')).$$

    On the torus we proved that we can compute the cohomology using only algebraic methods and on the homogeneous manifold, namely $$ H^{0,s}(\Omega; \pi_*(\frk h'')). $$ It is still an open problem how to deal with invariant elliptic involutive on homogeneous compact manifolds.
\end{exa}


==> sec-cohomology-of-lie-algebras.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COHOMOLOGY OF LIE ALGEBRAS %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Cohomology of Lie algebras}
\label{sec:cohomology_of_lie_algebras}

In this section we will define algebraic counterparts of the objects related to bidegree cohomology. These objects are the same, but using a different notation, of the paper by Hochschild and Serre \cite{hochschild1953cohomology}. A good part of this section was inspired by Bott's paper \cite{bott1957homogeneous}, but the notation was changed to better suit the necessities of this work. Most of the results in this section were written for convenience of the reader, but in order to not make the text too long the proofs were omitted. We suggest the reader to consult the original paper by  Hochschild and Serre \cite{hochschild1953cohomology} and the work of Bott \cite{bott1957homogeneous}.

The next two definitions are fundamental for this section. First we define what is a representation of a Lie algebra and then we use it to give to a vector space a structure of an action of elements from a Lie algebra on a vector space. This notion is necessary for the definition of cohomology of Lie algebras. 

\begin{dfn} Let $\frk g$ be a Lie algebra over $\C$ and $M$ a vector space over $\C$. A \emph{representation} of $\frk g$ is a Lie algebra homomorphism of $\frk g$ into the Lie algebra of all linear transformations of $M$ into $M$.
\end{dfn}

\begin{dfn}
Let $\frk g$ be a Lie algebra over $\C$ and $M$ a vector space over $\C$. We say that the pair $(M, \phi)$ is a \emph{$\frk g$-module} if $\phi$ is a representation of the Lie algebra $\frk g$ into $M$.
We denote by $X \cdot x$ the action of $\phi(X)$ on the element $x \in M$.
\end{dfn}

By definition, we have the following properties:

\begin{itemize}

\item If $X, Y \in \frk g$, $\lambda, \mu \in \C$ and $x \in M$, then
$$(\lambda X +  \mu Y) \cdot x = (\lambda X) \cdot x + (\mu Y) \cdot x.$$

\item If $X \in \frk g$, $\lambda, \mu \in \C$ and $x, y \in M$, then
$$X \cdot (\lambda x + \mu y)  = X \cdot (\lambda x) + X \cdot (\mu x).$$

\item If $X, Y \in \frk g$ and $x, y \in M$, then
$$[X,Y] \cdot x  = X \cdot ( Y \cdot x ) - Y \cdot (X \cdot x).$$

\end{itemize}

We denote by $M^{\frk g}$ the subspace of $M$ which consists of all $x \in M$ with $X \cdot x = 0$, for all $X \in \frk g$. We denote by $C^p(\frk g; M)$ the set of all alternating multi-linear $p$-forms on $\frk g$ with values in $M$ and by $C(\frk g; M)$ the formal sum $\sum_p C^p(\frk g; M)$. We identify $C^0(\frk g; M)$ with $M$. Notice that each $C^p(\frk g; M)$ is a vector space.

If $\frk h$ is an ideal of $\frk g$ (here we allow $\frk h = \frk g$), we can turn $C^p(\frk h; M)$ into a $\frk g$-module. Indeed, since $C^0(\frk h; M) = M$, it already has a structure of a $\frk g$-module. For $p > 0$, $u \in C^p(\frk h; M)$ and $X \in \frk g$, $Y_1, \ldots, Y_p \in \frk h$, we define
$$(\mathcal L_Y u)(Y_1, \ldots, Y_p) = X \cdot u(Y_1, \ldots, Y_p) - \sum_{i=1}^n u(Y_1, \ldots, Y_{i-1}, [X,Y_i],Y_{i+1}, \ldots, Y_p).$$

\begin{lem} It holds that $\mathcal L_Y u \in C^p(\frk h; M)$ for all $u \in C^p(\frk h; M)$ and it depends linearly on $Y$ and on $u$. % and
%$$ \mathcal L_{[X,Y]} u = \phi(X) \cdot (\phi(Y) \cdot u) - \phi(Y) \cdot (\phi(X) \cdot u).$$
\end{lem}

If $ u \in C^{p+1}(\frk h; M) $ and $Y \in \frk h$, we define $\imath_Y u \in C^p(\frk h; M)$ by

$$\imath_Y u (Y_1, \ldots, Y_p) = u (Y, Y_1, \ldots, Y_p).$$

Notice that this is an algebraic definition of the Lie derivative we know from the basic theory of smooth manifolds and differential geometry. The Lie derivative has the following property: for $X, Y \in \frk g$ and $u \in C^p(\frk g; M)$ we have
$$\imath_X (\mathcal L_Y u) - \mathcal L_Y ( \imath_X u) = \imath_{[X,Y]} u.$$


The coboundary operator is the unique $\frk g$-homomorphism $$\dext : C^p(\frk g; M) \to C^{p+1}(\frk g; M)$$ such that $$\imath_X \circ \dext + \dext \circ \imath_X = \mathcal L_X$$
for all $X \in \frk g.$

It is a basic exercise to verify that for all $X \in \frk g$ it holds that $ \dext (\mathcal L_X u) = \mathcal L_X (\dext u)$ and that for $p > 0$ and $u \in C^p(\frk g; M)$ and $X_1, \ldots, X_{p+1} \in \frk g$ we have the following formula
$$
\begin{aligned}
	\dext u(X_1, \ldots, X_{p+1})
		= & \sum_{j=1}^{p+1} (-1)^{j+1} X_j \cdot u(X_1, \ldots, \hat{X}_j, \ldots, X_{p+1})  \\
		 + & \sum_{j < k} (-1)^{j+k+1} u([X_j, X_k], X_1, \ldots, \hat X_j, \ldots, \hat X_k, \ldots, X_p). 
\end{aligned}
$$

From the formula above we see that this operator $\dext$ is just the algebraic version of the usual exterior differentiation on a smooth manifolds and have similar properties like, if $u \in C^0(\frk g; M) = M$, then $(\dext u)(X) = X \cdot u$ and it obviously holds that $\dext^2 = 0$.

Therefore, we have a complex with respect to $\dext$ and its cohomology module of $\frk g$ with coefficients in $M$ is a vector space over $\C$ and is written $H^*(\frk g; M).$

Now we want to discuss some conditions on modules and Lie algebras to have isomorphisms between cohomology spaces. Let $\lambda : \frk{g}' \to \frk{g}$ be a Lie homomorphism and $\eta : M \to M'$ be a linear map of the $\frk g$-module $M$ into the $\frk g'$-module $M'$. Let $\lambda^* \otimes \eta : C(\frk g; M) \to C(\frk g'; M')$ be the following linear map:

$$ [(\lambda^* \otimes \eta) u](X_1, \ldots, X_n) = \eta [u (\lambda X_1, \ldots, \lambda X_n)] \quad X_i \in \frk {g}',~u \in C^n(\frk g; M).$$



\begin{dfn} We say that the maps $\lambda$ and $\eta$ are \emph{compatibles} if
$$ \eta( \lambda X \cdot u) = X \cdot \eta u \qquad X \in \frk g',~u \in M.$$
\end{dfn}

With the notion of compatibility introduced, we can state the following basic but important result: 

\begin{lem} If $\lambda$ and $\eta$ are compatibles, the map $\lambda^* \otimes \eta $ commutes with the differential operators of the complexes in question, so it induces a homomorphism between $H^*(\frk g; M)$ and $H^*(\frk g'; M')$.
\end{lem}

Now we want to expand a little bit the notions we just introduced in order to be able to cover the cohomologies related to involutive structures. Let $R$ be a commutative algebra over $\C$. The Lie algebra of all derivations of $R$ is then itself a left $R$-module, which we denote by $\mathcal{D}$.

\begin{dfn}
If $M$ is a $R$-module, $B_R(\mathcal{D}; M)$ will denote the graded $R$-module of $R$-linear alternating functions from $\mathcal{D}$ to $M$.
\end{dfn}

\begin{dfn}
Let $M$ be a $R$-module also having a $\mathcal{D}$-module structure. We say that the $R$-module structure is compatible with the $\mathcal{D}$-module structure if
$$ X \cdot (\lambda u) = (X \cdot \lambda)u + \lambda (X \cdot u) \qquad X \in \mathcal{D},~\lambda \in R,~u \in M.$$
\end{dfn}

Suppose that $M$ is a $R$-module having a compatible $\mathcal{D}$-module structure. In this situation $C(\mathcal{D}; M)$ is well defined and $B_R(\mathcal{D}; M)$ can be identified with the subspace of $R$-linear maps in $C(\mathcal D; F).$

\begin{lem}
The subspace $B_R(\mathcal{D}; M)$ is closed under $\mathcal L_X,~ \imath_X$ and $\dext$.
\end{lem}

As a consequence, $B_R(\mathcal{D}; M)$ is a subcomplex of $C(\mathcal{D}; M)$. This subcomplex is denoted $C_R(\mathcal{D}; M)$ and its cohomology module is denoted by $H^*_R(\mathcal D; M)$. If $\mathcal{D}_0$ is a subalgebra of $\mathcal D$, closed under $R$, then $H^*_R(\mathcal D_0; M)$ and $H^*_R(\mathcal D, \mathcal D_0; M)$ are defined analogously from the complexes $C_R(\mathcal D_0; M)$ and $C_R(\mathcal D, \mathcal D_0; M)$ respectively.

Now we are finally able to show how to use the algebraic language introduced above to describe one the most important examples of involutive structures:

\begin{exa}
Let $\Omega$ be a smooth manifold and let $R = C^\infty(\Omega)$ be the algebra of all smooth complex valued functions on $\Omega$. The set of all derivations of $R$ is the Lie algebra of all smooth vector fields $\frk X (\Omega)$, then take $\mathcal D = \frk X (\Omega)$ and $M = C^\infty(\Omega)$.

In this case, $C^q_R(\mathcal D; M)$ becomes the complex $\mathcal C^\infty(\Omega; \Lambda^q)$ of all complex valued differential forms on $\Omega$, and $H^*_R(\mathcal D; M)$ is the cohomology of $\Omega$ in the sense of de Rham. We usually write $H^q(\Omega; \C)$ for $H^q_R(\mathcal D; M)$.
\end{exa}

 If $f : \Omega' \to \Omega$ is a smooth map, then $f$ induces a homomorphism $$f^* : C_R(\mathcal D; M) \to C_{R'}(\mathcal D'; M')$$ which commutes with $\dext$ and so determines a homomorphism $$f^* : H^*(\Omega; \C) \to H^*(\Omega'; \C).$$

\begin{rmk} The map $f$ does not induce a Lie homomorphism from $\mathcal D'$ into $\mathcal D$, and this is the disadvantage of treating differential forms on $\Omega$ from this point of view. 
\end{rmk}

The following example and the theorem are fundamental for this text. They provide the main motivation for this project.

\begin{exa} Let $G$ be a Lie group, and let $R = C^\infty(G; \C)$ and $\frk g$ be the complex Lie algebra of $G$.

In this case, the injection $$\rho : \frk g \to \mathcal D$$ extends to a $R$-linear Lie homomorphism
$$\rho : \frk g \otimes_\C R \to \mathcal D$$
which is bijective because $\frk g$ is a $R$-base for $\mathcal D$. Hence the induced map
$$ \rho^* : C_R(\mathcal D; R) \to C_R(\frk g; R) $$ is bijective and a chain homomorphism. We conclude that
$$ H_R^*(\mathcal D; R) \cong H^*(\frk g; R).$$

In this case we also have $H^*(G; \C) \cong H^*(\frk g; R)$.

\end{exa}

In \cite{chevalley1948cohomology}, Theorem 2.3, Chevalley and Eilenberg proved the following result.

\begin{thm} Let $G$ be a connected compact Lie group, then
$$ H^*(G) = H^*(\frk g; \C).$$
\end{thm}


\begin{exa}
Suppose that $\Omega$ is a smooth manifold and let $R = C^\infty(\Omega)$. Let $\mathbb{E}$ be a smooth vector bundle over $\Omega$ and take $M = \Gamma^\infty(\mathbb E)$ to be the set of all smooth global sections of $\mathbb{E}$. We endow $M$ with a structure of $R$-module by  pointwise multiplication. Unfortunately, we can only endow it with a compatible $\mathcal D$-structure if $\mathbb{E}$ is locally constant. The $R$-module $B_R(\mathcal D; M)$ is the space of all $\mathbb{E}$-valued forms on $\Omega$.
\end{exa}


\subsection{The cohomology induced by subalgebras}

Now we are going to introduce the concept of Lie algebra cohomology induced by subalgebras. We reinforce here that this is the algebraic version of the cohomology induced by involutive subbundles of the tangent bundle and is going to be really important for our main results. Let $\frk h \subset \frk g$ be a subalgebra.

We set $N^{0,q}_{\frk h}(\frk g; M) = C^q(\frk g; M)$ and for $p > 0$
$$N^{p,q}_{\frk h}(\frk g; M) = \{ u \in C^{p+q}(\frk g; M): u(X_1, \ldots, X_{p+q}) = 0 \text{ when } q+1 \text{ arguments are in } \frk h \}.$$
If $q < 0$ we will define $N^{p,q}_{\frk h}(\frk g; M) = \{0\}$.

Since $N^{p,q}_{\frk h}(\frk g; M) \subset N^{p+1,q-1}_{\frk h}(\frk g; M) $
we can define
$$ C^{p,q}_{\frk h}(\frk g; M) \doteq N^{p,q}_{\frk h}(\frk g; M) / N^{p+1,q-1}_{\frk h}(\frk g; M)  $$
and since $\dext N^{p,q}_{\frk h}(\frk g; M) \subset N^{p,q+1}_{\frk h}(\frk g; M)$ we can define an operator
$$ \dext_{\frk h} : C^{p,q}_{\frk h}(\frk g; M) \to C^{p,q+1}_{\frk h}(\frk g; M)$$
and we have a complex.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% YOU HAVE TO FINISH DEFINING THIS OBJECTS !!! %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Therefore define for $p \geq 0$ we denote the set of the $(p,q)$-cocycles elements by $$ Z^{p,q}_{\frk h} (\frk g; M) = \ker \left( \dext : C^{p,q}_{\frk h}(\frk g; M) \to C^{p,q+1}_{\frk h}(\frk g; M) \right),$$
the set of $(p,q)$-coboundaries by
 $$ B^{p,q}_{\frk h}(\frk g; M) = \img \left( \dext : C^{p,q-1}_{\frk h}(\frk g; M) \to C^{p,q}_{\frk h}(\frk g; M) \right),$$
and the $(p,q)$-cohomology classes by
 $$ H^{p,q}_{\frk h}(\frk g; M) = \frac{Z^{p,q}_{\frk h}(\frk g; M)}{B^{p,q}_{\frk h}(\frk g; M)}.$$
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% I WAS DOING SOMETHING HERE AND I STOPED. WHAT WAS I DOIND ? %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \begin{exa} Let $G$ be a semisimple compact Lie group endowed with a complex Lie algebra $\frk h \subset \frk g$.
% \end{exa}
 
Notice that if $\frk h$ is a subalgebra of $\frk g$, then the space $C^p(\frk g / \frk h; M)$ has a natural structure of $\frk h$-module given by $$(X \cdot u)([X_1], \ldots, [X_p]) = X \cdot u([X_1], \ldots, [X_p]) - \sum_{j=1}^p  u([X_1], \ldots, [ [X, X_j] ], \ldots, [X_p]).$$


 With this structure we have the following theorem:
 
\begin{thm}
The complexes $(C^{p,q}_{\frk h}(\frk g; M), \dext_{\frk h})$ and $(C^q(\frk h; C^p(\frk g / \frk h; M)), \dext)$ are isomorphic and $$ H^{p,q}_{\frk h}(\frk g; M) = H^{q}(\frk h; C^p(\frk g / \frk h ; M)). $$
\end{thm}

To prove this theorem we need the following definition and two results from Hochschild and Serre \cite{hochschild1953cohomology}.

\begin{dfn}
We define the map $\tilde r : N^{p,q}_{\frk h}(\frk g; M) \to C^q(\frk h; C^p(\frk g/ \frk h; M))$ by

	$$ [(ru)(X_1, \ldots, X_q)]([Y_1], \ldots, [Y_p]) = u(X_1, \ldots, X_q, Y_1, \ldots, Y_p) $$
    with $X_1, \ldots, X_q \in \frk h$ and $[Y_1], \ldots, [Y_p] \in \frk g / \frk h$.
\end{dfn}

\begin{lem}
The map $$ r : N^{p,q}_{\frk h}(\frk g; M) \to C^q(\frk h; C^p(\frk g/ \frk h; M))$$ is surjective and it induces a isomorphism of $C^{p,q}_{\frk h}(\frk g; M)$ on $C^q(\frk h; C^p(\frk g/ \frk h; M))$ which we denote by $$r^{p,q} : C^{p,q}_{\frk h}(\frk g; M) \to C^p(\frk h; C^q(\frk g/ \frk h; M)).$$
\end{lem}

\begin{proof}
The surjectivity is easy. Take $\pi : \frk g \to \frk g / \frk h$ as the quotient map and $T : \frk g \to \frk h$ any linear map being the identity when restricted to $\frk h$. Now, let $v \in C^q(\frk h; C^p(\frk g/ \frk h; M))$ and define $$ u(X_1, \ldots, X_{p+q}) =  \frac{1}{p!q!} \sum_{\sigma \in S_{p+q}} v(TX_{\sigma(1)}, \dots, TX_{\sigma(q)})(\pi X_{\sigma(p+1)}, \ldots, \pi X_{\sigma(p+q)}).$$ Then clearly $u \in N^{p,q}_{\frk h}(\frk g; M)$. We have to verify that $ru \in C^q(\frk h; C^p(\frk g/ \frk h; M))$. Let $X_1, \ldots, X_q \in \frk h$ and $[Y_1], \ldots, [Y_p] \in \frk g/ \frk h$. We have that, by writing $X_{q+j} = Y_j$, we have
$$
\begin{aligned}
(ru)(X_1, \ldots, X_q) & ([X_{q+1}], \ldots, [X_{q+p}]) =  \\
	& = \frac{1}{p!q!} \sum_{\sigma \in S_{p+q}} v(TX_{\sigma(1)}, \dots, TX_{\sigma(q)})(\pi X_{\sigma(p+1)}, \ldots, \pi X_{\sigma(p+q)}) \\
    & = \frac{1}{p!q!} \sum_{\sigma \in S_{p}} \sum_{\tau \in S_{p}} v(TX_{\sigma(1)}, \dots, TX_{\sigma(p)})(\pi Y_{\tau(1)}, \ldots, \pi Y_{\tau(q)}).
\end{aligned}
$$
The last equality holds because any term whose permutation change $X_j$ with $X_{j+q}$ is going to be zero, therefore we can sum only over permutation of the form $(\sigma, \tau)$ with $\sigma$ permuting the first $q$ elements and $\tau$ the last $p$ elements.

Now notice that $$
\begin{aligned}
\frac{1}{p!q!} \sum_{\sigma \in S_{p}} \sum_{\tau \in S_{p}} & v(TX_{\sigma(1)}, \dots, TX_{\sigma(p)})(\pi Y_{\tau(1)}, \ldots, \pi Y_{\tau(q)}) \\
	& = \frac{1}{q!}\sum_{\sigma \in S_{q}} \frac{1}{p!}\sum_{\tau \in S_{p}} v(TX_{\sigma(1)}, \dots, TX_{\sigma(p)})(\pi Y_{\tau(1)}, \ldots, \pi Y_{\tau(q)}) \\
    & =  \frac{1}{q!}\sum_{\sigma \in S_{q}}  v(TX_{\sigma(1)}, \dots, TX_{\sigma(p)})(\pi Y_1, \ldots, \pi Y_q) \\
    & =  \sum_{\sigma \in S_{q}} v(TX_{1}, \dots, TX_{p})(\pi Y_1, \ldots, \pi Y_q) \\
\end{aligned}
$$ and so we proved the surjectivity. Therefore, to finish the proof all we need to do is show that $\ker r = N^{p+1, q-1}_{\frk h}(\frk g; M)$. Clearly it holds that $N^{p+1, q-1}_{\frk h}(\frk g; M) \subset \ker r$ and the other side follows directly from the definition.
\end{proof}

And we have the following result that follows directly from the definition of the operators $\dext$ and $\dext'$.

\begin{lem}
\label{bott_like_formula_commutativity} We have that $ r^{p,q+1} \circ \dext' = \dext \circ r^{p,q}$ in which $\dext$ is the coboundary operator on $C^q(\frk h; C^p(\frk g/ \frk h; M))$ and $\dext'$ is the coboundary operator on $C^{p,q}_{\frk h}(\frk g; M)$, in other words, the following diagram is commutative:
$$ \xymatrix{
C^{p,q}_{\frk h}(\frk g; M) \ar[r]^{ \dext' } \ar[d]_{ r^{p,q} } & C^{p,q+1}_{\frk h}(\frk g; M) \ar[d]^{ r^{p,q+1} } \\
C^q(\frk h; C^p(\frk g/ \frk h; M)) \ar[r]_{ \dext } & C^{q+1}(\frk h; C^p(\frk g/ \frk h; M)) \\
}$$
\end{lem}

\begin{cor} The isomorphism above induces an isomorphism
$$ r^{p,q} : H^{p,q}_{\frk h}(\frk g; M) \to H^q(\frk h; C^p(\frk g/ \frk h; M)).$$
\end{cor}

With the language introduced in this subsection we have the following important example.

\begin{exa}
Let $\Omega$ be a complex manifold and $\mathbb{E}$ a holomorphic vector bundle over $\Omega$. We set $R = C^\infty(\Omega; \C)$ and $M = \Gamma^\infty(\mathbb{E})$ the set of all smooth global sections of $\mathbb{E}$. Under pointwise multiplication, $M$ is a $R$-module.

In this case we can decompose $\mathcal D$, as $R$-modules, into the direct sum of two $R$-closed Lie subalgebras:
$$ \mathcal D = \mathcal D_\alpha \oplus \mathcal D_\beta$$
where $\mathcal D_\alpha$ is the set of all derivations which annihilate all local anti-holomorphic functions in $\Omega$ and $\mathcal D_\beta$ the set of all derivations which annihilate all local holomorphic functions.

In this case, $M$ admits a $\mathcal D_\beta$-structure compatible to its $R$-structure, which can be extended to a $\mathcal D$-structure only if $\mathbb{E}$ is locally constant.

The $\mathcal D_\beta$-structure is defined as follows. Let $r = \operatorname{rank}\mathbb{E}$, then every section $s \in M$ can be expressed locally in the form
$s = \sum \lambda_i e_i$ with $\lambda_i \in R$ and $(e_i)_{i=1}^r$ a holomorphic local frame of $\mathbb{E}$ in an open neighborhood $U$. Now, for $X \in \mathcal D_\beta$, let $X \cdot s$ be given by
$$ X \cdot s = \sum_i (X \cdot \lambda_i) e_i.$$

This operation is well-defined because the transitions are holomorphic, in fact, suppose that $(f_i)_{i=1}^r$ is another holomorphic local frame of $\mathbb{E}$ in $U$ and write $ s = \sum_i \mu_i f_i.$

We can write $f_i = \sum_j \nu_{ij} e_j$ with $\nu_{ij}$ holomorphic functions in $U$ and so
$$ s = \sum_i \mu_i (\sum_j \nu_{ij} e_j) = \sum_j ( \sum_i \mu_i\nu_{ij}) e_j.$$

Since $(e_i)_{i=1}^r$ is a local frame we have that $\sum_i \mu_i\nu_{ij} = \lambda_i$ for all $i$  and since $X$ annihilates every local holomorphic function we obtain 
$$X \cdot \lambda_i = X \cdot (\sum_i \mu_i\nu_{ij}) = \sum_i (X \cdot \mu_i) \nu_{ij} .$$

Therefore
$$ X \cdot s = \sum_j X \cdot ( \sum_i \mu_i\nu_{ij}) e_j = \sum_i (X \cdot \mu_i) (\sum_j \nu_{ij} e_j) = \sum_i (X \cdot \mu_i) f_i.$$

The proof that this $\mathcal D_\beta$ structure is compatible with the $R$-structure follows directly from the product rule of derivations.

The complex $C_R(\mathcal D_\beta; M)$ is referred to as the \emph{complex of $\bb E$-valued forms on $X$ of type $(0,q)$} and $H^q(\mathcal D_\beta; M)$ will be denoted by $H^{0,q}(X; \bb E)$.
\end{exa}


Let $\bb E \to \Omega$ and $\bb E' \to \Omega'$ be two holomorphic vector bundles and suppose that $f : \bb E' \to \bb E$ is a holomphic bundle map. Then, as expected, we have induced maps $f^*: C_R(\mathcal D_\beta; M) \to  C_R(\mathcal D_\beta'; M')$ and $f^*: H^{0,q}(\Omega; \bb E) \to  H^{0,q}(\Omega'; \bb E')$.



\begin{lem}
The $R$-modules $B^p_R(\mathcal D_\alpha; M)$ admit a compatible $\mathcal D_\beta$-structure.
\end{lem}

\begin{proof}
In fact, for $X \in \mathcal D_\beta$, $X_i \in \mathcal D_\alpha$ and $u \in B^p_R(\mathcal D_\alpha; M)$ we define
$$ (X \cdot u)(X_1, \ldots, X_p) = X \cdot u(X_1, \ldots, X_p) - \sum_{i} u(X_1, \ldots, \alpha[X, X_i], \ldots, X_p)$$
with $a : \mathcal D \to \mathcal D_\alpha$ being the projection.
The proof that this $\mathcal D_\beta$ structure is compatible with the $R$-structure follows directly from the product rule of derivations.
\end{proof}

\begin{rmk}
The vector space $H^q_R (\mathcal D_\beta; B^p_R(\mathcal D_\alpha; M))$ is written $H^{p,q}(\Omega; \bb E)$ and is refered to as the $(p,q)$-cohomology of $\bb E$.
\end{rmk}


We have a canonical injection of $B^q_R (\mathcal D_\beta; B^p_R(\mathcal D_\alpha; M))$ into $B_R(\mathcal D; M)$ given by the map
$$ (t_{p,q} w)(X_1, \ldots, X_{p,q}) = \frac{1}{(p+q)!} \sum_{\sigma \in S_{p+q}} w(\beta X_{\sigma(1)}, \ldots, \beta X_{\sigma(q)})(\alpha X_{\sigma(q+1)}, \ldots, \alpha X_{\sigma(q+p)})$$
with $\alpha : \mathcal D \to \mathcal D_\alpha$ and $\beta : \mathcal D \to \mathcal D_\beta$ the projections associated to the decomposition $\mathcal D = \mathcal D_\alpha \oplus \mathcal D_\beta$.

Thus $B_R(\mathcal D; M)$ is decomposed into a direct sum $B_R^{p,q}(\mathcal D; M)$ of $\mathbb{E}$-valued forms of the type $(p,q)$. Under the set $\sum t_{p,q}$ the operator $\dext$ of the complex $C_R(\mathcal D_\beta, B_R(\mathcal D_\alpha); M)$ is taken into an operation $\delbar$ on $B_R(\mathcal D; M)$.

%%% and the relation between the operator $\dext$ of the complex $C_R (\mathcal D_\beta; B_R(\mathcal D_\alpha; M))$ and the operation $\delbar$ on $B_R(\mathcal D; M)$.

In the special case when $M = R = C^\infty(\Omega; \C)$, that is, when $\mathbb{E}$ is the trivial bundle $1$, then $B_R(\mathcal D; M) = C_R(\mathcal D; M)$ already has a differential operator $\dext$, and $\dext = \del + \delbar$.

%%%%% \textcolor{red}{Write about line bundles and filtrations if relevant...}

We denote by $C(\frk g, \frk u; R)$ the set of elements of $C(\frk g; R)$ that vanishes when have any parameter is in $\frk u$. This subset is stable under the operator $\dext$ and thus we also can introduce its cohomology space, which is going to be denoted by $H^*(\frk g, \frk u; R)$. With this notation we have:

\begin{exa} Let $U$ be a connected, closed subgroup of $G$ and write $X = G / U$, then
$$ H^*(X; \C) \cong H^*(\frk g, \frk u; R).$$

In fact, the projection $\pi : G \to G / U$ imbeds the chain complex of the forms which are invariant under left translations by $U$ and annihilate vector fields parallel to $U$. Under $\rho^*$ this image therefore maps into $C(\frk g, \frk u; R)$. Because $U$ is connected, $\rho^*$ is onto.
\end{exa}


%\begin{exa} Let $G$ and $U$ be complex Lie groups, with $U$ connected and closed in $G$. Let $\tilde \phi : U \to \operatorname{End}$ be a holomorphic representation of $U$, and $\bb E$ the \textcolor{red}{corresponding} bundle over $G / U = X$. We set $R = C^\infty(G / U; \C)$, $R' = C^\infty(G; \C)$ and $\mathcal D = \mathcal D_\alpha + \mathcal D_\beta$ as defined before.

%The Lie algebras $\frk g$ and $\frk h$ break correspondingly $\frk g = \frk g_\alpha + \frk g_\beta$, $\frk h = \frk h_\alpha + \frk h_\beta$.



%\end{exa}

%%% \todo[inline]{If $G$ is a complex Lie group and $X \in \frk g_\alpha$ and $Y \in \frk g_\beta$ then $[X,Y] = 0$. Since $\frk g = \frk g_\alpha \oplus \frk g_\beta$ and so $\frk g_\alpha$ is an ideal of $\frk g$. But, if $G$ is semisimple, then $\frk g_\R$ is semisimple and this means that $\frk g$ is semisimple and so $\frk g_\alpha $ cannot be an ideal unless $\frk g_\alpha = \frk g$ or $\frk g_\alpha = {0}$. This appears to be a contradiction.}
%%% There is no contradiction: a semisimple Lie algebra has no non-zero ABELIAN ideals



















%%%%%%%%%%%%%%%%%%%%%%%
%%% THE END IS NEAR %%%
%%%%%%%%%%%%%%%%%%%%%%%


==> sec-hodge-decomposition.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% HODGE DECOMPOSITION %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Hodge decomposition}
\label{sec:hodge_theory}

In this section we are going to explain how to use the Hodge decomposition for the operator $\dext'$. With this decomposition we are going to find some simple conditions so that the cohomology is finite dimensional on a specific degree. Usually, Hodge decomposition is introduced in the context of elliptic differential operators between Hermitian vector bundles. Here we made a small improvement, we assumed that the operator is subelliptic. See Definition \ref{dfn:subellipticity_and_stuff}.

Suppose that $\Omega$ is a compact manifold with a positive $\mathcal C^\infty$-density $\mu$ and let $E_j$, for $j = 1, 2, 3$ be three Hermitian vector bundles over $\Omega$. We denote by $\ip{,}_j$ the hermitian inner product on $E_j$. Let $$A_j : \mathcal C^\infty(\Omega; E_j) \to \mathcal C^\infty(\Omega; E_{j+1}), \qquad j = 1, 2$$ be partial differential operators of order $m$ satisfying $A_2 \circ A_1 = 0$. That is we have 
$$ \mathcal C^\infty(\Omega; E_1) \xrightarrow{A_1}{} \mathcal C^\infty(\Omega; E_{2})  \xrightarrow{A_2}{}  \mathcal C^\infty(\Omega; E_3).$$

We endow $\mathcal C^\infty(\Omega; E_j)$ with the inner product
$$\iip{u,v}_j \doteq \int_\Omega \ip{u(x),v(x)}_j \dint \mu(x),$$
for $u, v \in \mathcal C^\infty(\Omega; E_j)$ and we  define the operators $A_j^* : \mathcal C^\infty(\Omega; E_{j+1}) \to \mathcal C^\infty(\Omega; E_{j})$ by
$$ \iip{A_j u, v }_{j+1} = \iip{u, A^*_j v}_{j+1}$$
for $u \in \mathcal C^\infty(\Omega; E_{j})$ and $v \in \mathcal C^\infty(\Omega; E_{j+1}).$

Now we have everything we need to introduce the Hodge operator:

\begin{dfn}
For $u \in \mathcal C^\infty(\Omega; E_2)$ we define $\Box u \doteq (A_1 A_1^* + A_2^* A_2) u$, and, in the sense of distributions, we define $$D(\Box) = \{u \in L^2(\Omega; E_2): \Box u \in L^2(\Omega; E_2) \}$$ and $$\Box : D(\Box) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ is a densely defined operator called \emph{Hodge operator}, \emph{Hodge Laplacian} or just \emph{Box operator}.
\end{dfn}

% because $\mathcal C^\infty(\Omega; E_2) \subset D(\Box)$ is a dense subset of $L^2(\Omega; E_2)$.

The operator $\Box$ has closed graph. In fact, let $u_j, v_j \in L^2(\Omega; E_2)$ be a sequence satisfying $\Box u_j = v_j$ and suppose that $u_j \to u \in L^2(\Omega; E_2)$ and $v_j \to v \in L^2(\Omega; E_2)$. We want to show that $u \in D(\Box)$ and $\Box u = v$. Since $u_j \to u$ and $v_j \to v$ in $L^2(\Omega; E_2)$ we have have this convergence in $\mc D'(\Omega; E_2)$ and since $\Box$ is a differential operator it is continuous in $\mc D'(\Omega; E_2)$ so we can apply the closed graph theorem and conclude that $\Box u = v$ in the sense of distributions. By hypothesis we have $u,v \in L^2(\Omega; E_2)$ and so $u \in D(\Box)$.

We also remark that
$$
\begin{aligned}
\iip{\Box u, u}
	& = \iip{A_1 A_1^*u, u} + \iip{A_2^* A_2u, u} \\
	& = \iip{A_1^*u, A_1^*u} + \iip{A_2 u, A_2 u} \\
	& = \|A_1^*u\|_1^2 + \|A_2 u\|_3^2
\end{aligned}
$$
and so we have the following result:

\begin{prp}
\label{prp:kernel_Box_decomposition} The kernel of the operator $\Box$ is
$$ \ker \Box = \{u \in L^2(\Omega; E_2): A_1^*u = 0 \text{ and } A_2 u = 0\}. $$
\end{prp}

In the following definition we introduce two concepts regarding the regularity of differential operators. Under certain conditions, these concepts provide sufficient conditions so that the kernel of the differential operator has finite dimension.

\begin{dfn}
\label{dfn:subellipticity_and_stuff} Let $E$ be a vector bundle over $\Omega$ and consider a linear partial differential operator $P : \mc D' (\Omega; E) \to \mc D'(\Omega; E)$. For an $\epsilon > 0$, the operator $P$ is said to be \emph{$\epsilon$-subelliptic} if $Pu \in H^s(\Omega;E)$ implies that $u \in H^{s+\epsilon}(\Omega; E)$ for all $u \in H^s(\Omega; E)$. The operator $P$ is said to be \emph{globally hypoelliptic} if, given $u \in \mc D'(\Omega; E)$ such that $Pu \in \mathcal C^\infty(\Omega;F)$ it holds that $u \in \mathcal C^\infty(\Omega;E)$. Notice that subellipticity implies global hypoellipticity.
\end{dfn}

On the above definition it is not necessary to assume that the manifold $\Omega$ is compact.

The following proposition is a well known result about differential operators on compact manifolds. 

\begin{prp} If $P : \mc D' (\Omega; E) \to \mc D'(\Omega; F)$ is globally hypoelliptic, then $$\dim \ker P < \infty.$$
\end{prp}

\begin{proof} 
Since $P$ is globally hypoelliptic we have that $\ker P \subset \mathcal C^\infty(\Omega; E)$. Consider $\ker P$ with the topology induced by $L^2(\Omega; E)$. Notice that this induced topology agrees with the topology induced by $H^s(\Omega; E)$ for any $s \in \R$ and take $B = \{ u \in \ker P: \|u\|_1 \leq 1 \}$ and note that $B$ is closed and bounded. By the Rellich lemma, we know that the inclusion $H^1(\Omega; E) \to H^0(\Omega; E) = L^2(\Omega; E)$ is compact and so $B$ is compact.
\end{proof}

In this work we are interested in the case in which $P$ is the Hodge operator. Therefore, we need to establish some conditions so that the Hodge operator is globally hypoelliptic. But first we need to finish our decomposition. We need the next lemma which is a basic result on Hilbert spaces. 

%\begin{lem} 
%Let $H_1$ and $H_2$ be Hilbert spaces with norms $\|.\|_1$ and $\|.\|_2$. If $T : H_1 \to H_2$ is a linear, closed and densely defined operator such that there is a constant $C > 0$ such that
%$$\|f\|_1 \leq C \|Tf\|_2$$
%for all $ f \in D(T) \cap \overline{\img(T^*)}$,
%then $\img(T)$ is closed.
%\end{lem}
%
%\begin{proof} 
%Let $f_k \in \img(T)$ such that $f_k \to f$ in $H_2$. We want to show that there exist $g \in D(T)$ satisfying $Tg = f$. Let $g_k \in D(T)$ with $Tg_k = f_k$. Since $\ker T^\perp = \overline{\img(T^*)}$, we can assume that $g_k \in \overline{\img (T^*)}$. Notice that we have
%$$\|g_k - g_l\|_1 \leq C\|Tg_k - Tg_l \|_2 = C\|f_k - f_l\|_2.$$
%Since $\{f_k\}$ is a convergent sequence, it is a Cauchy sequence and so also is $\{g_k\}$. Therefore there exists $g \in H_1$ with $g_k \to g$. Since $T$ has closed graph we have that $(g_k, f_k) \to (g,f) \in \{(x, Tx): x \in H_1\}$ and so $f = Tg$.
%\end{proof}

This next proposition shows another important result regarding subellipticity of the Hodge operator. By itself this proposition is interesting, but it is also necessary for the decomposition.

\begin{prp} If the operator $\Box$ is $\epsilon$-subelliptic, then there exists $C > 0$  such that
\begin{equation}
    \|u\|_0 \leq C \|\Box u\|_0, \qquad u \in (\ker \Box)^\perp \cap D(\Box).
\end{equation}
%$\img(\Box)$ is closed in $L^2(\Omega; E_2).$
\end{prp}

\begin{proof} %Since $\Box$ is $\epsilon$-subelliptic, we have that if $u \in D(\Box)$ then $u \in H^\epsilon(\Omega; E_2)$ and by 
Defining the norm $$ u \mapsto \left\{ \|u\|_0^2 + \|\Box u\|_0^2 \right\}^{1/2} $$ on $$ D(\Box) = \{ u \in L^2(\Box; E_2) : \Box u \in L^2(\Box; E_2) \}$$ gives a Hilbert space and subellipticity gives $D(\Box) \subset H^\epsilon(\Omega; E_2)$. By the closed graph theorem, there exists a constant $C > 0$ such that
$$ \|u\|_\epsilon \leq C (\|\Box u\|_0 + \|u\|_0)$$
for all $u \in D(\Box)$. So, if $u \in (\ker \Box)^\perp \cap D(\Box)$, we have that $$\|u\|_\epsilon \leq C \|\Box u\|_0.$$
Indeed, suppose that this last inequality is not valid, then for every $j$ there exist a $u_j$ such that $\|u\|_\epsilon \geq j\|\Box u _j\|_0$. Notice that if we take $v_j = u_j/\|u\|_\epsilon\|$ we have $\|v_j\|_\epsilon = 1$ and $\|\Box v_j\| < 1/j$. There exists a subsequence $\{v_{j_k}\}$ such that $v_{j_k} \to v$ in $L^2(\Omega; E_2)$ and clearly $v \in \ker \Box \cap (\ker \Box)^\perp$. Notice that $$ 1 \leq C (\|\Box v_{j_k}\|_0 + \|v_{j_k}\|_0)$$ and so
$$ 1 \leq C \|v\|_0$$
a contradiction. The proof is complete.
\end{proof}

A standard argument, making use of 2.10 (see, for instance, Lemma 4.1.1 in \cite{hormander1973introduction}), shows the existence of a bounded linear operator $G : (\ker \Box)^\perp \to (\ker \Box)^\perp$ with $\|G\| \leq C$ such that $\Box G f = f$ for $f \in \ker \Box.$ Now, given $g \in L^2(\Omega; E_2)$, we can write $g = f + h$ with $h \in \ker \Box$ and $f \in (\ker \Box)^\perp$. Hence $g = \Box G f + h$. Moreover, if $g \in \mc C^\infty(\Omega; E_2)$ both $f$ and $h$ also are in $\mc C^\infty(\Omega; E_2)$, and also $Gf \in \mc C^\infty(\Omega; E_2)$ because $\Box$ is hypoelliptic.   
%Now we are going to see that even with weaker conditions, the Hodge Laplacian still has some nice properties.

%\begin{prp} 
%Suppose that $\Box$ is $\epsilon$-subelliptic. Let $D(T) = H^{\epsilon}(\Omega; E_2)$ and define $$T : D(T) \subset L^2(\Omega; E_2) \to L^2(\Omega; E_2)$$ by $Tu = \Box u$ for $u \in D(T)$. Then $T$ is a self-adjoint operator. Particularly, we have $$L^2(\Omega;E_2) = \ker T \oplus \img T.$$
%\end{prp}

%\begin{proof}
% Notice that $$\iip{\Box u, v}_2 = \iip{u, \Box v}_2$$
%for all $u, v \in \mathcal C^\infty(\Omega; E_2).$ Since $\mathcal C^\infty(\Omega; E_2)$ is a dense subset of $H^{\epsilon}(\Omega; E_2)$, given $u, v \in H^{\epsilon}(\Omega; E_2)$ there exist sequences $\{u_j\}$ and $\{v_j\}$ in $\mathcal C^\infty(\Omega; E_2)$ such that $u_j \to u$ and $v_j \to v$ in $H^{\epsilon}(\Omega; E_2)$ and so
%$\Box u_j \to \Box u$ and $\Box v_j \to \Box v$ in $L^2(\Omega; E_2)$ and since $$\iip{\Box u_j, v_j}_2 = \iip{u_j, \Box v_j}_2$$
%for all $j$. Therefore we conclude that $\iip{\Box u, v}_2 = \iip{u, \Box v}_2$ and so $\iip{T u, v}_2 = \iip{u, T v}_2$ and $T$ is a symmetric operator.

%To conclude we have to show that $D(T) = D(T^*)$. Let $v \in D(T^*)$. The operator $$ u \in D(T) \mapsto \iip{Tu, v}_2 $$ is continuous in $D(T)$ and so there exists a constant $C > 0$ such that
%$$ |\iip{Tu, v}_2 | \leq C\|u\|_2, \qquad \forall u \in D(T).$$
%Particularly, if we define $S \in \mc D'(M; E_2)$ by $S(\phi) = \iip{T\phi, u}$ for $\phi \in \mathcal C^\infty(\Omega; E_2)$, we have that there exists $w \in L^2(\Omega; E_2)$ such that $\iip{T \phi, u}_2 = \iip{\phi,w}_2$ and so $$ \overline{w}(\phi) = \overline{u}(\Box \phi)$$ for all $\phi \in \mathcal C^\infty(\Omega; E_2)$, that is $\Box \overline{u} = \overline{w}$ in $\mc D'(\Omega;E_2)$ and since $w \in L^2(\Omega;E_2)$ we have $w \in H^{\epsilon}(\Omega;E_2) = D(T)$.
%\end{proof}

% Assume that $\Box$ is $\epsilon$-subelliptic. We have that there exists $C > 0$ satisfying
% $$ \|u\|_0 \leq C\|\Box u\|_0$$
% for all $u \in D(\Box) \cap \ker \Box^\perp$ and according to Lemma 4.1.1 in \cite{hormander1973introduction} given any $f \in \ker \Box^\perp$ there is $u \in L^2(\Omega; E_2)$, $\|u\|_0 \leq C \|f\|_0$ such that $\Box u = f$. Let $\Pi$ denote the orthogonal projection on $\ker \Box^\perp$ and, for $f \in L^2(\Omega; E_2)$ let $Gf$ be the unique solution to $\Box u = \Pi f$ which is orthogonal to the kernel of $\Box$ in $L^2(\Omega; E_2)$. Then $G : L^2(\Omega; E_2) \to L^2(\Omega; E_2)$ is bounded, with norm $ \leq C$, and $\Box G = \Pi$ in $L^2(\Omega; E_2)$. We shall refer to $G$ as the Green operator of $\Box$.

% And we have everything we need to prove the main result of this section.

We have proved:

\begin{prp} If $\Box$ is $\epsilon$-subelliptic then
we have the Hodge decomposition
\begin{equation}
	\label{eq:hodge_decomposition}
	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box(\mathcal  C^\infty(\Omega;E_2) ) = \ker \Box \oplus A_1 ( \mathcal C^\infty(\Omega;E_1) ) \oplus A_2^* (\mathcal C^\infty(\Omega;E_3))
\end{equation}
and
\begin{equation}
	\label{eq:hodge_decomposition_isomorphism}
	\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.
\end{equation}

\end{prp}

% \begin{proof} Let $f \in \mathcal C^\infty(\Omega; E_2)$. We write $f = f_1 + f_2$ with $f_1 \in \ker \Box $ and $f_2 \in \img(T)$. Since $f_2 \in \img(\Box)$ we can write $f_2 = \Box u$ for some $u \in H^\epsilon(\Omega; E_2)$. Notice that since $\Box f_1 = 0$ we have $f_1 \in \mathcal C^\infty(\Omega;E_2)$ and so $f_2 = f - f_1 \in \mathcal C^\infty(\Omega;E_2)$ and since $f_2 = \Box u$ we have $u \in \mathcal C^\infty(\Omega;E_2)$ and we obtained the Hodge decomposition:
% $$ \mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus \Box( \mathcal C^\infty(\Omega;E_2) ) .$$

% If $u \in \mathcal C^\infty(\Omega;E_2)$ such that $A_2u=0$, then we can write $u = u_1 + \Box u_2$ with $\Box u_1 = 0$ and $u_2 \in \mathcal C^\infty(\Omega;E_2).$ We have $u = u_1 + A^*_2 A_2 u_2 + A_1 A^*_1 u_2$. Applying $A_2$ on both sides of this equality and using Proposition \ref{prp:kernel_Box_decomposition} we conclude that
% $$ A_2 A^*_2 A_2 u_2 = 0.$$
% We have $A_2^*A_2 u_2 = 0$ because $\iip{A_2^* A_2 u_2, A_2^* A_2 u_2} = \iip{A_2 u_2, A_2 A_2^* A_2 u_2} = 0$ and then $u = u_1 + A_1 A^*_1 u_2,$ that is $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} \cong \ker \Box.$$
% \end{proof}

% The following version of the decomposition is more suitable for the application in this work.

% \begin{prp} If $\Box$ is $\epsilon$-subelliptic, then
% we have the decomposition
% \begin{equation}
% 	\label{eq:second_hodge_decomposition}
% 	\mathcal C^\infty(\Omega;E_2) = \ker \Box \oplus A_1 ( \mathcal C^\infty(\Omega;E_1) ) \oplus A_2^* (\mathcal C^\infty(\Omega;E_3)).
% \end{equation}
% The space $$\frac{ \ker A_2 }{ A_1(\mathcal C^\infty(\Omega; E_2))} $$ is isomorphic to $\ker \Box$ with each equivalence class in the former having a unique representative in the latter.
% \end{prp}

